The Near and Mid-infrared photometric properties of known redshift $z\geq5$ Quasars

We assemble a catalogue of 488 spectroscopically confirmed very high ($z\geq5.00$) redshift quasars and report their near- ($ZYJHK_{s}/K$) and mid- (WISE W1234) infrared properties. 97\% of the VH$z$Q sample is detected in one or more NIR ($ZYJHK/K_{s}$) band, with lack of coverage rather than lack of depth being the reason for the non-detections. 389 (80\%) of the very high redshift quasars are detected at 3.4$\mu$m in the W1 band from the unWISE catalog and all of the $z\geq7$ quasars are detected in both unWISE W1 and W2. Using archival WFCAM/UKIRT and VIRCAM/VISTA data we check for photometric variability that might be expected from super-Eddington accretion. We find 28 of the quasars have sufficient NIR measurements and signal-to-noise ratio to look for variability. Weak variability was detected in multiple bands of SDSS J0959+0227, and very marginally in the $Y$-band of MMT J0215-0529. Only one quasar, SDSS J0349+0034, shows significant differences between WFCAM and VISTA magnitudes in one band. With supermassive black hole accretion likely to be redshift invariant up to very high-redshift, further monitoring of these sources is warranted. All the data, analysis codes and plots used and generated here can be found at: https://github.com/d80b2t/VHzQ}{\tt github.com/d80b2t/VHzQ.

==> Makefile <==

TEXFILE=VHzQ_MNRAS_rv1
TEXFILE_TWO=PhotometricBands_Conversions
default: all

# just run it


bib: 
	bibtex ${TEXFILE}

all :
	pdflatex  ${TEXFILE}
	pdflatex  ${TEXFILE}
	bibtex ${TEXFILE}
	bibtex ${TEXFILE}
	bibtex ${TEXFILE}
	pdflatex  ${TEXFILE}
	pdflatex  ${TEXFILE}
#	pdflatex  ${TEXFILE}
#	dvipdf ${TEXFILE}
	rm -f  ${TEXFILE}.aux
#	rm -f  ${TEXFILE}.bbl
	rm -f  ${TEXFILE}.blg
	rm -f  ${TEXFILE}.dvi
	rm -f  ${TEXFILE}.log
	rm -f  ${TEXFILE}.out
	rm -f  ${TEXFILE}.toc
#	dvips ERQs_PaperI_rv2.dvi 
#	ps2pdf ERQs_PaperI_rv2.ps
#	rm -f ERQs_PaperI_rv2.ps
	open ${TEXFILE}.pdf

tect :
	tectonic ${TEXFILE}.tex
	open ${TEXFILE}.pdf


clean:
	rm -f \
	${TEXFILE}.dvi \
	${TEXFILE}.ps \
	${TEXFILE}.out \
	${TEXFILE}.aux \
	${TEXFILE}.bbl \
	${TEXFILE}.blg \
	${TEXFILE}.toc \
	${TEXFILE}.log 
#	${TEXFILE}.pdf


PhotometricBands :
	pdflatex  ${TEXFILE_TWO}
	pdflatex  ${TEXFILE_TWO}
	bibtex ${TEXFILE_TWO}
	bibtex ${TEXFILE_TWO}
	pdflatex  ${TEXFILE_TWO}
	pdflatex  ${TEXFILE_TWO}
	rm -f  ${TEXFILE_TWO}.aux
	rm -f  ${TEXFILE_TWO}.bbl
	rm -f  ${TEXFILE_TWO}.blg
	rm -f  ${TEXFILE_TWO}.dvi
	rm -f  ${TEXFILE_TWO}.log
	rm -f  ${TEXFILE_TWO}.out
	rm -f  ${TEXFILE_TWO}.toc
	open ${TEXFILE_TWO}.pdf


==> RossCrossTable3Update.tex <==
PSO & J000.3401+26.8358 & 0.34011 & 26.83588 & 5.75 & --- & 19.32\pm0.048 & --- & ---
SDSS & J0002+2550 & 0.66412 & 25.84304 & 5.82 & --- & 19.37\pm0.087 & --- & ---
SDSS & J0005-0006 & 1.46808 & -0.1155 & 5.85 & 20.70\pm0.211 & 20.73\pm0.177 & 20.05\pm0.082 & 20.49\pm0.140
PSO & J002.1073-06.4345 & 2.10739 & -6.43456 & 5.93 & --- & 20.26\pm0.040 & --- & 19.74\pm0.082
SDWISE & J0008+3616 & 2.21429 & 36.27041 & 5.17 & --- & 19.33\pm0.079 & --- & ---
PSO & J002.3786+32.8702 & 2.3787 & 32.87026 & 6.1 & --- & 22.17\pm0.855 & --- & ---
SDSS & J0012+3632 & 3.137 & 36.53781 & 5.44 & --- & 19.01\pm0.061 & --- & ---
SDSS & J0017-1000 & 4.31117 & -10.0154 & 5.01 & 19.24\pm0.032 & 19.26\pm0.045 & --- & 18.78\pm0.065
PSO & J004.3936+17.0862 & 4.39361 & 17.0863 & 5.8 & --- & 20.74\pm0.075 & --- & 20.28\pm0.114
PSO & J004.8140-24.2991 & 4.81408 & -24.29916 & 5.68 & 19.54\pm0.048 & 19.19\pm0.049 & --- & 19.07\pm0.090
VDES & J0020-3653 & 5.13112 & -36.89495 & 6.9 & --- & 20.42\pm0.100 & --- & 19.32\pm0.096
SDSS & J0023-0018 & 5.87779 & -0.31011 & 5.06 & 20.62\pm0.148 & 20.50\pm0.083 & 20.25\pm0.118 & 20.27\pm0.102
PSO & J006.1240+39.2219 & 6.12404 & 39.22193 & 6.62 & --- & 21.28\pm0.483 & --- & ---
SDWISE & J0025-0145 & 6.36183 & -1.75903 & 5.07 & 18.03\pm0.020 & 17.95\pm0.020 & 17.74\pm0.004 & 17.59\pm0.022
PSO & J007.0273+04.9571 & 7.02733 & 4.95712 & 6.0 & 20.22\pm0.088 & 20.04\pm0.108 & 20.40\pm0.196 & 20.27\pm0.188
SDWISE & J0031+0710 & 7.85775 & 7.17692 & 5.33 & 20.03\pm0.099 & 20.20\pm0.206 & 19.49\pm0.141 & 19.61\pm0.157
CFHQS & J0033-0125 & 8.2975 & -1.42358 & 6.13 & --- & 21.41\pm0.264 & 21.32\pm0.335 & 20.79\pm0.206
SDSS & J0034+3759 & 8.55979 & 37.99833 & 5.63 & --- & 19.70\pm0.113 & --- & ---
PSO & J009.3573-08.1190 & 9.35733 & -8.11902 & 5.72 & 20.13\pm0.050 & 19.88\pm0.063 & --- & 19.80\pm0.138
DELS & J0038-1527 & 9.65042 & -15.45656 & 7.02 & --- & --- & --- & ---
PSO & J009.7355-10.4316 & 9.73551 & -10.43164 & 6.0 & --- & --- & --- & ---
PSO & J011.3899+09.0325 & 11.38987 & 9.03249 & 6.42 & 21.04\pm0.304 & --- & 20.64\pm0.244 & 20.76\pm0.336
PSO & J0046-2837 & 11.59854 & -28.62982 & 5.99 & 21.25\pm0.125 & 20.89\pm0.079 & 20.61\pm0.112 & 20.22\pm0.111
CFHQS & J0050+3445 & 12.52777 & 34.75601 & 6.25 & --- & 19.97\pm0.151 & --- & ---


==> Ross_Cross_2020_Table3.tex <==
\begin{table}
\begin{tabular}{llrrc cccc cccc}
 \hline
 \hline
  \multirow{2}{*}{Survey} &  \multirow{2}{*}{QsoName} &   R.A. / deg  &   Decl. / deg  &  \multirow{2}{*}{redshift}   &  \multirow{2}{*}{Y}  &  \multirow{2}{*}{J}   &  \multirow{2}{*}{H}  &  \multirow{2}{*}{K}     &  \multicolumn{2}{c}{unWISE}  &  \multicolumn{2}{c}{AllWISE} \\ 
                          &                           &   (J2000)     &  (J2000)       &                              &                      &                       &                      &                         &          W1       & W2       & W3   & W4 \\ 
  \hline
  \hline
  \\
PSO & J000.3401+26.8358 &    0.34011 &   26.83588 &  5.75   &   $-999999500.00\pm-999999500.000$  &  $19.32\pm0.048$  &  $-999999500.00\pm-999999500.000$   & $-999999500.00\pm-999999500.000$    &   $18.949\pm0.026$   &  $18.80\pm0.050$   &   $17.74\pm0.492$   &   $15.42\pm-999999488.000$   \\
SDSS & J0002+2550 &    0.66412 &   25.84304 &  5.82   &   $-999999500.00\pm-999999500.000$  &  $19.37\pm0.087$  &  $-999999500.00\pm-999999500.000$   & $-999999500.00\pm-999999500.000$    &   $18.919\pm0.026$   &  $18.70\pm0.047$   &   $17.56\pm0.423$   &   $15.34\pm-999999488.000$   \\
SDSS & J0005-0006 &    1.46808 &   -0.11550 &  5.85   &   $20.70\pm0.211$  &  $20.73\pm0.177$  &  $20.05\pm0.082$   & $20.49\pm0.140$    &   $20.162\pm0.079$   &  $19.98\pm0.153$   &   $17.59\pm-999999488.000$   &   $15.67\pm-999999488.000$   \\
PSO & J002.1073-06.4345 &    2.10739 &   -6.43456 &  5.93   &   $-999999500.00\pm-999999500.000$  &  $20.26\pm0.040$  &  $-999999500.00\pm-999999500.000$   & $19.74\pm0.082$    &   $19.471\pm0.045$   &  $19.24\pm0.078$   &   $17.04\pm-999999488.000$   &   $15.42\pm-999999488.000$   \\
SDWISE & J0008+3616 &    2.21429 &   36.27041 &  5.17   &   $-999999500.00\pm-999999500.000$  &  $19.33\pm0.079$  &  $-999999500.00\pm-999999500.000$   & $-999999500.00\pm-999999500.000$    &   $18.687\pm0.021$   &  $18.71\pm0.044$   &   $17.19\pm-999999488.000$   &   $15.45\pm-999999488.000$   \\
PSO & J002.3786+32.8702 &    2.37870 &   32.87026 &  6.10   &   $-999999500.00\pm-999999500.000$  &  $22.17\pm0.855$  &  $-999999500.00\pm-999999500.000$   & $-999999500.00\pm-999999500.000$    &   $20.620\pm0.106$   &  $-999999484.72\pm-999999488.000$   &   $-999999482.85\pm-999999488.000$   &   $-999999481.34\pm-999999488.000$   \\
SDSS & J0017-1000 &    4.31117 &  -10.01540 &  5.01   &   $19.24\pm0.032$  &  $19.26\pm0.045$  &  $-999999500.00\pm-999999500.000$   & $18.78\pm0.065$    &   $18.645\pm0.022$   &  $18.60\pm0.045$   &   $17.17\pm0.334$   &   $15.18\pm-999999488.000$   \\
PSO & J004.3936+17.0862 &    4.39361 &   17.08630 &  5.80   &   $-999999500.00\pm-999999500.000$  &  $20.74\pm0.075$  &  $-999999500.00\pm-999999500.000$   & $20.28\pm0.114$    &   $20.503\pm0.103$   &  $19.98\pm0.145$   &   $-999999482.85\pm-999999488.000$   &   $-999999481.34\pm-999999488.000$   \\
PSO & J004.8140-24.2991 &    4.81408 &  -24.29916 &  5.68   &   $19.54\pm0.048$  &  $19.19\pm0.049$  &  $-999999500.00\pm-999999500.000$   & $19.07\pm0.090$    &   $18.989\pm0.028$   &  $18.96\pm0.061$   &   $17.27\pm0.344$   &   $15.48\pm-999999488.000$   \\
VDES & J0020-3653 &    5.13112 &  -36.89495 &  6.90   &   $-999999500.00\pm-999999500.000$  &  $20.42\pm0.100$  &  $-999999500.00\pm-999999500.000$   & $19.32\pm0.096$    &   $19.536\pm0.041$   &  $19.69\pm0.102$   &   $17.83\pm-999999488.000$   &   $15.00\pm-999999488.000$   \\
SDSS & J0023-0018 &    5.87779 &   -0.31011 &  5.06   &   $20.62\pm0.148$  &  $20.50\pm0.083$  &  $20.25\pm0.118$   & $20.27\pm0.102$    &   $19.518\pm0.046$   &  $19.41\pm0.093$   &   $17.02\pm-999999488.000$   &   $15.15\pm-999999488.000$   \\
PSO & J006.1240+39.2219 &    6.12404 &   39.22193 &  6.62   &   $-999999500.00\pm-999999500.000$  &  $21.28\pm0.483$  &  $-999999500.00\pm-999999500.000$   & $-999999500.00\pm-999999500.000$    &   $20.033\pm0.064$   &  $-999999484.72\pm-999999488.000$   &   $-999999482.85\pm-999999488.000$   &   $-999999481.34\pm-999999488.000$   \\
SDWISE & J0025-0145 &    6.36183 &   -1.75903 &  5.07   &   $18.03\pm0.020$  &  $17.95\pm0.020$  &  $17.74\pm0.004$   & $17.59\pm0.022$    &   $17.520\pm0.009$   &  $17.51\pm0.018$   &   $16.54\pm0.222$   &   $15.17\pm-999999488.000$   \\
PSO & J007.0273+04.9571 &    7.02733 &    4.95712 &  6.00   &   $20.22\pm0.088$  &  $20.04\pm0.108$  &  $20.40\pm0.196$   & $20.27\pm0.188$    &   $19.847\pm0.060$   &  $19.89\pm0.135$   &   $17.40\pm-999999488.000$   &   $14.98\pm-999999488.000$   \\
SDWISE & J0031+0710 &    7.85775 &    7.17692 &  5.33   &   $20.03\pm0.099$  &  $20.20\pm0.206$  &  $19.49\pm0.141$   & $19.61\pm0.157$    &   $19.327\pm0.039$   &  $18.96\pm0.063$   &   $17.34\pm-999999488.000$   &   $15.06\pm-999999488.000$   \\
CFHQS & J0033-0125 &    8.29750 &   -1.42358 &  6.13   &   $-999999500.00\pm-999999500.000$  &  $21.41\pm0.264$  &  $21.32\pm0.335$   & $20.79\pm0.206$    &   $20.874\pm0.142$   &  $-999999484.72\pm-999999488.000$   &   $-999999482.85\pm-999999488.000$   &   $-999999481.34\pm-999999488.000$   \\
PSO & J009.3573-08.1190 &    9.35733 &   -8.11902 &  5.72   &   $20.13\pm0.050$  &  $19.88\pm0.063$  &  $-999999500.00\pm-999999500.000$   & $19.80\pm0.138$    &   $19.489\pm0.042$   &  $19.48\pm0.095$   &   $17.34\pm-999999488.000$   &   $15.02\pm-999999488.000$   \\
PSO & J009.7355-10.4316 &    9.73551 &  -10.43164 &  6.00   &   $-999999500.00\pm-999999500.000$  &  $-999999500.00\pm-999999500.000$  &  $-999999500.00\pm-999999500.000$   & $-999999500.00\pm-999999500.000$    &   $19.160\pm0.032$   &  $19.00\pm0.061$   &   $17.35\pm-999999488.000$   &   $15.07\pm-999999488.000$   \\
PSO & J011.3899+09.0325 &   11.38987 &    9.03249 &  6.42   &   $21.04\pm0.304$  &  $-999999500.00\pm-999999500.000$  &  $20.64\pm0.244$   & $20.76\pm0.336$    &   $20.442\pm0.104$   &  $-999999484.72\pm-999999488.000$   &   $17.13\pm-999999488.000$   &   $15.44\pm-999999488.000$   \\
CFHQS & J0050+3445 &   12.52777 &   34.75601 &  6.25   &   $-999999500.00\pm-999999500.000$  &  $19.97\pm0.151$  &  $-999999500.00\pm-999999500.000$   & $-999999500.00\pm-999999500.000$    &   $19.250\pm0.033$   &  $18.99\pm0.055$   &   $18.08\pm-999999488.000$   &   $15.96\pm-999999488.000$   \\
SDSS & J0054-0109 &   13.58925 &   -1.15600 &  5.09   &   $19.60\pm0.082$  &  $19.58\pm0.039$  &  $19.35\pm0.045$   & $19.41\pm0.029$    &   $19.651\pm0.057$   &  $19.43\pm0.103$   &   $16.03\pm-999999488.000$   &   $15.04\pm-999999488.000$   \\
CFHQS & J0055+0146 &   13.76212 &    1.77175 &  6.01   &   $24.12\pm3.114$  &  $23.03\pm1.965$  &  $22.38\pm1.552$   & $21.08\pm0.439$    &   $-999999485.331\pm-999999488.000$   &  $-999999484.72\pm-999999488.000$   &   $-999999482.85\pm-999999488.000$   &   $-999999481.34\pm-999999488.000$   \\
SDSS & J0100+2802 &   15.05426 &   28.04053 &  6.33   &   $-999999500.00\pm-999999500.000$  &  $17.60\pm0.016$  &  $17.48\pm0.023$   & $-999999500.00\pm-999999500.000$    &   $17.115\pm0.006$   &  $16.93\pm0.011$   &   $16.86\pm0.211$   &   $15.64\pm0.445$   \\
CFHQS & J0102-0218 &   15.71100 &   -2.30275 &  5.95   &   $-999999488.00\pm-999999488.000$  &  $21.65\pm0.465$  &  $22.65\pm1.628$   & $22.51\pm1.884$    &   $-999999485.331\pm-999999488.000$   &  $-999999484.72\pm-999999488.000$   &   $-999999482.85\pm-999999488.000$   &   $-999999481.34\pm-999999488.000$   \\
SUVAW & J0108+0711 &   17.02750 &    7.18906 &  5.53   &   $19.96\pm0.082$  &  $19.82\pm0.102$  &  $19.55\pm0.114$   & $19.56\pm0.120$    &   $19.008\pm0.031$   &  $18.77\pm0.054$   &   $17.17\pm0.318$   &   $15.23\pm0.401$   \\
SDSS & J0108-0100 &   17.12483 &   -1.00433 &  5.11   &   $20.91\pm0.253$  &  $21.84\pm0.198$  &  $21.15\pm0.204$   & $21.52\pm0.277$    &   $-999999485.331\pm-999999488.000$   &  $-999999484.72\pm-999999488.000$   &   $-999999482.85\pm-999999488.000$   &   $-999999481.34\pm-999999488.000$   \\
VIK & J0109-3047 &   17.47138 &  -30.79064 &  6.79   &   $21.25\pm0.139$  &  $21.28\pm0.135$  &  $21.13\pm0.178$   & $-999999500.00\pm-999999500.000$    &   $20.630\pm0.110$   &  $-999999484.72\pm-999999488.000$   &   $-999999482.85\pm-999999488.000$   &   $-999999481.34\pm-999999488.000$   \\
SUVAW & J0113+0559 &   18.47396 &    5.99753 &  5.00   &   $20.34\pm0.110$  &  $20.21\pm0.141$  &  $19.77\pm0.139$   & $19.62\pm0.112$    &   $19.354\pm0.041$   &  $19.41\pm0.094$   &   $17.64\pm0.501$   &   $15.04\pm-999999488.000$   \\
SDSS & J0115+0015 &   18.93658 &    0.25414 &  5.10   &   $20.77\pm0.148$  &  $20.46\pm0.036$  &  $20.15\pm0.057$   & $19.92\pm0.041$    &   $19.837\pm0.065$   &  $19.98\pm0.157$   &   $17.64\pm-999999488.000$   &   $15.19\pm-999999488.000$   \\
SDWISE & J0115-0253 &   18.94279 &   -2.88673 &  5.07   &   $19.74\pm0.034$  &  $19.63\pm0.033$  &  $19.47\pm0.042$   & $19.49\pm0.052$    &   $19.036\pm0.030$   &  $19.11\pm0.070$   &   $16.91\pm-999999488.000$   &   $14.98\pm-999999488.000$   \\
SDWISE & J0116+0538 &   19.05958 &    5.63825 &  5.33   &   $19.12\pm0.049$  &  $18.91\pm0.054$  &  $18.95\pm0.075$   & $18.92\pm0.071$    &   $19.023\pm0.031$   &  $18.92\pm0.061$   &   $17.38\pm0.361$   &   $15.50\pm-999999488.000$   \\
PSO & J021.4213-25.8822 &   21.42134 &  -25.88229 &  5.79   &   $-999999500.00\pm-999999500.000$  &  $-999999500.00\pm-999999500.000$  &  $-999999500.00\pm-999999500.000$   & $-999999500.00\pm-999999500.000$    &   $18.892\pm0.025$   &  $18.88\pm0.053$   &   $17.68\pm0.422$   &   $15.00\pm-999999488.000$   \\
SDSS & J0129-0028 &   22.28100 &   -0.47931 &  5.01   &   $21.07\pm0.259$  &  $21.65\pm0.114$  &  $21.45\pm0.177$   & $21.11\pm0.170$    &   $20.803\pm0.135$   &  $-999999484.72\pm-999999488.000$   &   $-999999482.85\pm-999999488.000$   &   $-999999481.34\pm-999999488.000$   \\
SDSS & J0129-0035 &   22.49379 &   -0.59436 &  5.78   &   $22.02\pm0.618$  &  $21.72\pm0.122$  &  $21.56\pm0.196$   & $21.62\pm0.273$    &   $-999999485.331\pm-999999488.000$   &  $-999999484.72\pm-999999488.000$   &   $-999999482.85\pm-999999488.000$   &   $-999999481.34\pm-999999488.000$   \\
SDWISE & J0131-0321 &   22.86392 &   -3.35005 &  5.18   &   $17.84\pm0.015$  &  $17.68\pm0.008$  &  $17.36\pm0.012$   & $17.36\pm0.018$    &   $17.211\pm0.007$   &  $17.17\pm0.014$   &   $16.59\pm0.174$   &   $15.15\pm-999999488.000$   \\
PSO & J023.0071-02.2675 &   23.00710 &   -2.26753 &  5.90   &   $20.20\pm0.161$  &  $20.16\pm0.156$  &  $19.89\pm0.211$   & $19.70\pm0.166$    &   $19.237\pm0.034$   &  $18.72\pm0.048$   &   $17.16\pm-999999488.000$   &   $15.39\pm-999999488.000$   \\
SDSS & J0133+0106 &   23.36183 &    1.11047 &  5.30   &   $20.28\pm0.115$  &  $20.67\pm0.054$  &  $20.09\pm0.059$   & $20.11\pm0.062$    &   $19.519\pm0.047$   &  $19.15\pm0.076$   &   $17.59\pm-999999488.000$   &   $15.49\pm-999999488.000$   \\
CFHQS & J0136+0226 &   24.01321 &    2.43492 &  6.21   &   $22.41\pm0.650$  &  $-999999488.00\pm-999999488.000$  &  $22.22\pm0.933$   & $-999999488.00\pm-999999488.000$    &   $-999999485.331\pm-999999488.000$   &  $-999999484.72\pm-999999488.000$   &   $-999999482.85\pm-999999488.000$   &   $-999999481.34\pm-999999488.000$   \\
PSO & J025.2376-11.6831 &   25.23764 &  -11.68319 &  5.85   &   $-999999500.00\pm-999999500.000$  &  $-999999500.00\pm-999999500.000$  &  $-999999500.00\pm-999999500.000$   & $-999999500.00\pm-999999500.000$    &   $19.434\pm0.041$   &  $19.18\pm0.071$   &   $17.41\pm0.427$   &   $15.14\pm-999999488.000$   \\
ATLAS & J025.6821-33.4627 &   25.68220 &  -33.46263 &  6.34   &   $19.14\pm0.015$  &  $19.11\pm0.012$  &  $18.95\pm0.024$   & $18.75\pm0.029$    &   $18.799\pm0.022$   &  $18.64\pm0.040$   &   $17.73\pm0.434$   &   $15.38\pm-999999488.000$   \\
VDES & J0143-5545 &   25.79267 &  -55.75297 &  6.25   &   $-999999500.00\pm-999999500.000$  &  $20.60\pm0.083$  &  $-999999500.00\pm-999999500.000$   & $20.10\pm0.140$    &   $19.739\pm0.040$   &  $19.21\pm0.054$   &   $17.42\pm-999999488.000$   &   $15.84\pm-999999488.000$   \\
ULAS & J0148+0600 &   27.15681 &    6.00557 &  5.98   &   $19.52\pm0.063$  &  $19.11\pm0.022$  &  $19.13\pm0.071$   & $19.02\pm0.076$    &   $18.776\pm0.024$   &  $18.64\pm0.046$   &   $17.32\pm0.296$   &   $15.62\pm0.392$   \\
SDWISE & J0155+0415 &   28.88867 &    4.25187 &  5.37   &   $19.63\pm0.070$  &  $19.21\pm0.063$  &  $19.01\pm0.057$   & $18.91\pm0.064$    &   $18.799\pm0.025$   &  $18.55\pm0.043$   &   $17.45\pm-999999488.000$   &   $15.03\pm-999999488.000$   \\
PSO & J029.5172-29.0886 &   29.51726 &  -29.08868 &  5.99   &   $19.21\pm0.019$  &  $19.14\pm0.014$  &  $19.13\pm0.027$   & $18.91\pm0.029$    &   $18.918\pm0.026$   &  $18.78\pm0.048$   &   $17.16\pm0.289$   &   $15.17\pm-999999488.000$   \\
ATLAS & J029.9915-36.5658 &   29.99155 &  -36.56572 &  6.02   &   $-999999500.00\pm-999999500.000$  &  $19.48\pm0.028$  &  $-999999500.00\pm-999999500.000$   & $19.23\pm0.056$    &   $19.277\pm0.032$   &  $19.19\pm0.065$   &   $17.77\pm-999999488.000$   &   $15.42\pm-999999488.000$   \\
SHELLQs & J0202-0251 &   30.74254 &   -2.86489 &  6.03   &   $-999999500.00\pm-999999500.000$  &  $22.61\pm0.645$  &  $21.48\pm0.325$   & $21.20\pm0.331$    &   $-999999485.331\pm-999999488.000$   &  $-999999484.72\pm-999999488.000$   &   $-999999482.85\pm-999999488.000$   &   $-999999481.34\pm-999999488.000$   \\
ULAS & J0203+0012 &   30.88492 &    0.20813 &  5.72   &   $20.46\pm0.116$  &  $19.76\pm0.019$  &  $19.25\pm0.044$   & $19.12\pm0.021$    &   $19.190\pm0.034$   &  $19.16\pm0.072$   &   $17.47\pm0.400$   &   $15.72\pm-999999488.000$   \\
SDSS & J0205-0955 &   31.44429 &   -9.92325 &  5.37   &   $-999999500.00\pm-999999500.000$  &  $23.73\pm1.853$  &  $-999999500.00\pm-999999500.000$   & $22.50\pm1.324$    &   $-999999485.331\pm-999999488.000$   &  $-999999484.72\pm-999999488.000$   &   $-999999482.85\pm-999999488.000$   &   $-999999481.34\pm-999999488.000$   \\
SHELLQs & J0206-0255 &   31.54667 &   -2.92717 &  6.03   &   $-999999500.00\pm-999999500.000$  &  $21.12\pm0.104$  &  $21.16\pm0.212$   & $20.85\pm0.144$    &   $-999999485.331\pm-999999488.000$   &  $-999999484.72\pm-999999488.000$   &   $-999999482.85\pm-999999488.000$   &   $-999999481.34\pm-999999488.000$   \\
SDSS & J0208-0112 &   32.01796 &   -1.20953 &  5.23   &   $21.10\pm0.217$  &  $20.91\pm0.080$  &  $21.11\pm0.129$   & $20.88\pm0.149$    &   $20.676\pm0.120$   &  $-999999484.72\pm-999999488.000$   &   $18.00\pm-999999488.000$   &   $15.87\pm-999999488.000$   \\
CFHQS & J0210-0456 &   32.55496 &   -4.93914 &  6.43   &   $-999999500.00\pm-999999500.000$  &  $22.15\pm0.118$  &  $22.61\pm0.725$   & $21.11\pm0.279$    &   $-999999485.331\pm-999999488.000$   &  $-999999484.72\pm-999999488.000$   &   $-999999482.85\pm-999999488.000$   &   $-999999481.34\pm-999999488.000$   \\
SDSS & J0210+0003 &   32.73612 &    0.05131 &  5.05   &   $21.39\pm0.285$  &  $21.06\pm0.048$  &  $20.74\pm0.161$   & $20.03\pm0.038$    &   $19.584\pm0.046$   &  $19.36\pm0.083$   &   $17.68\pm0.374$   &   $15.77\pm0.542$   \\
SHELLQs & J0211-0203 &   32.93554 &   -2.05108 &  6.37   &   $-999999500.00\pm-999999500.000$  &  $23.25\pm1.113$  &  $21.48\pm0.352$   & $22.51\pm0.947$    &   $20.410\pm0.092$   &  $-999999484.72\pm-999999488.000$   &   $-999999482.85\pm-999999488.000$   &   $-999999481.34\pm-999999488.000$   \\
SHELLQs & J0213-0626 &   33.32058 &   -6.43756 &  6.72   &   $-999999500.00\pm-999999500.000$  &  $22.06\pm0.320$  &  $24.48\pm4.155$   & $21.46\pm0.345$    &   $-999999485.331\pm-999999488.000$   &  $-999999484.72\pm-999999488.000$   &   $-999999482.85\pm-999999488.000$   &   $-999999481.34\pm-999999488.000$   \\
MMT & J0215-0529 &   33.84696 &   -5.49606 &  5.13   &   $20.71\pm0.009$  &  $20.74\pm0.023$  &  $20.08\pm0.102$   & $20.38\pm0.186$    &   $20.513\pm0.101$   &  $20.16\pm0.164$   &   $-999999482.85\pm-999999488.000$   &   $-999999481.34\pm-999999488.000$   \\
SDWISE & J0216+2304 &   34.10067 &   23.06930 &  5.26   &   $-999999500.00\pm-999999500.000$  &  $19.33\pm0.085$  &  $-999999500.00\pm-999999500.000$   & $-999999500.00\pm-999999500.000$    &   $19.127\pm0.033$   &  $18.99\pm0.065$   &   $16.83\pm-999999488.000$   &   $15.29\pm-999999488.000$   \\
CFHQS & J0216-0455 &   34.11588 &   -4.92614 &  6.01   &   $25.82\pm0.338$  &  $27.11\pm0.828$  &  $-999999500.00\pm-999999500.000$   & $-999999500.00\pm-999999500.000$    &   $-999999485.331\pm-999999488.000$   &  $-999999484.72\pm-999999488.000$   &   $-999999482.85\pm-999999488.000$   &   $-999999481.34\pm-999999488.000$   \\
SHELLQs & J0217-0208 &   34.33996 &   -2.14794 &  6.20   &   $-999999500.00\pm-999999500.000$  &  $-999999488.00\pm-999999488.000$  &  $22.47\pm1.298$   & $22.37\pm1.200$    &   $-999999485.331\pm-999999488.000$   &  $-999999484.72\pm-999999488.000$   &   $17.60\pm-999999488.000$   &   $15.96\pm-999999488.000$   \\
SDSS & J0218-0027 &   34.58783 &   -0.46269 &  5.11   &   $21.63\pm0.354$  &  $20.96\pm0.058$  &  $21.12\pm0.229$   & $20.51\pm0.074$    &   $20.209\pm0.082$   &  $20.07\pm0.155$   &   $17.36\pm-999999488.000$   &   $15.38\pm-999999488.000$   \\
SHELLQs & J0220-0432 &   35.12383 &   -4.53444 &  5.90   &   $23.55\pm0.050$  &  $23.39\pm0.064$  &  $23.36\pm0.098$   & $22.97\pm0.105$    &   $-999999485.331\pm-999999488.000$   &  $-999999484.72\pm-999999488.000$   &   $17.95\pm-999999488.000$   &   $15.81\pm-999999488.000$   \\
MMT & J0221-0342A &   35.30133 &   -3.70878 &  5.02   &   $21.85\pm0.216$  &  $21.62\pm0.030$  &  $20.82\pm0.138$   & $21.06\pm0.025$    &   $21.054\pm0.165$   &  $-999999484.72\pm-999999488.000$   &   $-999999482.85\pm-999999488.000$   &   $-999999481.34\pm-999999488.000$   \\
SDSS & J0221-0342B &   35.30254 &   -3.71450 &  5.02   &   $19.41\pm0.024$  &  $19.48\pm0.005$  &  $19.13\pm0.030$   & $19.10\pm0.004$    &   $18.979\pm0.028$   &  $18.98\pm0.061$   &   $17.42\pm-999999488.000$   &   $15.59\pm-999999488.000$   \\
CFHQS & J0221-0802 &   35.34463 &   -8.04764 &  6.16   &   $-999999500.00\pm-999999500.000$  &  $22.10\pm0.239$  &  $-999999500.00\pm-999999500.000$   & $21.04\pm0.246$    &   $20.717\pm0.118$   &  $20.33\pm0.187$   &   $-999999482.85\pm-999999488.000$   &   $-999999481.34\pm-999999488.000$   \\
VDES & J0224-4711 &   36.11057 &  -47.19149 &  6.50   &   $-999999500.00\pm-999999500.000$  &  $19.73\pm0.048$  &  $19.45\pm0.066$   & $18.94\pm0.049$    &   $18.783\pm0.019$   &  $18.70\pm0.036$   &   $17.88\pm-999999488.000$   &   $15.78\pm-999999488.000$   \\
PSO & J036.5078+03.0498 &   36.50781 &    3.04984 &  6.54   &   $19.45\pm0.057$  &  $19.40\pm0.094$  &  $19.30\pm0.088$   & $19.28\pm0.087$    &   $19.326\pm0.038$   &  $19.46\pm0.093$   &   $17.18\pm-999999488.000$   &   $15.60\pm-999999488.000$   \\
CFHQS & J0227-0605 &   36.93037 &   -6.09172 &  6.20   &   $22.09\pm0.211$  &  $21.93\pm0.183$  &  $21.94\pm0.268$   & $21.49\pm0.226$    &   $-999999485.331\pm-999999488.000$   &  $-999999484.72\pm-999999488.000$   &   $-999999482.85\pm-999999488.000$   &   $-999999481.34\pm-999999488.000$   \\
SDSS & J0230+0046 &   37.50946 &    0.77967 &  5.41   &   $21.60\pm0.100$  &  $21.45\pm0.075$  &  $21.34\pm0.109$   & $21.46\pm0.153$    &   $-999999485.331\pm-999999488.000$   &  $-999999484.72\pm-999999488.000$   &   $-999999482.85\pm-999999488.000$   &   $-999999481.34\pm-999999488.000$   \\
SDSS & J0231-0728 &   37.90683 &   -7.48178 &  5.37   &   $-999999500.00\pm-999999500.000$  &  $19.21\pm0.029$  &  $-999999500.00\pm-999999500.000$   & $18.77\pm0.054$    &   $18.655\pm0.020$   &  $18.29\pm0.032$   &   $17.25\pm-999999488.000$   &   $15.84\pm-999999488.000$   \\
PSO & J037.9706-28.8389 &   37.97066 &  -28.83891 &  6.00   &   $20.99\pm0.128$  &  $21.09\pm0.152$  &  $20.96\pm0.199$   & $20.51\pm0.186$    &   $20.313\pm0.079$   &  $20.03\pm0.135$   &   $17.09\pm-999999488.000$   &   $15.33\pm-999999488.000$   \\
SHELLQs & J0235-0532 &   38.92675 &   -5.54489 &  6.09   &   $-999999500.00\pm-999999500.000$  &  $-999999488.00\pm-999999488.000$  &  $23.66\pm2.040$   & $22.56\pm1.086$    &   $-999999485.331\pm-999999488.000$   &  $-999999484.72\pm-999999488.000$   &   $-999999482.85\pm-999999488.000$   &   $-999999481.34\pm-999999488.000$   \\
SDSS & J0239-0045 &   39.87600 &   -0.75150 &  5.82   &   $21.28\pm0.436$  &  $22.14\pm0.241$  &  $21.58\pm0.278$   & $21.63\pm0.332$    &   $-999999485.331\pm-999999488.000$   &  $-999999484.72\pm-999999488.000$   &   $-999999482.85\pm-999999488.000$   &   $-999999481.34\pm-999999488.000$   \\
PSO & J040.0159+17.5458 &   40.01591 &   17.54581 &  5.68   &   $-999999500.00\pm-999999500.000$  &  $20.93\pm0.272$  &  $-999999500.00\pm-999999500.000$   & $-999999500.00\pm-999999500.000$    &   $20.214\pm0.083$   &  $-999999484.72\pm-999999488.000$   &   $-999999482.85\pm-999999488.000$   &   $-999999481.34\pm-999999488.000$   \\
SDWISE & J0241+0435 &   40.47050 &    4.59818 &  5.22   &   $19.85\pm0.090$  &  $19.52\pm0.087$  &  $19.02\pm0.108$   & $19.16\pm0.108$    &   $18.871\pm0.026$   &  $18.81\pm0.055$   &   $17.44\pm0.398$   &   $15.08\pm-999999488.000$   \\
VDES & J0244-5008 &   41.00000 &  -50.13333 &  6.74   &   $-999999500.00\pm-999999500.000$  &  $-999999488.00\pm-999999488.000$  &  $-999999488.00\pm-999999488.000$   & $-999999488.00\pm-999999488.000$    &   $-999999485.331\pm-999999488.000$   &  $-999999484.72\pm-999999488.000$   &   $-999999482.85\pm-999999488.000$   &   $-999999481.34\pm-999999488.000$   \\
PSO & J042.6690-02.9174 &   42.66909 &   -2.91745 &  5.89   &   $-999999500.00\pm-999999500.000$  &  $20.20\pm0.076$  &  $-999999500.00\pm-999999500.000$   & $20.38\pm0.204$    &   $20.550\pm0.111$   &  $-999999484.72\pm-999999488.000$   &   $16.69\pm-999999488.000$   &   $15.09\pm-999999488.000$   \\
SDWISE & J0251+0333 &   42.83887 &    3.55484 &  5.00   &   $-999999500.00\pm-999999500.000$  &  $19.13\pm0.066$  &  $-999999500.00\pm-999999500.000$   & $-999999500.00\pm-999999500.000$    &   $18.368\pm0.017$   &  $18.28\pm0.032$   &   $16.96\pm0.239$   &   $15.86\pm-999999488.000$   \\
PSO & J045.1840-22.5408 &   45.18408 &  -22.54088 &  5.68   &   $-999999500.00\pm-999999500.000$  &  $19.72\pm0.031$  &  $-999999500.00\pm-999999500.000$   & $19.10\pm0.045$    &   $18.864\pm0.025$   &  $19.06\pm0.060$   &   $17.85\pm0.391$   &   $15.43\pm-999999488.000$   \\
SDSS & J0301+0020 &   45.32087 &    0.34056 &  5.50   &   $-999999500.00\pm-999999488.000$  &  $23.16\pm0.797$  &  $23.78\pm2.384$   & $22.72\pm1.089$    &   $-999999485.331\pm-999999488.000$   &  $-999999484.72\pm-999999488.000$   &   $-999999482.85\pm-999999488.000$   &   $-999999481.34\pm-999999488.000$   \\
SDSS & J0303-0019 &   45.88083 &   -0.32025 &  6.08   &   $21.70\pm0.383$  &  $21.29\pm0.139$  &  $21.26\pm0.182$   & $20.75\pm0.268$    &   $-999999485.331\pm-999999488.000$   &  $19.89\pm0.134$   &   $-999999482.85\pm-999999488.000$   &   $-999999481.34\pm-999999488.000$   \\
VIK & J0305-3150 &   46.32048 &  -31.84886 &  6.61   &   $20.89\pm0.082$  &  $20.60\pm0.046$  &  $20.68\pm0.106$   & $20.27\pm0.085$    &   $20.140\pm0.064$   &  $20.17\pm0.139$   &   $17.99\pm-999999488.000$   &   $15.64\pm-999999488.000$   \\
SDWISE & J0306+1853 &   46.67712 &   18.88774 &  5.36   &   $-999999500.00\pm-999999500.000$  &  $17.11\pm0.007$  &  $-999999500.00\pm-999999500.000$   & $-999999500.00\pm-999999500.000$    &   $16.942\pm0.006$   &  $16.74\pm0.010$   &   $15.65\pm0.095$   &   $14.25\pm0.156$   \\
CFHQS & J0316-1340 &   49.20779 &  -13.67564 &  5.99   &   $-999999500.00\pm-999999500.000$  &  $22.30\pm0.416$  &  $-999999500.00\pm-999999500.000$   & $22.26\pm1.357$    &   $-999999485.331\pm-999999488.000$   &  $-999999484.72\pm-999999488.000$   &   $-999999482.85\pm-999999488.000$   &   $-999999481.34\pm-999999488.000$   \\
PSO & J049.2934-26.5543 &   49.29343 &  -26.55436 &  5.94   &   $-999999500.00\pm-999999500.000$  &  $-999999500.00\pm-999999500.000$  &  $-999999500.00\pm-999999500.000$   & $-999999500.00\pm-999999500.000$    &   $20.597\pm0.098$   &  $-999999484.72\pm-999999488.000$   &   $18.08\pm-999999488.000$   &   $16.25\pm-999999488.000$   \\
SDSS & J0321+0029 &   50.47946 &    0.49483 &  5.04   &   $22.11\pm0.577$  &  $21.52\pm0.111$  &  $20.75\pm0.116$   & $20.89\pm0.134$    &   $-999999485.331\pm-999999488.000$   &  $-999999484.72\pm-999999488.000$   &   $16.69\pm0.242$   &   $15.61\pm-999999488.000$   \\
VDES & J0323-4701 &   50.91808 &  -47.02226 &  6.25   &   $-999999500.00\pm-999999500.000$  &  $20.82\pm0.141$  &  $20.75\pm0.184$   & $20.35\pm0.184$    &   $20.572\pm0.076$   &  $20.44\pm0.146$   &   $17.86\pm-999999488.000$   &   $15.67\pm-999999488.000$   \\
VIK & J0328-3253 &   52.14794 &  -32.88968 &  5.86   &   $20.06\pm0.056$  &  $19.91\pm0.045$  &  $19.82\pm0.069$   & $19.69\pm0.063$    &   $19.648\pm0.041$   &  $19.40\pm0.071$   &   $18.11\pm-999999488.000$   &   $15.94\pm-999999488.000$   \\
VDES & J0330-4025 &   52.61633 &  -40.42122 &  6.25   &   $-999999500.00\pm-999999500.000$  &  $20.45\pm0.100$  &  $-999999500.00\pm-999999500.000$   & $20.04\pm0.163$    &   $20.165\pm0.060$   &  $-999999484.72\pm-999999488.000$   &   $18.05\pm0.370$   &   $16.13\pm-999999488.000$   \\
PSO & J053.9605-15.7956 &   53.96052 &  -15.79569 &  5.87   &   $-999999500.00\pm-999999500.000$  &  $-999999500.00\pm-999999500.000$  &  $-999999500.00\pm-999999500.000$   & $-999999500.00\pm-999999500.000$    &   $20.414\pm0.088$   &  $19.90\pm0.120$   &   $-999999482.85\pm-999999488.000$   &   $-999999481.34\pm-999999488.000$   \\
SDSS & J0338+0021 &   54.62212 &    0.36564 &  5.03   &   $19.76\pm0.059$  &  $19.68\pm0.009$  &  $19.49\pm0.040$   & $19.35\pm0.049$    &   $19.450\pm0.043$   &  $19.46\pm0.094$   &   $17.21\pm-999999488.000$   &   $15.56\pm-999999488.000$   \\
SDSS & J0341-0048 &   55.42437 &   -0.80354 &  5.68   &   $20.45\pm0.147$  &  $20.11\pm0.047$  &  $20.14\pm0.070$   & $20.14\pm0.095$    &   $19.942\pm0.064$   &  $19.82\pm0.125$   &   $-999999482.85\pm-999999488.000$   &   $-999999481.34\pm-999999488.000$   \\
PSO & J056.7168-16.4769 &   56.71685 &  -16.47691 &  5.99   &   $-999999500.00\pm-999999500.000$  &  $-999999500.00\pm-999999500.000$  &  $-999999500.00\pm-999999500.000$   & $-999999500.00\pm-999999500.000$    &   $19.308\pm0.035$   &  $18.99\pm0.057$   &   $17.78\pm-999999488.000$   &   $15.68\pm-999999488.000$   \\
SDSS & J0349+0034 &   57.49750 &    0.56764 &  5.20   &   $21.95\pm0.433$  &  $21.36\pm0.115$  &  $21.54\pm0.253$   & $20.50\pm0.100$    &   $20.793\pm0.145$   &  $-999999484.72\pm-999999488.000$   &   $-999999482.85\pm-999999488.000$   &   $-999999481.34\pm-999999488.000$   \\
SDSS & J0353+0104 &   58.45721 &    1.06796 &  6.07   &   $20.70\pm0.156$  &  $20.25\pm0.052$  &  $19.99\pm0.071$   & $19.82\pm0.070$    &   $19.533\pm0.047$   &  $19.59\pm0.105$   &   $17.07\pm-999999488.000$   &   $15.01\pm-999999488.000$   \\
PSO & J060.5529+24.8567 &   60.55289 &   24.85679 &  6.18   &   $20.28\pm0.122$  &  $19.95\pm0.092$  &  $20.08\pm0.157$   & $19.53\pm0.056$    &   $19.182\pm0.036$   &  $19.16\pm0.076$   &   $17.17\pm-999999488.000$   &   $15.50\pm-999999488.000$   \\
VDES & J0408-5632 &   62.08013 &  -56.54134 &  6.03   &   $-999999500.00\pm-999999500.000$  &  $19.85\pm0.046$  &  $-999999500.00\pm-999999500.000$   & $19.68\pm0.097$    &   $20.044\pm0.042$   &  $19.85\pm0.075$   &   $17.90\pm-999999488.000$   &   $16.14\pm-999999488.000$   \\
VDES & J0410-4414 &   62.51346 &  -44.24464 &  6.21   &   $-999999500.00\pm-999999500.000$  &  $20.69\pm0.115$  &  $-999999500.00\pm-999999500.000$   & $20.17\pm0.188$    &   $20.064\pm0.050$   &  $20.21\pm0.120$   &   $18.12\pm-999999488.000$   &   $15.70\pm-999999488.000$   \\
VDES & J0420-4453 &   65.04725 &  -44.88994 &  6.07   &   $-999999500.00\pm-999999500.000$  &  $20.55\pm0.090$  &  $-999999500.00\pm-999999500.000$   & $19.99\pm0.129$    &   $19.994\pm0.045$   &  $19.77\pm0.080$   &   $17.58\pm-999999488.000$   &   $15.72\pm-999999488.000$   \\
PSO & J065.4085-26.9543 &   65.40854 &  -26.95434 &  6.19   &   $-999999500.00\pm-999999500.000$  &  $19.37\pm0.031$  &  $-999999500.00\pm-999999500.000$   & $19.22\pm0.059$    &   $18.976\pm0.026$   &  $19.14\pm0.062$   &   $17.91\pm0.530$   &   $15.27\pm-999999488.000$   \\
PSO & J065.5041-19.4579 &   65.50415 &  -19.45797 &  6.12   &   $-999999500.00\pm-999999500.000$  &  $19.85\pm0.036$  &  $-999999500.00\pm-999999500.000$   & $19.17\pm0.078$    &   $18.691\pm0.021$   &  $18.33\pm0.032$   &   $17.22\pm0.311$   &   $15.55\pm0.434$   \\
PSO & J071.0322-04.5591 &   71.03221 &   -4.55919 &  5.89   &   $20.14\pm0.103$  &  $19.89\pm0.121$  &  $-999999500.00\pm-999999500.000$   & $19.72\pm0.208$    &   $20.023\pm0.062$   &  $20.00\pm0.133$   &   $-999999482.85\pm-999999488.000$   &   $-999999481.34\pm-999999488.000$   \\
PSO & J071.4507-02.3332 &   71.45075 &   -2.33329 &  5.69   &   $-999999500.00\pm-999999500.000$  &  $18.99\pm0.028$  &  $-999999500.00\pm-999999500.000$   & $18.91\pm0.070$    &   $18.912\pm0.025$   &  $18.96\pm0.056$   &   $16.83\pm-999999488.000$   &   $15.33\pm0.481$   \\
VDES & J0454-4448 &   73.50745 &  -44.80864 &  6.06   &   $-999999500.00\pm-999999500.000$  &  $20.20\pm0.054$  &  $-999999500.00\pm-999999500.000$   & $20.08\pm0.137$    &   $19.843\pm0.040$   &  $19.82\pm0.082$   &   $17.72\pm-999999488.000$   &   $15.31\pm-999999488.000$   \\
PSO & J075.9356-07.5061 &   75.93566 &   -7.50613 &  5.88   &   $-999999500.00\pm-999999500.000$  &  $20.52\pm0.186$  &  $-999999500.00\pm-999999500.000$   & $20.47\pm0.329$    &   $19.836\pm0.058$   &  $19.78\pm0.113$   &   $17.00\pm0.320$   &   $14.81\pm-999999488.000$   \\
PSO & J089.9394-15.5833 &   89.93944 &  -15.58339 &  6.05   &   $-999999500.00\pm-999999500.000$  &  $19.09\pm0.044$  &  $-999999500.00\pm-999999500.000$   & $18.43\pm0.052$    &   $18.184\pm0.014$   &  $17.80\pm0.020$   &   $17.22\pm0.279$   &   $15.69\pm-999999488.000$   \\
PSO & J108.4429+08.9257 &  108.44294 &    8.92574 &  5.92   &   $-999999500.00\pm-999999500.000$  &  $19.07\pm0.062$  &  $-999999500.00\pm-999999500.000$   & $-999999500.00\pm-999999500.000$    &   $18.687\pm0.023$   &  $18.40\pm0.039$   &   $17.68\pm0.539$   &   $14.96\pm-999999488.000$   \\
SDSS & J0731+4459 &  112.76303 &   44.99707 &  5.01   &   $-999999500.00\pm-999999500.000$  &  $18.87\pm0.043$  &  $-999999500.00\pm-999999500.000$   & $-999999500.00\pm-999999500.000$    &   $18.587\pm0.020$   &  $18.67\pm0.044$   &   $16.94\pm0.247$   &   $14.97\pm-999999488.000$   \\
SDSS & J0741+2520 &  115.47800 &   25.34157 &  5.19   &   $18.46\pm0.020$  &  $18.30\pm0.014$  &  $17.91\pm0.033$   & $17.71\pm0.028$    &   $17.397\pm0.009$   &  $17.15\pm0.014$   &   $16.74\pm0.241$   &   $15.03\pm0.344$   \\
SDWISE & J0747+1153 &  116.95492 &   11.89791 &  5.26   &   $-999999500.00\pm-999999500.000$  &  $18.04\pm0.024$  &  $-999999500.00\pm-999999500.000$   & $-999999500.00\pm-999999500.000$    &   $17.263\pm0.008$   &  $17.06\pm0.013$   &   $16.51\pm0.219$   &   $15.45\pm0.512$   \\
SDSS & J0756+4104 &  119.07558 &   41.06906 &  5.06   &   $-999999500.00\pm-999999500.000$  &  $19.80\pm0.085$  &  $-999999500.00\pm-999999500.000$   & $-999999500.00\pm-999999500.000$    &   $19.505\pm0.045$   &  $19.42\pm0.087$   &   $17.00\pm-999999488.000$   &   $15.29\pm-999999488.000$   \\
SDSS & J0810+5105 &  122.72631 &   51.09447 &  5.82   &   $-999999500.00\pm-999999500.000$  &  $19.89\pm0.093$  &  $-999999500.00\pm-999999500.000$   & $-999999500.00\pm-999999500.000$    &   $19.566\pm0.044$   &  $19.44\pm0.085$   &   $17.51\pm-999999488.000$   &   $15.65\pm-999999488.000$   \\
SDWISE & J0812+0440 &  123.20342 &    4.68237 &  5.29   &   $-999999500.00\pm-999999500.000$  &  $19.64\pm0.089$  &  $-999999500.00\pm-999999500.000$   & $-999999500.00\pm-999999500.000$    &   $19.002\pm0.030$   &  $18.69\pm0.051$   &   $17.58\pm-999999488.000$   &   $15.34\pm-999999488.000$   \\
SDSS & J0818+1722 &  124.61418 &   17.38111 &  6.02   &   $-999999500.00\pm-999999500.000$  &  $19.09\pm0.059$  &  $-999999500.00\pm-999999500.000$   & $-999999500.00\pm-999999500.000$    &   $18.281\pm0.017$   &  $18.16\pm0.032$   &   $17.07\pm0.328$   &   $14.90\pm-999999488.000$   \\
SDSS & J0824+1302 &  126.22506 &   13.03805 &  5.15   &   $-999999500.00\pm-999999500.000$  &  $19.34\pm0.066$  &  $-999999500.00\pm-999999500.000$   & $-999999500.00\pm-999999500.000$    &   $19.190\pm0.037$   &  $18.90\pm0.062$   &   $17.09\pm-999999488.000$   &   $14.82\pm-999999488.000$   \\
ULAS & J0828+2633 &  127.05586 &   26.56541 &  6.05   &   $20.60\pm0.062$  &  $20.53\pm0.071$  &  $20.36\pm0.336$   & $20.08\pm0.220$    &   $19.383\pm0.042$   &  $19.38\pm0.089$   &   $-999999482.85\pm-999999488.000$   &   $-999999481.34\pm-999999488.000$   \\
PSO & J127.2817+03.0657 &  127.28174 &    3.06570 &  5.85   &   $21.04\pm0.198$  &  $20.97\pm0.283$  &  $20.20\pm0.191$   & $20.10\pm0.185$    &   $20.094\pm0.071$   &  $19.84\pm0.128$   &   $17.59\pm-999999488.000$   &   $15.16\pm-999999488.000$   \\
SUVAW & J0829+2506 &  127.38792 &   25.11267 &  5.35   &   $19.83\pm0.064$  &  $19.63\pm0.052$  &  $19.50\pm0.132$   & $19.37\pm0.115$    &   $19.376\pm0.042$   &  $19.14\pm0.076$   &   $16.77\pm-999999488.000$   &   $14.90\pm-999999488.000$   \\
SDSS & J0833+2726 &  128.32358 &   27.44139 &  5.02   &   $20.63\pm0.210$  &  $20.32\pm0.194$  &  $20.16\pm0.240$   & $19.62\pm0.145$    &   $19.778\pm0.058$   &  $19.92\pm0.147$   &   $17.08\pm-999999488.000$   &   $15.46\pm-999999488.000$   \\
SHELLQs & J0834+0211 &  128.50367 &    2.19636 &  6.15   &   $22.33\pm0.287$  &  $23.31\pm0.955$  &  $23.09\pm1.069$   & $21.91\pm0.909$    &   $-999999485.331\pm-999999488.000$   &  $-999999484.72\pm-999999488.000$   &   $-999999482.85\pm-999999488.000$   &   $-999999481.34\pm-999999488.000$   \\
SDSS & J0835+3217 &  128.85733 &   32.29794 &  5.89   &   $-999999500.00\pm-999999500.000$  &  $21.09\pm0.304$  &  $-999999500.00\pm-999999500.000$   & $-999999500.00\pm-999999500.000$    &   $20.690\pm0.126$   &  $20.13\pm0.171$   &   $17.64\pm-999999488.000$   &   $15.35\pm-999999488.000$   \\
SDSS & J0835+0537 &  128.97651 &    5.63140 &  5.07   &   $19.89\pm0.064$  &  $19.58\pm0.045$  &  $19.30\pm0.068$   & $19.12\pm0.058$    &   $19.074\pm0.030$   &  $19.02\pm0.064$   &   $-999999482.85\pm-999999488.000$   &   $-999999481.34\pm-999999488.000$   \\
SDSS & J0836+0054 &  129.18277 &    0.91479 &  5.81   &   $18.88\pm0.004$  &  $18.65\pm0.003$  &  $18.36\pm0.009$   & $18.11\pm0.009$    &   $17.937\pm0.012$   &  $17.72\pm0.021$   &   $17.72\pm0.533$   &   $15.67\pm-999999488.000$   \\
VIK & J0839+0015 &  129.98065 &    0.26506 &  5.84   &   $21.10\pm0.069$  &  $20.82\pm0.063$  &  $20.68\pm0.111$   & $20.43\pm0.109$    &   $20.276\pm0.087$   &  $20.20\pm0.170$   &   $17.61\pm0.498$   &   $15.62\pm-999999488.000$   \\
SDSS & J0840+5624 &  130.14626 &   56.40562 &  5.84   &   $-999999500.00\pm-999999500.000$  &  $19.47\pm0.074$  &  $-999999500.00\pm-999999500.000$   & $-999999500.00\pm-999999500.000$    &   $19.486\pm0.042$   &  $19.47\pm0.085$   &   $17.51\pm-999999488.000$   &   $15.13\pm-999999488.000$   \\
SDSS & J0841+2905 &  130.33132 &   29.08460 &  5.98   &   $20.35\pm0.092$  &  $19.99\pm0.037$  &  $20.21\pm0.155$   & $19.80\pm0.044$    &   $19.856\pm0.065$   &  $19.68\pm0.120$   &   $17.44\pm-999999488.000$   &   $15.73\pm-999999488.000$   \\
SDSS & J0842+1218 &  130.62264 &   12.31405 &  6.08   &   $-999999500.00\pm-999999500.000$  &  $19.70\pm0.120$  &  $-999999500.00\pm-999999500.000$   & $19.38\pm0.110$    &   $19.004\pm0.029$   &  $19.03\pm0.067$   &   $17.50\pm0.428$   &   $15.68\pm-999999488.000$   \\
SHELLQs & J0844-0132 &  131.03588 &   -1.53792 &  6.18   &   $23.96\pm0.804$  &  $23.34\pm0.551$  &  $24.05\pm2.587$   & $-999999500.00\pm-999999500.000$    &   $-999999485.331\pm-999999488.000$   &  $-999999484.72\pm-999999488.000$   &   $-999999482.85\pm-999999488.000$   &   $-999999481.34\pm-999999488.000$   \\
SHELLQs & J0844-0052 &  131.13167 &   -0.88183 &  6.25   &   $23.91\pm1.142$  &  $23.54\pm0.886$  &  $23.39\pm2.141$   & $23.18\pm1.478$    &   $-999999485.331\pm-999999488.000$   &  $-999999484.72\pm-999999488.000$   &   $-999999482.85\pm-999999488.000$   &   $-999999481.34\pm-999999488.000$   \\
SDSS & J0846+0800 &  131.61600 &    8.01437 &  5.00   &   $19.72\pm0.051$  &  $19.57\pm0.055$  &  $19.36\pm0.062$   & $19.38\pm0.090$    &   $19.573\pm0.047$   &  $19.67\pm0.110$   &   $17.24\pm-999999488.000$   &   $15.40\pm-999999488.000$   \\
SDSS & J0850+3246 &  132.70103 &   32.77998 &  5.87   &   $-999999500.00\pm-999999500.000$  &  $19.66\pm0.083$  &  $-999999500.00\pm-999999500.000$   & $-999999500.00\pm-999999500.000$    &   $19.372\pm0.039$   &  $19.25\pm0.077$   &   $17.11\pm-999999488.000$   &   $15.25\pm-999999488.000$   \\
SHELLQs & J0853+0139 &  133.45350 &    1.65306 &  6.01   &   $23.63\pm0.574$  &  $23.52\pm0.675$  &  $22.33\pm0.506$   & $-999999500.00\pm-999999500.000$    &   $-999999485.331\pm-999999488.000$   &  $-999999484.72\pm-999999488.000$   &   $17.48\pm-999999488.000$   &   $15.62\pm-999999488.000$   \\
SDSS & J0854+2056 &  133.62655 &   20.94745 &  5.17   &   $19.43\pm0.040$  &  $19.46\pm0.051$  &  $19.06\pm0.049$   & $19.08\pm0.034$    &   $18.908\pm0.027$   &  $18.77\pm0.056$   &   $16.80\pm-999999488.000$   &   $15.50\pm-999999488.000$   \\
SHELLQs & J0857+0056 &  134.41054 &    0.93686 &  6.35   &   $23.35\pm0.446$  &  $24.04\pm0.814$  &  $26.70\pm13.151$   & $23.98\pm1.645$    &   $-999999485.331\pm-999999488.000$   &  $-999999484.72\pm-999999488.000$   &   $-999999482.85\pm-999999488.000$   &   $-999999481.34\pm-999999488.000$   \\
SHELLQs & J0858+0000 &  134.55629 &    0.01586 &  5.99   &   $21.98\pm0.098$  &  $21.15\pm0.055$  &  $21.05\pm0.076$   & $21.02\pm0.102$    &   $21.060\pm0.167$   &  $-999999484.72\pm-999999488.000$   &   $-999999482.85\pm-999999488.000$   &   $-999999481.34\pm-999999488.000$   \\
HSC & J0859+0022 &  134.77996 &    0.38219 &  6.39   &   $22.29\pm0.288$  &  $23.56\pm0.775$  &  $22.90\pm0.475$   & $22.10\pm0.347$    &   $-999999485.331\pm-999999488.000$   &  $-999999484.72\pm-999999488.000$   &   $-999999482.85\pm-999999488.000$   &   $-999999481.34\pm-999999488.000$   \\
PSO & J135.3860+16.2518 &  135.38604 &   16.25190 &  5.63   &   $-999999500.00\pm-999999500.000$  &  $20.60\pm0.242$  &  $-999999500.00\pm-999999500.000$   & $-999999500.00\pm-999999500.000$    &   $20.292\pm0.094$   &  $19.57\pm0.105$   &   $17.38\pm0.466$   &   $15.52\pm-999999488.000$   \\
SDSS & J0902+0851 &  135.69067 &    8.85442 &  5.22   &   $20.05\pm0.139$  &  $19.89\pm0.056$  &  $19.63\pm0.062$   & $19.49\pm0.067$    &   $19.419\pm0.043$   &  $19.14\pm0.072$   &   $17.64\pm-999999488.000$   &   $15.40\pm-999999488.000$   \\
SHELLQs & J0902+0155 &  135.72862 &    1.91969 &  6.01   &   $24.91\pm1.750$  &  $22.93\pm0.280$  &  $23.42\pm0.341$   & $-999999500.00\pm-999999500.000$    &   $-999999485.331\pm-999999488.000$   &  $-999999484.72\pm-999999488.000$   &   $-999999482.85\pm-999999488.000$   &   $-999999481.34\pm-999999488.000$   \\
SHELLQs & J0903+0211 &  135.81117 &    2.19119 &  5.92   &   $23.62\pm0.466$  &  $24.56\pm1.142$  &  $23.46\pm1.104$   & $24.63\pm3.310$    &   $-999999485.331\pm-999999488.000$   &  $-999999484.72\pm-999999488.000$   &   $-999999482.85\pm-999999488.000$   &   $-999999481.34\pm-999999488.000$   \\
PSO & J135.8704-13.8336 &  135.87046 &  -13.83369 &  5.91   &   $-999999500.00\pm-999999500.000$  &  $21.09\pm0.286$  &  $-999999500.00\pm-999999500.000$   & $20.91\pm0.483$    &   $20.028\pm0.068$   &  $19.75\pm0.112$   &   $-999999482.85\pm-999999488.000$   &   $-999999481.34\pm-999999488.000$   \\
SHELLQs & J0905+0300 &  136.43604 &    3.01633 &  6.27   &   $-999999500.00\pm-999999500.000$  &  $24.16\pm1.411$  &  $23.14\pm0.654$   & $22.19\pm0.549$    &   $-999999485.331\pm-999999488.000$   &  $-999999484.72\pm-999999488.000$   &   $-999999482.85\pm-999999488.000$   &   $-999999481.34\pm-999999488.000$   \\
SDSS & J0906+6930 &  136.62812 &   69.50856 &  5.47   &   $-999999500.00\pm-999999500.000$  &  $-999999500.00\pm-999999500.000$  &  $-999999500.00\pm-999999500.000$   & $-999999500.00\pm-999999500.000$    &   $19.368\pm0.034$   &  $19.10\pm0.056$   &   $17.84\pm0.486$   &   $15.29\pm-999999488.000$   \\
SHELLQs & J0909+0440 &  137.33958 &    4.67858 &  6.15   &   $21.61\pm0.291$  &  $22.17\pm0.665$  &  $22.95\pm2.576$   & $21.86\pm1.007$    &   $-999999485.331\pm-999999488.000$   &  $-999999484.72\pm-999999488.000$   &   $-999999482.85\pm-999999488.000$   &   $-999999481.34\pm-999999488.000$   \\
SHELLQs & J0911+0152 &  137.80946 &    1.87206 &  6.07   &   $-999999500.00\pm-999999500.000$  &  $-999999500.00\pm-999999500.000$  &  $25.02\pm3.026$   & $23.85\pm1.626$    &   $-999999485.331\pm-999999488.000$   &  $-999999484.72\pm-999999488.000$   &   $-999999482.85\pm-999999488.000$   &   $-999999481.34\pm-999999488.000$   \\
SDSS & J0913+5919 &  138.31896 &   59.32269 &  5.12   &   $-999999500.00\pm-999999500.000$  &  $20.24\pm0.180$  &  $-999999500.00\pm-999999500.000$   & $-999999500.00\pm-999999500.000$    &   $19.746\pm0.050$   &  $19.41\pm0.078$   &   $-999999482.85\pm-999999488.000$   &   $-999999481.34\pm-999999488.000$   \\
SDSS & J0915+4924 &  138.93184 &   49.40462 &  5.19   &   $-999999500.00\pm-999999500.000$  &  $19.51\pm0.077$  &  $-999999500.00\pm-999999500.000$   & $-999999500.00\pm-999999500.000$    &   $19.136\pm0.031$   &  $18.90\pm0.054$   &   $17.57\pm0.440$   &   $15.47\pm-999999488.000$   \\
SDSS & J0917+3830 &  139.49149 &   38.51115 &  5.11   &   $-999999500.00\pm-999999500.000$  &  $21.29\pm0.344$  &  $-999999500.00\pm-999999500.000$   & $-999999500.00\pm-999999500.000$    &   $20.256\pm0.078$   &  $20.14\pm0.156$   &   $17.78\pm-999999488.000$   &   $15.45\pm-999999488.000$   \\
SHELLQs & J0918+0139 &  139.63821 &    1.65647 &  6.19   &   $23.10\pm0.279$  &  $23.08\pm0.321$  &  $22.62\pm0.483$   & $22.48\pm0.615$    &   $-999999485.331\pm-999999488.000$   &  $-999999484.72\pm-999999488.000$   &   $-999999482.85\pm-999999488.000$   &   $-999999481.34\pm-999999488.000$   \\
SHELLQs & J0921+0007 &  140.33567 &    0.12303 &  6.56   &   $21.27\pm0.089$  &  $21.11\pm0.107$  &  $20.87\pm0.147$   & $20.40\pm0.093$    &   $20.058\pm0.073$   &  $-999999484.72\pm-999999488.000$   &   $17.06\pm-999999488.000$   &   $15.53\pm-999999488.000$   \\
SDSS & J0922+2653 &  140.57006 &   26.89974 &  5.05   &   $-999999500.00\pm-999999500.000$  &  $20.06\pm0.109$  &  $-999999500.00\pm-999999500.000$   & $-999999500.00\pm-999999500.000$    &   $19.701\pm0.052$   &  $19.89\pm0.132$   &   $17.09\pm-999999488.000$   &   $15.39\pm-999999488.000$   \\
SDSS & J0923+3009 &  140.90327 &   30.16377 &  5.07   &   $-999999500.00\pm-999999500.000$  &  $20.62\pm0.284$  &  $-999999500.00\pm-999999500.000$   & $-999999500.00\pm-999999500.000$    &   $20.149\pm0.075$   &  $19.90\pm0.132$   &   $-999999482.85\pm-999999488.000$   &   $-999999481.34\pm-999999488.000$   \\
SHELLQs & J0923+0402 &  140.94633 &    4.04844 &  6.60   &   $21.03\pm0.119$  &  $20.14\pm0.078$  &  $19.90\pm0.127$   & $19.44\pm0.072$    &   $19.200\pm0.035$   &  $19.05\pm0.066$   &   $17.10\pm-999999488.000$   &   $15.06\pm-999999488.000$   \\
SDSS & J0927+2001 &  141.84092 &   20.02323 &  5.77   &   $-999999500.00\pm-999999500.000$  &  $20.06\pm0.171$  &  $-999999500.00\pm-999999500.000$   & $-999999500.00\pm-999999500.000$    &   $19.577\pm0.049$   &  $19.86\pm0.142$   &   $17.01\pm-999999488.000$   &   $15.09\pm-999999488.000$   \\
SDSS & J0932+1222 &  143.20733 &   12.36828 &  5.02   &   $-999999500.00\pm-999999500.000$  &  $20.40\pm0.265$  &  $-999999500.00\pm-999999500.000$   & $-999999500.00\pm-999999500.000$    &   $-999999485.331\pm-999999488.000$   &  $19.82\pm0.128$   &   $-999999482.85\pm-999999488.000$   &   $-999999481.34\pm-999999488.000$   \\
SUVAQ & J0935-0207 &  143.84713 &   -2.13178 &  5.32   &   $20.11\pm0.047$  &  $20.09\pm0.058$  &  $19.97\pm0.092$   & $19.99\pm0.129$    &   $19.516\pm0.046$   &  $19.34\pm0.084$   &   $17.75\pm-999999488.000$   &   $15.81\pm-999999488.000$   \\
SDSS & J0948+2106 &  147.23068 &   21.10877 &  5.17   &   $-999999500.00\pm-999999500.000$  &  $19.67\pm0.099$  &  $-999999500.00\pm-999999500.000$   & $-999999500.00\pm-999999500.000$    &   $19.783\pm0.058$   &  $19.75\pm0.123$   &   $17.43\pm-999999488.000$   &   $15.42\pm-999999488.000$   \\
SDSS & J0957+0610 &  149.28199 &    6.18321 &  5.14   &   $19.20\pm0.022$  &  $19.02\pm0.025$  &  $18.72\pm0.029$   & $18.66\pm0.037$    &   $18.703\pm0.023$   &  $18.75\pm0.051$   &   $17.07\pm-999999488.000$   &   $15.09\pm-999999488.000$   \\
SUVAW & J0957+1016 &  149.30083 &   10.27181 &  5.14   &   $19.95\pm0.104$  &  $19.97\pm0.089$  &  $19.69\pm0.111$   & $19.87\pm0.131$    &   $19.892\pm0.063$   &  $19.81\pm0.126$   &   $17.33\pm0.413$   &   $15.52\pm0.510$   \\
SDSS & J0957+0519 &  149.36611 &    5.31813 &  5.18   &   $19.73\pm0.059$  &  $19.64\pm0.051$  &  $19.60\pm0.103$   & $19.68\pm0.124$    &   $19.546\pm0.047$   &  $19.70\pm0.115$   &   $-999999482.85\pm-999999488.000$   &   $-999999481.34\pm-999999488.000$   \\
SHELLQs & J0957+0053 &  149.41829 &    0.89267 &  6.05   &   $-999999488.00\pm-999999488.000$  &  $-999999488.00\pm-999999488.000$  &  $24.48\pm5.795$   & $23.45\pm2.691$    &   $-999999485.331\pm-999999488.000$   &  $-999999484.72\pm-999999488.000$   &   $-999999482.85\pm-999999488.000$   &   $-999999481.34\pm-999999488.000$   \\
SDSS & J0958+3524 &  149.55845 &   35.41356 &  5.12   &   $-999999500.00\pm-999999500.000$  &  $20.93\pm0.306$  &  $-999999500.00\pm-999999500.000$   & $-999999500.00\pm-999999500.000$    &   $19.353\pm0.036$   &  $19.55\pm0.093$   &   $17.33\pm-999999488.000$   &   $14.94\pm-999999488.000$   \\
SDSS & J0959+0227 &  149.78375 &    2.45204 &  5.07   &   $24.24\pm0.061$  &  $24.15\pm0.071$  &  $23.60\pm0.068$   & $23.43\pm0.090$    &   $-999999485.331\pm-999999488.000$   &  $-999999484.72\pm-999999488.000$   &   $-999999482.85\pm-999999488.000$   &   $-999999481.34\pm-999999488.000$   \\
SDSS & J1000+2103 &  150.18240 &   21.05741 &  5.07   &   $-999999500.00\pm-999999500.000$  &  $19.61\pm0.095$  &  $-999999500.00\pm-999999500.000$   & $-999999500.00\pm-999999500.000$    &   $19.243\pm0.037$   &  $19.13\pm0.072$   &   $17.32\pm0.451$   &   $15.10\pm-999999488.000$   \\
SDSS & J1000+0234 &  150.21458 &    2.58263 &  5.30   &   $26.44\pm0.388$  &  $26.86\pm0.597$  &  $27.19\pm1.600$   & $26.47\pm1.187$    &   $-999999485.331\pm-999999488.000$   &  $-999999484.72\pm-999999488.000$   &   $-999999482.85\pm-999999488.000$   &   $-999999481.34\pm-999999488.000$   \\
SHELLQs & J1004+0239 &  151.00567 &    2.65853 &  6.41   &   $23.25\pm1.263$  &  $22.55\pm0.094$  &  $22.44\pm0.138$   & $21.90\pm0.095$    &   $-999999485.331\pm-999999488.000$   &  $-999999484.72\pm-999999488.000$   &   $-999999482.85\pm-999999488.000$   &   $-999999481.34\pm-999999488.000$   \\
SUVAW & J1006-0310 &  151.56087 &   -3.17511 &  5.55   &   $19.80\pm0.038$  &  $19.76\pm0.042$  &  $19.31\pm0.069$   & $19.22\pm0.054$    &   $18.956\pm0.028$   &  $18.78\pm0.053$   &   $17.45\pm-999999488.000$   &   $15.06\pm-999999488.000$   \\
SDSS & J1013+4240 &  153.40139 &   42.67400 &  5.03   &   $-999999500.00\pm-999999500.000$  &  $20.19\pm0.185$  &  $-999999500.00\pm-999999500.000$   & $-999999500.00\pm-999999500.000$    &   $19.871\pm0.053$   &  $20.07\pm0.138$   &   $17.13\pm-999999488.000$   &   $15.27\pm-999999488.000$   \\
SUVAW & J1022+0801 &  155.50796 &    8.02283 &  5.30   &   $19.18\pm0.029$  &  $19.05\pm0.030$  &  $18.94\pm0.044$   & $18.81\pm0.040$    &   $18.625\pm0.023$   &  $18.17\pm0.032$   &   $16.62\pm0.219$   &   $15.07\pm-999999488.000$   \\
SDSS & J1022+2252 &  155.54186 &   22.87374 &  5.47   &   $-999999500.00\pm-999999500.000$  &  $19.37\pm0.071$  &  $-999999500.00\pm-999999500.000$   & $-999999500.00\pm-999999500.000$    &   $18.471\pm0.018$   &  $18.11\pm0.028$   &   $17.60\pm0.489$   &   $15.18\pm-999999488.000$   \\
SDSS & J1026+2542 &  156.59845 &   25.71651 &  5.25   &   $-999999500.00\pm-999999500.000$  &  $19.43\pm0.092$  &  $-999999500.00\pm-999999500.000$   & $-999999500.00\pm-999999500.000$    &   $19.358\pm0.039$   &  $18.99\pm0.062$   &   $17.22\pm-999999488.000$   &   $15.10\pm-999999488.000$   \\
SDSS & J1028+0746 &  157.13940 &    7.77193 &  5.15   &   $19.98\pm0.052$  &  $19.83\pm0.062$  &  $19.66\pm0.074$   & $19.60\pm0.075$    &   $19.547\pm0.048$   &  $19.46\pm0.101$   &   $17.21\pm-999999488.000$   &   $14.96\pm-999999488.000$   \\
SDSS & J1030+0524 &  157.61296 &    5.41529 &  6.31   &   $19.97\pm0.063$  &  $19.87\pm0.076$  &  $19.79\pm0.109$   & $19.49\pm0.083$    &   $19.182\pm0.036$   &  $19.02\pm0.067$   &   $17.20\pm-999999488.000$   &   $15.14\pm-999999488.000$   \\
PSO & J157.9070-02.6599 &  157.90704 &   -2.65991 &  5.88   &   $20.30\pm0.038$  &  $20.30\pm0.034$  &  $20.12\pm0.065$   & $19.82\pm0.053$    &   $19.619\pm0.049$   &  $19.49\pm0.097$   &   $17.15\pm-999999488.000$   &   $15.68\pm-999999488.000$   \\
SDSS & J1034+5722 &  158.55971 &   57.37436 &  5.40   &   $-999999500.00\pm-999999500.000$  &  $23.33\pm0.177$  &  $-999999500.00\pm-999999500.000$   & $23.11\pm0.319$    &   $-999999485.331\pm-999999488.000$   &  $-999999484.72\pm-999999488.000$   &   $-999999482.85\pm-999999488.000$   &   $-999999481.34\pm-999999488.000$   \\
SDSS & J1034+2033 &  158.57771 &   20.55006 &  5.01   &   $-999999500.00\pm-999999500.000$  &  $19.74\pm0.100$  &  $-999999500.00\pm-999999500.000$   & $-999999500.00\pm-999999500.000$    &   $18.494\pm0.019$   &  $18.41\pm0.039$   &   $17.12\pm0.341$   &   $15.08\pm0.437$   \\
ATLAS & J158.6938-14.4211 &  158.69382 &  -14.42108 &  6.07   &   $19.28\pm0.074$  &  $19.25\pm0.077$  &  $19.15\pm0.095$   & $18.68\pm0.086$    &   $18.616\pm0.021$   &  $18.47\pm0.040$   &   $16.57\pm0.184$   &   $14.81\pm-999999488.000$   \\
PSO & J159.2257-02.5438 &  159.22579 &   -2.54387 &  6.38   &   $20.09\pm0.124$  &  $20.09\pm0.028$  &  $19.94\pm0.044$   & $19.62\pm0.043$    &   $19.499\pm0.046$   &  $18.99\pm0.064$   &   $17.62\pm0.510$   &   $15.56\pm-999999488.000$   \\
SDSS & J1040-1155 &  160.20250 &  -11.93061 &  5.44   &   $21.97\pm0.594$  &  $21.59\pm0.526$  &  $22.15\pm1.499$   & $20.49\pm0.765$    &   $-999999485.331\pm-999999488.000$   &  $-999999484.72\pm-999999488.000$   &   $-999999482.85\pm-999999488.000$   &   $-999999481.34\pm-999999488.000$   \\
SDSS & J1043+1010 &  160.89664 &   10.17627 &  5.09   &   $20.83\pm0.139$  &  $20.83\pm0.210$  &  $20.06\pm0.162$   & $20.56\pm0.273$    &   $20.515\pm0.113$   &  $20.06\pm0.167$   &   $17.59\pm-999999488.000$   &   $15.38\pm-999999488.000$   \\
SDSS & J1044-0125 &  161.13767 &   -1.41728 &  5.78   &   $19.35\pm0.014$  &  $19.16\pm0.009$  &  $19.10\pm0.014$   & $18.89\pm0.020$    &   $18.888\pm0.026$   &  $18.88\pm0.056$   &   $17.60\pm0.516$   &   $15.68\pm0.540$   \\
DELS & J1048-0109 &  162.07954 &   -1.16117 &  6.68   &   $21.08\pm0.063$  &  $20.86\pm0.060$  &  $20.50\pm0.084$   & $20.44\pm0.091$    &   $20.172\pm0.080$   &  $20.02\pm0.151$   &   $17.67\pm-999999488.000$   &   $15.02\pm-999999488.000$   \\
SDSS & J1048+4637 &  162.18777 &   46.62182 &  6.23   &   $19.50\pm0.071$  &  $19.10\pm0.043$  &  $18.92\pm0.061$   & $18.94\pm0.071$    &   $18.922\pm0.025$   &  $19.00\pm0.055$   &   $17.20\pm-999999488.000$   &   $15.32\pm-999999488.000$   \\
SDSS & J1050+5804 &  162.65195 &   58.07352 &  5.16   &   $19.79\pm0.013$  &  $19.91\pm0.007$  &  $-999999500.00\pm-999999500.000$   & $19.43\pm0.010$    &   $19.171\pm0.029$   &  $18.93\pm0.050$   &   $17.88\pm0.528$   &   $15.80\pm-999999488.000$   \\
SDSS & J1053+5804 &  163.34579 &   58.07004 &  5.26   &   $19.38\pm0.010$  &  $19.46\pm0.005$  &  $-999999500.00\pm-999999500.000$   & $19.24\pm0.007$    &   $19.344\pm0.033$   &  $19.27\pm0.066$   &   $17.37\pm-999999488.000$   &   $15.57\pm0.341$   \\
SDSS & J1054+1633 &  163.68930 &   16.56039 &  5.14   &   $-999999500.00\pm-999999500.000$  &  $19.52\pm0.064$  &  $-999999500.00\pm-999999500.000$   & $-999999500.00\pm-999999500.000$    &   $18.675\pm0.023$   &  $18.58\pm0.045$   &   $-999999482.85\pm-999999488.000$   &   $-999999481.34\pm-999999488.000$   \\
CFHQS & J1059-0906 &  164.86920 &   -9.10567 &  5.92   &   $21.70\pm0.538$  &  $20.35\pm0.182$  &  $21.73\pm0.992$   & $20.83\pm0.487$    &   $20.220\pm0.079$   &  $20.04\pm0.149$   &   $17.54\pm0.497$   &   $14.97\pm-999999488.000$   \\
SDSS & J1101+0531 &  165.39317 &    5.52607 &  5.00   &   $18.90\pm0.031$  &  $18.99\pm0.040$  &  $18.91\pm0.036$   & $19.01\pm0.056$    &   $19.254\pm0.039$   &  $19.42\pm0.095$   &   $17.03\pm-999999488.000$   &   $15.19\pm0.439$   \\
PSO & J167.4726+56.9521 &  167.47263 &   56.95211 &  5.95   &   $-999999500.00\pm-999999500.000$  &  $20.59\pm0.222$  &  $-999999500.00\pm-999999500.000$   & $-999999500.00\pm-999999500.000$    &   $20.521\pm0.087$   &  $-999999484.72\pm-999999488.000$   &   $17.79\pm-999999488.000$   &   $15.40\pm-999999488.000$   \\
PSO & J167.6415-13.4960 &  167.64157 &  -13.49600 &  6.51   &   $20.89\pm0.235$  &  $20.59\pm0.184$  &  $21.73\pm0.716$   & $20.23\pm0.265$    &   $20.465\pm0.103$   &  $-999999484.72\pm-999999488.000$   &   $-999999482.85\pm-999999488.000$   &   $-999999481.34\pm-999999488.000$   \\
SDSS & J1119+3452 &  169.83600 &   34.88003 &  5.01   &   $-999999500.00\pm-999999500.000$  &  $19.77\pm0.103$  &  $-999999500.00\pm-999999500.000$   & $-999999500.00\pm-999999500.000$    &   $19.435\pm0.037$   &  $19.34\pm0.073$   &   $17.44\pm-999999488.000$   &   $15.28\pm-999999488.000$   \\
ULAS & J1120+0641 &  170.00616 &    6.69008 &  7.08   &   $20.24\pm0.045$  &  $20.16\pm0.069$  &  $20.16\pm0.064$   & $19.61\pm0.053$    &   $19.607\pm0.050$   &  $19.76\pm0.127$   &   $17.50\pm-999999488.000$   &   $14.86\pm-999999488.000$   \\
SDSS & J1122+1342 &  170.70851 &   13.71012 &  5.19   &   $20.61\pm0.150$  &  $21.06\pm0.093$  &  $20.69\pm0.053$   & $20.49\pm0.049$    &   $20.142\pm0.077$   &  $20.07\pm0.157$   &   $17.66\pm-999999488.000$   &   $15.30\pm-999999488.000$   \\
SDSS & J1123-0044 &  170.79646 &   -0.73851 &  5.00   &   $20.26\pm0.040$  &  $20.11\pm0.039$  &  $19.96\pm0.052$   & $19.71\pm0.049$    &   $19.772\pm0.058$   &  $19.72\pm0.118$   &   $17.32\pm-999999488.000$   &   $15.58\pm-999999488.000$   \\
SDSS & J1125+4448 &  171.31714 &   44.81248 &  5.11   &   $-999999500.00\pm-999999500.000$  &  $19.44\pm0.085$  &  $-999999500.00\pm-999999500.000$   & $-999999500.00\pm-999999500.000$    &   $18.755\pm0.021$   &  $18.69\pm0.042$   &   $17.61\pm0.385$   &   $15.01\pm-999999488.000$   \\
SDSS & J1126+1734 &  171.65821 &   17.58293 &  5.22   &   $-999999500.00\pm-999999500.000$  &  $19.55\pm0.083$  &  $-999999500.00\pm-999999500.000$   & $-999999500.00\pm-999999500.000$    &   $19.340\pm0.038$   &  $19.17\pm0.072$   &   $16.98\pm-999999488.000$   &   $15.30\pm-999999488.000$   \\
PSO & J172.1770+26.8866 &  172.17700 &   26.88667 &  5.77   &   $-999999500.00\pm-999999500.000$  &  $20.26\pm0.178$  &  $-999999500.00\pm-999999500.000$   & $-999999500.00\pm-999999500.000$    &   $19.831\pm0.055$   &  $19.88\pm0.125$   &   $17.45\pm-999999488.000$   &   $15.06\pm-999999488.000$   \\
SDSS & J1128+5759 &  172.24103 &   57.98607 &  5.00   &   $-999999500.00\pm-999999500.000$  &  $19.12\pm0.055$  &  $-999999500.00\pm-999999500.000$   & $-999999500.00\pm-999999500.000$    &   $19.191\pm0.030$   &  $19.25\pm0.066$   &   $17.58\pm0.378$   &   $15.70\pm-999999488.000$   \\
SDSS & J1132+1209 &  173.19375 &   12.15047 &  5.17   &   $19.36\pm0.053$  &  $19.18\pm0.045$  &  $18.94\pm0.044$   & $18.98\pm0.066$    &   $18.697\pm0.022$   &  $18.54\pm0.044$   &   $16.87\pm0.289$   &   $15.05\pm-999999488.000$   \\
SUVAW & J1133+1603 &  173.28658 &   16.06547 &  5.61   &   $19.71\pm0.071$  &  $19.80\pm0.073$  &  $19.63\pm0.104$   & $19.47\pm0.101$    &   $18.993\pm0.028$   &  $18.92\pm0.057$   &   $17.25\pm-999999488.000$   &   $15.46\pm-999999488.000$   \\
SUVAW & J1134+0828 &  173.55929 &    8.48147 &  5.69   &   $20.23\pm0.058$  &  $20.30\pm0.074$  &  $19.92\pm0.083$   & $19.76\pm0.087$    &   $19.050\pm0.033$   &  $18.41\pm0.040$   &   $17.39\pm0.405$   &   $14.86\pm-999999488.000$   \\
SDSS & J1137+3549 &  174.32387 &   35.83246 &  6.03   &   $-999999500.00\pm-999999500.000$  &  $19.40\pm0.067$  &  $-999999500.00\pm-999999500.000$   & $-999999500.00\pm-999999500.000$    &   $19.102\pm0.028$   &  $19.01\pm0.057$   &   $17.08\pm-999999488.000$   &   $15.39\pm-999999488.000$   \\
PSO & J174.7920-12.2845 &  174.79204 &  -12.28455 &  5.81   &   $20.54\pm0.169$  &  $20.20\pm0.136$  &  $20.40\pm0.266$   & $19.64\pm0.167$    &   $19.796\pm0.056$   &  $19.84\pm0.135$   &   $17.65\pm-999999488.000$   &   $15.38\pm-999999488.000$   \\
PSO & J175.4091-20.2654 &  175.40918 &  -20.26546 &  5.69   &   $20.20\pm0.110$  &  $19.94\pm0.128$  &  $-999999500.00\pm-999999500.000$   & $19.65\pm0.183$    &   $19.449\pm0.043$   &  $19.15\pm0.073$   &   $17.20\pm-999999488.000$   &   $14.77\pm-999999488.000$   \\
SDSS & J1143+3808 &  175.90978 &   38.14134 &  5.80   &   $-999999500.00\pm-999999500.000$  &  $19.92\pm0.137$  &  $-999999500.00\pm-999999500.000$   & $-999999500.00\pm-999999500.000$    &   $19.547\pm0.040$   &  $19.42\pm0.077$   &   $17.95\pm-999999488.000$   &   $15.62\pm-999999488.000$   \\
SHELLQs & J1146-0154 &  176.63608 &   -1.91064 &  6.16   &   $23.37\pm0.688$  &  $23.06\pm0.361$  &  $-999999500.00\pm-999999500.000$   & $23.27\pm1.108$    &   $19.740\pm0.057$   &  $19.88\pm0.139$   &   $17.67\pm-999999488.000$   &   $15.66\pm-999999488.000$   \\
SHELLQs & J1146+0124 &  176.70175 &    1.40558 &  6.27   &   $-999999500.00\pm-999999500.000$  &  $22.62\pm0.221$  &  $-999999500.00\pm-999999500.000$   & $22.56\pm0.297$    &   $-999999485.331\pm-999999488.000$   &  $-999999484.72\pm-999999488.000$   &   $-999999482.85\pm-999999488.000$   &   $-999999481.34\pm-999999488.000$   \\
SDSS & J1146+4037 &  176.74080 &   40.61907 &  5.01   &   $-999999500.00\pm-999999500.000$  &  $19.34\pm0.076$  &  $-999999500.00\pm-999999500.000$   & $-999999500.00\pm-999999500.000$    &   $18.563\pm0.018$   &  $18.46\pm0.034$   &   $17.29\pm-999999488.000$   &   $15.21\pm-999999488.000$   \\
SHELLQs & J1146-0005 &  176.74537 &   -0.09381 &  6.30   &   $24.82\pm1.489$  &  $25.24\pm2.344$  &  $23.41\pm1.135$   & $22.44\pm0.457$    &   $-999999485.331\pm-999999488.000$   &  $-999999484.72\pm-999999488.000$   &   $-999999482.85\pm-999999488.000$   &   $-999999481.34\pm-999999488.000$   \\
SUVAW & J1147-0109 &  176.77671 &   -1.16617 &  5.31   &   $19.22\pm0.012$  &  $19.03\pm0.010$  &  $18.84\pm0.016$   & $18.89\pm0.022$    &   $19.155\pm0.035$   &  $19.07\pm0.069$   &   $17.09\pm0.344$   &   $15.35\pm0.420$   \\
ULAS & J1148+0702 &  177.01370 &    7.03563 &  6.34   &   $20.31\pm0.038$  &  $20.20\pm0.051$  &  $19.77\pm0.121$   & $19.42\pm0.115$    &   $19.225\pm0.036$   &  $18.97\pm0.062$   &   $17.23\pm-999999488.000$   &   $14.90\pm-999999488.000$   \\
RD & J1148+5253 &  177.06754 &   52.89425 &  5.70   &   $21.46\pm0.441$  &  $24.55\pm6.455$  &  $22.91\pm2.328$   & $22.19\pm1.445$    &   $21.031\pm0.132$   &  $-999999484.72\pm-999999488.000$   &   $-999999482.85\pm-999999488.000$   &   $-999999481.34\pm-999999488.000$   \\
SDSS & J1148+5251 &  177.06938 &   52.86400 &  6.42   &   $18.97\pm0.051$  &  $19.01\pm0.041$  &  $18.77\pm0.052$   & $18.71\pm0.059$    &   $18.732\pm0.019$   &  $18.71\pm0.039$   &   $17.71\pm0.452$   &   $15.57\pm0.468$   \\
SDSS & J1148+3020 &  177.10903 &   30.33870 &  5.13   &   $-999999500.00\pm-999999500.000$  &  $19.67\pm0.077$  &  $-999999500.00\pm-999999500.000$   & $-999999500.00\pm-999999500.000$    &   $19.590\pm0.044$   &  $19.63\pm0.099$   &   $17.39\pm-999999488.000$   &   $15.27\pm-999999488.000$   \\
VIK & J1148+0056 &  177.13825 &    0.94507 &  5.84   &   $21.39\pm0.066$  &  $21.58\pm0.067$  &  $21.61\pm0.149$   & $21.09\pm0.065$    &   $20.892\pm0.152$   &  $-999999484.72\pm-999999488.000$   &   $-999999482.85\pm-999999488.000$   &   $-999999481.34\pm-999999488.000$   \\
SUVAW & J1149+0748 &  177.44354 &    7.81406 &  5.66   &   $20.35\pm0.078$  &  $20.29\pm0.099$  &  $20.08\pm0.137$   & $19.88\pm0.135$    &   $20.018\pm0.073$   &  $19.47\pm0.097$   &   $17.69\pm-999999488.000$   &   $14.94\pm-999999488.000$   \\
VIK & J1152+0055 &  178.08863 &    0.92686 &  6.36   &   $21.72\pm0.095$  &  $21.54\pm0.094$  &  $21.49\pm0.183$   & $21.44\pm0.306$    &   $-999999485.331\pm-999999488.000$   &  $-999999484.72\pm-999999488.000$   &   $-999999482.85\pm-999999488.000$   &   $-999999481.34\pm-999999488.000$   \\
PSO & J178.5594-12.1881 &  178.55941 &  -12.18819 &  5.83   &   $21.20\pm0.313$  &  $20.34\pm0.148$  &  $20.42\pm0.298$   & $20.27\pm0.270$    &   $20.098\pm0.073$   &  $19.91\pm0.143$   &   $-999999482.85\pm-999999488.000$   &   $-999999481.34\pm-999999488.000$   \\
SDSS & J1154+2333 &  178.58299 &   23.56591 &  5.01   &   $-999999500.00\pm-999999500.000$  &  $20.05\pm0.022$  &  $19.81\pm0.030$   & $19.79\pm0.030$    &   $19.479\pm0.039$   &  $19.21\pm0.070$   &   $17.65\pm0.496$   &   $14.88\pm-999999488.000$   \\
SDSS & J1154+1341 &  178.60306 &   13.69605 &  5.01   &   $20.06\pm0.087$  &  $19.84\pm0.094$  &  $19.66\pm0.079$   & $19.54\pm0.095$    &   $19.429\pm0.042$   &  $19.38\pm0.088$   &   $17.71\pm-999999488.000$   &   $15.48\pm-999999488.000$   \\
SDSS & J1157+0637 &  179.45161 &    6.61998 &  5.14   &   $20.19\pm0.057$  &  $20.11\pm0.081$  &  $19.89\pm0.086$   & $20.20\pm0.143$    &   $19.642\pm0.052$   &  $19.69\pm0.118$   &   $17.28\pm-999999488.000$   &   $15.49\pm-999999488.000$   \\
SHELLQs & J1201+0133 &  180.26258 &    1.56567 &  6.06   &   $22.92\pm0.402$  &  $22.89\pm0.391$  &  $22.46\pm0.444$   & $22.40\pm0.525$    &   $-999999485.331\pm-999999488.000$   &  $-999999484.72\pm-999999488.000$   &   $-999999482.85\pm-999999488.000$   &   $-999999481.34\pm-999999488.000$   \\
SDSS & J1202+3235 &  180.53242 &   32.59411 &  5.26   &   $-999999500.00\pm-999999500.000$  &  $18.71\pm0.037$  &  $18.76\pm0.098$   & $-999999500.00\pm-999999500.000$    &   $18.654\pm0.020$   &  $18.54\pm0.038$   &   $17.57\pm0.508$   &   $15.72\pm0.539$   \\
HSC & J1202-0057 &  180.69321 &   -0.95047 &  5.93   &   $24.54\pm1.060$  &  $23.35\pm0.371$  &  $23.06\pm0.851$   & $24.42\pm2.967$    &   $-999999485.331\pm-999999488.000$   &  $-999999484.72\pm-999999488.000$   &   $-999999482.85\pm-999999488.000$   &   $-999999481.34\pm-999999488.000$   \\
SDSS & J1204-0021 &  181.17389 &   -0.36379 &  5.09   &   $19.09\pm0.010$  &  $19.04\pm0.011$  &  $18.84\pm0.023$   & $18.80\pm0.025$    &   $18.853\pm0.027$   &  $18.57\pm0.047$   &   $17.23\pm0.345$   &   $14.78\pm-999999488.000$   \\
HSC & J1205-0000 &  181.27124 &   -0.00777 &  6.75   &   $22.70\pm0.161$  &  $22.10\pm0.120$  &  $21.40\pm0.143$   & $20.98\pm0.065$    &   $20.122\pm0.076$   &  $20.06\pm0.165$   &   $17.71\pm-999999488.000$   &   $15.49\pm-999999488.000$   \\
ULAS & J1207+0630 &  181.90600 &    6.50284 &  6.04   &   $20.20\pm0.042$  &  $20.22\pm0.054$  &  $20.05\pm0.204$   & $19.43\pm0.124$    &   $19.814\pm0.061$   &  $19.68\pm0.120$   &   $17.19\pm-999999488.000$   &   $14.88\pm-999999488.000$   \\
HSC & J1207-0005 &  181.97558 &   -0.09814 &  6.01   &   $26.37\pm6.561$  &  $23.99\pm0.830$  &  $22.81\pm2.357$   & $-999999500.00\pm-999999500.000$    &   $-999999485.331\pm-999999488.000$   &  $-999999484.72\pm-999999488.000$   &   $17.67\pm-999999488.000$   &   $15.29\pm-999999488.000$   \\
SDSS & J1208+0010 &  182.09925 &    0.17436 &  5.27   &   $20.37\pm0.041$  &  $20.34\pm0.041$  &  $20.10\pm0.192$   & $20.37\pm0.085$    &   $20.580\pm0.116$   &  $-999999484.72\pm-999999488.000$   &   $-999999482.85\pm-999999488.000$   &   $-999999481.34\pm-999999488.000$   \\
SDSS & J1208+2110 &  182.21945 &   21.17610 &  5.06   &   $-999999500.00\pm-999999500.000$  &  $19.39\pm0.081$  &  $-999999500.00\pm-999999500.000$   & $-999999500.00\pm-999999500.000$    &   $18.742\pm0.022$   &  $18.71\pm0.046$   &   $17.50\pm-999999488.000$   &   $15.17\pm-999999488.000$   \\
SHELLQs & J1208-0200 &  182.24679 &   -2.00967 &  6.20   &   $22.26\pm0.151$  &  $21.84\pm0.110$  &  $22.84\pm0.832$   & $21.49\pm0.190$    &   $20.828\pm0.138$   &  $-999999484.72\pm-999999488.000$   &   $-999999482.85\pm-999999488.000$   &   $-999999481.34\pm-999999488.000$   \\
SHELLQs & J1209-0006 &  182.34996 &   -0.11292 &  5.86   &   $-999999500.00\pm-999999500.000$  &  $23.51\pm0.536$  &  $22.94\pm2.785$   & $22.95\pm0.797$    &   $20.105\pm0.075$   &  $-999999484.72\pm-999999488.000$   &   $17.55\pm-999999488.000$   &   $15.50\pm-999999488.000$   \\
SDSS & J1209+1831 &  182.46971 &   18.52978 &  5.15   &   $-999999500.00\pm-999999500.000$  &  $19.34\pm0.098$  &  $-999999500.00\pm-999999500.000$   & $-999999500.00\pm-999999500.000$    &   $18.952\pm0.027$   &  $18.97\pm0.059$   &   $17.39\pm0.400$   &   $15.21\pm-999999488.000$   \\
PSO & J183.1124+05.0926 &  183.11242 &    5.09264 &  6.44   &   $19.86\pm0.091$  &  $-999999500.00\pm-999999500.000$  &  $19.54\pm0.109$   & $19.74\pm0.151$    &   $19.633\pm0.050$   &  $19.70\pm0.122$   &   $17.65\pm-999999488.000$   &   $15.58\pm-999999488.000$   \\
PSO & J183.2991-12.7676 &  183.29919 &  -12.76762 &  5.86   &   $19.23\pm0.037$  &  $19.07\pm0.033$  &  $19.10\pm0.042$   & $19.10\pm0.077$    &   $18.933\pm0.029$   &  $19.14\pm0.075$   &   $17.57\pm-999999488.000$   &   $15.57\pm-999999488.000$   \\
VIK & J1215+0023 &  183.82030 &    0.39018 &  5.93   &   $21.57\pm0.094$  &  $21.26\pm0.084$  &  $21.35\pm0.161$   & $20.96\pm0.169$    &   $-999999485.331\pm-999999488.000$   &  $-999999484.72\pm-999999488.000$   &   $-999999482.85\pm-999999488.000$   &   $-999999481.34\pm-999999488.000$   \\
PSO & J184.3389+01.5284 &  184.33893 &    1.52846 &  6.20   &   $21.22\pm0.066$  &  $21.28\pm0.075$  &  $21.14\pm0.110$   & $20.74\pm0.115$    &   $20.505\pm0.107$   &  $20.01\pm0.156$   &   $17.30\pm-999999488.000$   &   $14.85\pm-999999488.000$   \\
SHELLQs & J1219+0050 &  184.77225 &    0.84375 &  6.01   &   $22.62\pm0.281$  &  $22.29\pm0.203$  &  $22.10\pm0.456$   & $21.94\pm0.420$    &   $-999999485.331\pm-999999488.000$   &  $-999999484.72\pm-999999488.000$   &   $-999999482.85\pm-999999488.000$   &   $-999999481.34\pm-999999488.000$   \\
SDSS & J1221+4445 &  185.44342 &   44.75779 &  5.19   &   $-999999500.00\pm-999999500.000$  &  $19.68\pm0.102$  &  $-999999500.00\pm-999999500.000$   & $-999999500.00\pm-999999500.000$    &   $19.032\pm0.025$   &  $18.83\pm0.045$   &   $17.15\pm0.293$   &   $15.54\pm0.470$   \\
SDSS & J1222+1958 &  185.65818 &   19.97859 &  5.13   &   $-999999500.00\pm-999999500.000$  &  $19.79\pm0.129$  &  $-999999500.00\pm-999999500.000$   & $-999999500.00\pm-999999500.000$    &   $19.042\pm0.029$   &  $19.10\pm0.066$   &   $17.78\pm-999999488.000$   &   $14.98\pm-999999488.000$   \\
PSO & J187.1047-02.5609 &  187.10479 &   -2.56090 &  5.77   &   $20.99\pm0.055$  &  $20.89\pm0.051$  &  $20.69\pm0.082$   & $20.45\pm0.078$    &   $20.985\pm0.162$   &  $-999999484.72\pm-999999488.000$   &   $16.92\pm-999999488.000$   &   $15.40\pm-999999488.000$   \\
PSO & J187.3050+04.3243 &  187.30503 &    4.32437 &  5.89   &   $20.96\pm0.190$  &  $20.97\pm0.183$  &  $21.26\pm0.519$   & $20.86\pm0.358$    &   $-999999485.331\pm-999999488.000$   &  $-999999484.72\pm-999999488.000$   &   $-999999482.85\pm-999999488.000$   &   $-999999481.34\pm-999999488.000$   \\
SDSS & J1233+0622 &  188.38947 &    6.37617 &  5.30   &   $19.81\pm0.058$  &  $19.75\pm0.021$  &  $19.36\pm0.059$   & $19.22\pm0.020$    &   $19.121\pm0.037$   &  $18.69\pm0.053$   &   $17.32\pm0.382$   &   $15.38\pm-999999488.000$   \\
SDSS & J1236+6209 &  189.19983 &   62.16156 &  5.19   &   $-999999500.00\pm-999999500.000$  &  $-999999500.00\pm-999999500.000$  &  $-999999500.00\pm-999999500.000$   & $-999999500.00\pm-999999500.000$    &   $-999999485.331\pm-999999488.000$   &  $-999999484.72\pm-999999488.000$   &   $17.78\pm-999999488.000$   &   $15.98\pm-999999488.000$   \\
SDSS & J1242+5213 &  190.69966 &   52.21853 &  5.04   &   $-999999500.00\pm-999999500.000$  &  $19.43\pm0.104$  &  $-999999500.00\pm-999999500.000$   & $-999999500.00\pm-999999500.000$    &   $19.091\pm0.025$   &  $19.08\pm0.051$   &   $17.63\pm-999999488.000$   &   $15.30\pm-999999488.000$   \\
ULAS & J1243+2529 &  190.92005 &   25.48997 &  5.83   &   $20.18\pm0.034$  &  $20.12\pm0.048$  &  $19.66\pm0.057$   & $19.36\pm0.051$    &   $19.136\pm0.030$   &  $18.78\pm0.048$   &   $17.71\pm-999999488.000$   &   $15.47\pm-999999488.000$   \\
SDSS & J1250+3130 &  192.71636 &   31.50608 &  6.15   &   $20.25\pm0.072$  &  $20.02\pm0.082$  &  $19.63\pm0.113$   & $19.33\pm0.069$    &   $19.067\pm0.028$   &  $18.67\pm0.043$   &   $17.26\pm-999999488.000$   &   $15.68\pm0.528$   \\
PSO & J194.1290+25.5476 &  194.12903 &   25.54762 &  5.91   &   $20.48\pm0.168$  &  $20.82\pm0.323$  &  $20.74\pm0.283$   & $19.92\pm0.157$    &   $19.667\pm0.046$   &  $19.04\pm0.058$   &   $17.37\pm-999999488.000$   &   $15.54\pm-999999488.000$   \\
SDSS & J1257+6349 &  194.48948 &   63.82699 &  6.02   &   $-999999500.00\pm-999999500.000$  &  $-999999500.00\pm-999999500.000$  &  $-999999500.00\pm-999999500.000$   & $-999999500.00\pm-999999500.000$    &   $19.613\pm0.036$   &  $19.65\pm0.079$   &   $17.67\pm-999999488.000$   &   $15.42\pm-999999488.000$   \\
SDSS & J1306+0356 &  196.53447 &    3.94066 &  6.03   &   $19.97\pm0.034$  &  $19.69\pm0.033$  &  $19.65\pm0.045$   & $19.34\pm0.038$    &   $19.631\pm0.051$   &  $19.51\pm0.099$   &   $17.42\pm0.377$   &   $15.75\pm-999999488.000$   \\
PSO & J197.7198+25.5351 &  197.71980 &   25.53519 &  5.84   &   $20.98\pm0.236$  &  $20.50\pm0.190$  &  $21.06\pm0.369$   & $20.45\pm0.241$    &   $20.046\pm0.062$   &  $-999999484.72\pm-999999488.000$   &   $17.57\pm-999999488.000$   &   $15.54\pm-999999488.000$   \\
SUVAW & J1317-0239 &  199.33658 &   -2.65361 &  5.25   &   $20.61\pm0.039$  &  $20.55\pm0.042$  &  $20.27\pm0.063$   & $20.29\pm0.076$    &   $20.043\pm0.072$   &  $19.83\pm0.129$   &   $17.90\pm-999999488.000$   &   $15.90\pm-999999488.000$   \\
ULAS & J1319+0950 &  199.79709 &    9.84764 &  6.13   &   $19.84\pm0.059$  &  $19.58\pm0.045$  &  $19.72\pm0.129$   & $19.44\pm0.082$    &   $19.574\pm0.042$   &  $19.53\pm0.088$   &   $17.73\pm-999999488.000$   &   $15.51\pm-999999488.000$   \\
PSO & J201.9222+57.5440 &  201.92218 &   57.54399 &  5.74   &   $-999999500.00\pm-999999500.000$  &  $20.59\pm0.267$  &  $-999999500.00\pm-999999500.000$   & $-999999500.00\pm-999999500.000$    &   $19.946\pm0.047$   &  $19.58\pm0.073$   &   $18.01\pm-999999488.000$   &   $15.72\pm-999999488.000$   \\
SDWISE & J1332+2208 &  203.23937 &   22.14331 &  5.11   &   $19.13\pm0.043$  &  $19.02\pm0.040$  &  $18.71\pm0.036$   & $18.48\pm0.036$    &   $18.269\pm0.014$   &  $18.22\pm0.029$   &   $17.32\pm0.347$   &   $15.14\pm-999999488.000$   \\
SDSS & J1334+1220 &  203.55235 &   12.33909 &  5.12   &   $19.45\pm0.056$  &  $19.28\pm0.038$  &  $19.06\pm0.059$   & $19.01\pm0.056$    &   $19.226\pm0.033$   &  $19.01\pm0.060$   &   $17.55\pm0.372$   &   $15.56\pm-999999488.000$   \\
SDSS & J1335+3533 &  203.96171 &   35.55439 &  5.90   &   $19.99\pm0.111$  &  $19.78\pm0.126$  &  $19.73\pm0.114$   & $19.56\pm0.142$    &   $19.377\pm0.033$   &  $19.20\pm0.060$   &   $17.30\pm-999999488.000$   &   $15.96\pm-999999488.000$   \\
SUVAW & J1335-0328 &  203.98433 &   -3.47728 &  5.67   &   $18.65\pm0.008$  &  $18.66\pm0.008$  &  $18.55\pm0.016$   & $18.34\pm0.014$    &   $18.303\pm0.017$   &  $18.12\pm0.029$   &   $17.43\pm0.339$   &   $15.37\pm-999999488.000$   \\
SDSS & J1337+4155 &  204.37004 &   41.92774 &  5.03   &   $-999999500.00\pm-999999500.000$  &  $19.50\pm0.087$  &  $-999999500.00\pm-999999500.000$   & $-999999500.00\pm-999999500.000$    &   $19.326\pm0.031$   &  $19.26\pm0.062$   &   $17.94\pm0.524$   &   $15.78\pm-999999488.000$   \\
SDSS & J1340+3926 &  205.06263 &   39.44186 &  5.03   &   $-999999500.00\pm-999999500.000$  &  $19.30\pm0.052$  &  $-999999500.00\pm-999999500.000$   & $-999999500.00\pm-999999500.000$    &   $18.920\pm0.023$   &  $18.84\pm0.044$   &   $17.80\pm0.363$   &   $15.55\pm-999999488.000$   \\
SDSS & J1340+2813 &  205.16767 &   28.22449 &  5.34   &   $19.46\pm0.046$  &  $19.28\pm0.051$  &  $19.08\pm0.053$   & $18.95\pm0.050$    &   $18.747\pm0.020$   &  $18.38\pm0.031$   &   $17.50\pm0.343$   &   $15.80\pm0.495$   \\
SDSS & J1341+4611 &  205.42275 &   46.18619 &  5.02   &   $-999999500.00\pm-999999500.000$  &  $20.60\pm0.257$  &  $-999999500.00\pm-999999500.000$   & $-999999500.00\pm-999999500.000$    &   $19.699\pm0.045$   &  $19.83\pm0.106$   &   $17.11\pm-999999488.000$   &   $15.82\pm-999999488.000$   \\
SDSS & J1341+3510 &  205.47508 &   35.16825 &  5.23   &   $19.70\pm0.085$  &  $19.46\pm0.111$  &  $19.14\pm0.116$   & $19.10\pm0.091$    &   $19.044\pm0.025$   &  $18.85\pm0.046$   &   $17.28\pm-999999488.000$   &   $15.90\pm-999999488.000$   \\
ULAS & J1342+0928 &  205.53375 &    9.47739 &  7.54   &   $21.36\pm0.169$  &  $20.64\pm0.082$  &  $20.01\pm0.118$   & $20.01\pm0.119$    &   $20.294\pm0.080$   &  $20.26\pm0.170$   &   $17.98\pm0.498$   &   $15.92\pm-999999488.000$   \\
SDSS & J1345+2329 &  206.36093 &   23.49705 &  5.06   &   $18.36\pm0.022$  &  $18.33\pm0.027$  &  $18.21\pm0.034$   & $18.23\pm0.036$    &   $18.323\pm0.015$   &  $18.37\pm0.031$   &   $16.72\pm0.146$   &   $15.66\pm0.417$   \\
PSO & J209.2058-26.7083 &  209.20586 &  -26.70840 &  5.72   &   $19.42\pm0.048$  &  $19.44\pm0.061$  &  $-999999500.00\pm-999999500.000$   & $19.15\pm0.105$    &   $19.293\pm0.038$   &  $18.82\pm0.056$   &   $17.64\pm0.420$   &   $15.86\pm-999999488.000$   \\
MMT & J1357+5305 &  209.44725 &   53.09514 &  5.32   &   $20.72\pm0.028$  &  $20.74\pm0.024$  &  $-999999500.00\pm-999999500.000$   & $-999999500.00\pm-999999500.000$    &   $20.354\pm0.071$   &  $20.15\pm0.124$   &   $-999999482.85\pm-999999488.000$   &   $-999999481.34\pm-999999488.000$   \\
SHELLQs & J1400-0011 &  210.11996 &   -0.19764 &  6.04   &   $23.52\pm0.557$  &  $22.39\pm0.239$  &  $25.42\pm9.016$   & $23.77\pm2.399$    &   $-999999485.331\pm-999999488.000$   &  $-999999484.72\pm-999999488.000$   &   $-999999482.85\pm-999999488.000$   &   $-999999481.34\pm-999999488.000$   \\
SHELLQs & J1400-0125 &  210.12496 &   -1.42250 &  6.04   &   $22.80\pm0.285$  &  $22.49\pm0.226$  &  $22.16\pm0.310$   & $21.87\pm0.292$    &   $-999999485.331\pm-999999488.000$   &  $-999999484.72\pm-999999488.000$   &   $-999999482.85\pm-999999488.000$   &   $-999999481.34\pm-999999488.000$   \\
PSO & J210.4472+27.8263 &  210.44723 &   27.82640 &  6.14   &   $20.85\pm0.123$  &  $20.45\pm0.101$  &  $20.58\pm0.179$   & $20.23\pm0.158$    &   $20.202\pm0.070$   &  $20.24\pm0.156$   &   $17.49\pm-999999488.000$   &   $15.65\pm-999999488.000$   \\
PSO & J210.7277+40.4008 &  210.72777 &   40.40089 &  6.04   &   $-999999500.00\pm-999999500.000$  &  $21.02\pm0.416$  &  $-999999500.00\pm-999999500.000$   & $-999999500.00\pm-999999500.000$    &   $20.593\pm0.092$   &  $20.22\pm0.144$   &   $-999999482.85\pm-999999488.000$   &   $-999999481.34\pm-999999488.000$   \\
PSO & J210.8297+09.0474 &  210.82970 &    9.04750 &  5.88   &   $20.29\pm0.118$  &  $20.09\pm0.030$  &  $19.93\pm0.094$   & $19.83\pm0.108$    &   $19.905\pm0.058$   &  $19.99\pm0.134$   &   $17.42\pm-999999488.000$   &   $15.71\pm0.419$   \\
PSO & J210.8722-12.0094 &  210.87222 &  -12.00948 &  5.84   &   $20.71\pm0.223$  &  $20.34\pm0.157$  &  $20.68\pm0.388$   & $21.34\pm0.765$    &   $20.709\pm0.130$   &  $-999999484.72\pm-999999488.000$   &   $-999999482.85\pm-999999488.000$   &   $-999999481.34\pm-999999488.000$   \\
SHELLQs & J1406-0116 &  211.62133 &   -1.26978 &  6.33   &   $22.13\pm0.108$  &  $21.83\pm0.095$  &  $21.97\pm0.227$   & $21.78\pm0.211$    &   $-999999485.331\pm-999999488.000$   &  $-999999484.72\pm-999999488.000$   &   $-999999482.85\pm-999999488.000$   &   $-999999481.34\pm-999999488.000$   \\
SHELLQs & J1406-0144 &  211.69533 &   -1.73406 &  6.10   &   $-999999500.00\pm-999999500.000$  &  $22.95\pm0.323$  &  $22.65\pm0.500$   & $22.42\pm0.489$    &   $-999999485.331\pm-999999488.000$   &  $-999999484.72\pm-999999488.000$   &   $-999999482.85\pm-999999488.000$   &   $-999999481.34\pm-999999488.000$   \\
MMT & J1408+5300 &  212.09550 &   53.00581 &  5.07   &   $-999999500.00\pm-999999500.000$  &  $21.17\pm0.067$  &  $-999999500.00\pm-999999500.000$   & $20.65\pm0.063$    &   $20.547\pm0.080$   &  $20.24\pm0.134$   &   $18.00\pm-999999488.000$   &   $15.97\pm-999999488.000$   \\
PSO & J212.2974-15.9865 &  212.29743 &  -15.98657 &  5.83   &   $20.65\pm0.234$  &  $20.85\pm0.309$  &  $22.56\pm2.092$   & $23.32\pm5.197$    &   $20.554\pm0.116$   &  $-999999484.72\pm-999999488.000$   &   $-999999482.85\pm-999999488.000$   &   $-999999481.34\pm-999999488.000$   \\
SDSS & J1411+1217 &  212.79703 &   12.29369 &  5.90   &   $20.07\pm0.058$  &  $20.06\pm0.055$  &  $19.66\pm0.064$   & $19.42\pm0.062$    &   $19.123\pm0.030$   &  $18.74\pm0.046$   &   $17.90\pm-999999488.000$   &   $15.90\pm-999999488.000$   \\
PSO & J213.3629-22.5617 &  213.36299 &  -22.56174 &  5.92   &   $19.71\pm0.060$  &  $19.81\pm0.083$  &  $-999999500.00\pm-999999500.000$   & $19.38\pm0.121$    &   $19.372\pm0.041$   &  $19.07\pm0.069$   &   $17.38\pm0.421$   &   $15.25\pm-999999488.000$   \\
MMT & J1414+5115 &  213.51817 &   51.25994 &  5.24   &   $-999999500.00\pm-999999500.000$  &  $21.83\pm0.788$  &  $-999999500.00\pm-999999500.000$   & $-999999500.00\pm-999999500.000$    &   $20.675\pm0.083$   &  $-999999484.72\pm-999999488.000$   &   $18.21\pm-999999488.000$   &   $16.00\pm-999999488.000$   \\
MMT & J1414+5732 &  213.63154 &   57.54281 &  5.16   &   $21.38\pm0.102$  &  $21.25\pm0.148$  &  $20.68\pm0.492$   & $21.86\pm1.089$    &   $20.711\pm0.087$   &  $20.45\pm0.148$   &   $-999999482.85\pm-999999488.000$   &   $-999999481.34\pm-999999488.000$   \\
SHELLQs & J1414+0130 &  213.66475 &    1.51014 &  5.94   &   $23.25\pm0.428$  &  $23.65\pm0.697$  &  $23.57\pm1.689$   & $23.59\pm1.793$    &   $-999999485.331\pm-999999488.000$   &  $-999999484.72\pm-999999488.000$   &   $-999999482.85\pm-999999488.000$   &   $-999999481.34\pm-999999488.000$   \\
MMT & J1414+5446 &  213.69508 &   54.77550 &  5.42   &   $22.55\pm0.251$  &  $23.49\pm0.661$  &  $-999999500.00\pm-999999500.000$   & $-999999488.00\pm-999999488.000$    &   $-999999485.331\pm-999999488.000$   &  $-999999484.72\pm-999999488.000$   &   $-999999482.85\pm-999999488.000$   &   $-999999481.34\pm-999999488.000$   \\
PSO & J213.7329-13.4803 &  213.73292 &  -13.48035 &  5.78   &   $20.83\pm0.105$  &  $20.77\pm0.113$  &  $20.46\pm0.113$   & $20.33\pm0.123$    &   $20.306\pm0.093$   &  $20.08\pm0.168$   &   $17.94\pm-999999488.000$   &   $15.75\pm-999999488.000$   \\
SHELLQs & J1416+0015 &  214.05296 &    0.26283 &  6.03   &   $23.71\pm0.645$  &  $24.41\pm1.355$  &  $24.16\pm1.926$   & $24.23\pm2.664$    &   $-999999485.331\pm-999999488.000$   &  $-999999484.72\pm-999999488.000$   &   $-999999482.85\pm-999999488.000$   &   $-999999481.34\pm-999999488.000$   \\
SHELLQs & J1416+0147 &  214.22088 &    1.78394 &  6.07   &   $23.76\pm0.647$  &  $23.26\pm0.488$  &  $22.42\pm0.500$   & $24.09\pm2.412$    &   $-999999485.331\pm-999999488.000$   &  $-999999484.72\pm-999999488.000$   &   $-999999482.85\pm-999999488.000$   &   $-999999481.34\pm-999999488.000$   \\
SHELLQs & J1417+0117 &  214.36946 &    1.28678 &  6.02   &   $23.68\pm0.584$  &  $23.83\pm0.788$  &  $22.15\pm0.356$   & $-999999500.00\pm-999999500.000$    &   $-999999485.331\pm-999999488.000$   &  $-999999484.72\pm-999999488.000$   &   $-999999482.85\pm-999999488.000$   &   $-999999481.34\pm-999999488.000$   \\
MMT & J1419+5553 &  214.98537 &   55.88783 &  5.00   &   $23.45\pm0.785$  &  $22.47\pm0.390$  &  $-999999500.00\pm-999999500.000$   & $-999999500.00\pm-999999500.000$    &   $-999999485.331\pm-999999488.000$   &  $-999999484.72\pm-999999488.000$   &   $-999999482.85\pm-999999488.000$   &   $-999999481.34\pm-999999488.000$   \\
PSO & J215.1514-16.0417 &  215.15143 &  -16.04173 &  5.73   &   $19.24\pm0.048$  &  $18.82\pm0.033$  &  $18.68\pm0.042$   & $18.63\pm0.056$    &   $18.324\pm0.018$   &  $18.18\pm0.032$   &   $-999999482.85\pm-999999488.000$   &   $-999999481.34\pm-999999488.000$   \\
SHELLQs & J1422+0011 &  215.50096 &    0.18417 &  5.89   &   $-999999500.00\pm-999999488.000$  &  $23.32\pm0.707$  &  $22.89\pm0.682$   & $26.04\pm11.949$    &   $-999999485.331\pm-999999488.000$   &  $-999999484.72\pm-999999488.000$   &   $-999999482.85\pm-999999488.000$   &   $-999999481.34\pm-999999488.000$   \\
SDSS & J1423+1303 &  215.85801 &   13.05020 &  5.02   &   $19.32\pm0.047$  &  $19.22\pm0.038$  &  $19.02\pm0.045$   & $18.93\pm0.046$    &   $18.773\pm0.022$   &  $18.83\pm0.049$   &   $17.55\pm-999999488.000$   &   $15.60\pm-999999488.000$   \\
SHELLQs & J1423-0018 &  215.88213 &   -0.30253 &  6.13   &   $-999999500.00\pm-999999500.000$  &  $24.52\pm1.540$  &  $-999999500.00\pm-999999500.000$   & $23.01\pm0.863$    &   $-999999485.331\pm-999999488.000$   &  $-999999484.72\pm-999999488.000$   &   $-999999482.85\pm-999999488.000$   &   $-999999481.34\pm-999999488.000$   \\
NDWFS & J1425+3254 &  216.31805 &   32.90265 &  5.89   &   $20.35\pm0.023$  &  $20.19\pm0.175$  &  $-999999500.00\pm-999999500.000$   & $20.15\pm0.026$    &   $19.790\pm0.045$   &  $19.63\pm0.082$   &   $17.58\pm-999999488.000$   &   $15.61\pm-999999488.000$   \\
SHELLQs & J1425-0015 &  216.32383 &   -0.26136 &  6.18   &   $24.00\pm0.858$  &  $23.27\pm0.525$  &  $23.00\pm0.759$   & $21.98\pm0.325$    &   $-999999485.331\pm-999999488.000$   &  $-999999484.72\pm-999999488.000$   &   $-999999482.85\pm-999999488.000$   &   $-999999481.34\pm-999999488.000$   \\
SDSS & J1427+3522 &  216.87371 &   35.36916 &  5.53   &   $-999999500.00\pm-999999500.000$  &  $20.72\pm0.322$  &  $-999999500.00\pm-999999500.000$   & $-999999500.00\pm-999999500.000$    &   $20.078\pm0.058$   &  $19.81\pm0.099$   &   $18.10\pm0.536$   &   $15.94\pm-999999488.000$   \\
FIRST & J1427+3312 &  216.91079 &   33.21167 &  6.12   &   $21.13\pm0.039$  &  $20.71\pm0.304$  &  $-999999500.00\pm-999999500.000$   & $19.93\pm0.020$    &   $19.348\pm0.031$   &  $19.11\pm0.054$   &   $17.75\pm-999999488.000$   &   $15.95\pm-999999488.000$   \\
PSO & J217.0891-16.0453 &  217.08913 &  -16.04536 &  6.15   &   $20.02\pm0.079$  &  $19.71\pm0.060$  &  $19.73\pm0.079$   & $19.37\pm0.092$    &   $19.091\pm0.033$   &  $19.05\pm0.069$   &   $-999999482.85\pm-999999488.000$   &   $-999999481.34\pm-999999488.000$   \\
SHELLQs & J1429-0104 &  217.26283 &   -1.07872 &  6.80   &   $26.48\pm12.233$  &  $-999999500.00\pm-999999500.000$  &  $24.19\pm2.368$   & $23.05\pm1.073$    &   $-999999485.331\pm-999999488.000$   &  $-999999484.72\pm-999999488.000$   &   $-999999482.85\pm-999999488.000$   &   $-999999481.34\pm-999999488.000$   \\
SHELLQs & J1429-0002 &  217.33425 &   -0.03539 &  6.04   &   $22.76\pm0.352$  &  $22.93\pm0.424$  &  $23.07\pm0.933$   & $22.34\pm0.502$    &   $-999999485.331\pm-999999488.000$   &  $-999999484.72\pm-999999488.000$   &   $17.42\pm-999999488.000$   &   $15.93\pm-999999488.000$   \\
SDSS & J1429+3304 &  217.40821 &   33.07117 &  5.39   &   $20.66\pm0.032$  &  $20.74\pm0.258$  &  $-999999500.00\pm-999999500.000$   & $20.45\pm0.035$    &   $20.556\pm0.087$   &  $20.13\pm0.129$   &   $17.59\pm-999999488.000$   &   $16.15\pm-999999488.000$   \\
CFHQS & J1429+5447 &  217.46737 &   54.78825 &  6.18   &   $20.80\pm0.057$  &  $20.71\pm0.070$  &  $-999999500.00\pm-999999500.000$   & $-999999500.00\pm-999999500.000$    &   $20.015\pm0.047$   &  $20.13\pm0.110$   &   $17.80\pm-999999488.000$   &   $16.11\pm-999999488.000$   \\
PSO & J217.9185-07.4120 &  217.91853 &   -7.41207 &  6.14   &   $20.33\pm0.116$  &  $19.85\pm0.076$  &  $19.84\pm0.118$   & $19.82\pm0.146$    &   $19.918\pm0.065$   &  $19.67\pm0.111$   &   $17.28\pm-999999488.000$   &   $15.49\pm-999999488.000$   \\
SDSS & J1436+2132 &  219.02085 &   21.54424 &  5.22   &   $-999999500.00\pm-999999500.000$  &  $19.45\pm0.078$  &  $-999999500.00\pm-999999500.000$   & $-999999500.00\pm-999999500.000$    &   $19.191\pm0.029$   &  $19.22\pm0.063$   &   $17.55\pm-999999488.000$   &   $15.43\pm-999999488.000$   \\
SDSS & J1436+5007 &  219.04892 &   50.11865 &  5.85   &   $-999999500.00\pm-999999500.000$  &  $19.89\pm0.146$  &  $-999999500.00\pm-999999500.000$   & $-999999500.00\pm-999999500.000$    &   $19.868\pm0.043$   &  $19.91\pm0.096$   &   $18.06\pm-999999488.000$   &   $15.75\pm-999999488.000$   \\
SDSS & J1437+2323 &  219.46594 &   23.38704 &  5.30   &   $-999999500.00\pm-999999500.000$  &  $19.30\pm0.064$  &  $-999999500.00\pm-999999500.000$   & $-999999500.00\pm-999999500.000$    &   $18.717\pm0.019$   &  $18.33\pm0.029$   &   $17.55\pm-999999488.000$   &   $16.19\pm-999999488.000$   \\
MMT & J1437+5151 &  219.48558 &   51.85419 &  5.17   &   $22.33\pm0.183$  &  $22.19\pm0.167$  &  $-999999500.00\pm-999999500.000$   & $-999999500.00\pm-999999500.000$    &   $-999999485.331\pm-999999488.000$   &  $-999999484.72\pm-999999488.000$   &   $-999999482.85\pm-999999488.000$   &   $-999999481.34\pm-999999488.000$   \\
SHELLQs & J1440-0107 &  220.00542 &   -1.11728 &  6.13   &   $23.05\pm0.408$  &  $25.59\pm3.872$  &  $23.61\pm1.053$   & $22.39\pm0.453$    &   $-999999485.331\pm-999999488.000$   &  $-999999484.72\pm-999999488.000$   &   $-999999482.85\pm-999999488.000$   &   $-999999481.34\pm-999999488.000$   \\
SDSS & J1443+3623 &  220.96111 &   36.38754 &  5.12   &   $-999999500.00\pm-999999500.000$  &  $18.97\pm0.056$  &  $-999999500.00\pm-999999500.000$   & $-999999500.00\pm-999999500.000$    &   $18.517\pm0.016$   &  $18.27\pm0.026$   &   $16.34\pm0.096$   &   $15.36\pm0.264$   \\
CFHQS & J1509-1749 &  227.42408 &  -17.82411 &  6.12   &   $19.80\pm0.043$  &  $19.75\pm0.051$  &  $-999999500.00\pm-999999500.000$   & $19.49\pm0.093$    &   $-999999485.331\pm-999999488.000$   &  $19.25\pm0.092$   &   $-999999482.85\pm-999999488.000$   &   $-999999481.34\pm-999999488.000$   \\
SDSS & J1510+5148 &  227.64705 &   51.81142 &  5.06   &   $-999999500.00\pm-999999500.000$  &  $19.49\pm0.080$  &  $-999999500.00\pm-999999500.000$   & $-999999500.00\pm-999999500.000$    &   $18.918\pm0.019$   &  $18.91\pm0.038$   &   $17.92\pm0.341$   &   $16.21\pm-999999488.000$   \\
SUVAW & J1513+0854 &  228.41517 &    8.90181 &  5.47   &   $19.87\pm0.067$  &  $19.97\pm0.059$  &  $19.78\pm0.078$   & $19.76\pm0.103$    &   $19.947\pm0.057$   &  $19.93\pm0.123$   &   $17.71\pm-999999488.000$   &   $15.70\pm-999999488.000$   \\
PSO & J228.6871+21.2388 &  228.68712 &   21.23883 &  5.92   &   $-999999500.00\pm-999999500.000$  &  $20.52\pm0.231$  &  $-999999500.00\pm-999999500.000$   & $-999999500.00\pm-999999500.000$    &   $19.818\pm0.051$   &  $19.61\pm0.088$   &   $-999999482.85\pm-999999488.000$   &   $-999999481.34\pm-999999488.000$   \\
SDWISE & J1523+5916 &  230.76208 &   59.27584 &  5.11   &   $-999999500.00\pm-999999500.000$  &  $19.12\pm0.071$  &  $-999999500.00\pm-999999500.000$   & $-999999500.00\pm-999999500.000$    &   $19.015\pm0.022$   &  $18.64\pm0.030$   &   $17.25\pm0.183$   &   $15.65\pm0.286$   \\
SDSS & J1523+3347 &  230.94042 &   33.79996 &  5.33   &   $-999999500.00\pm-999999500.000$  &  $19.90\pm0.111$  &  $-999999500.00\pm-999999500.000$   & $-999999500.00\pm-999999500.000$    &   $19.469\pm0.032$   &  $19.02\pm0.046$   &   $17.91\pm-999999488.000$   &   $15.90\pm-999999488.000$   \\
SDSS & J1524+0816 &  231.01708 &    8.27758 &  5.08   &   $20.70\pm0.172$  &  $20.53\pm0.121$  &  $20.35\pm0.181$   & $20.14\pm0.076$    &   $20.089\pm0.067$   &  $19.82\pm0.114$   &   $17.50\pm-999999488.000$   &   $15.66\pm-999999488.000$   \\
PSO & J231.6576-20.8335 &  231.65767 &  -20.83352 &  6.59   &   $-999999500.00\pm-999999500.000$  &  $19.60\pm0.077$  &  $-999999500.00\pm-999999500.000$   & $19.53\pm0.128$    &   $19.598\pm0.054$   &  $19.56\pm0.111$   &   $17.38\pm-999999488.000$   &   $15.60\pm-999999488.000$   \\
SUVAW & J1527+0641 &  231.80358 &    6.68942 &  5.57   &   $19.85\pm0.076$  &  $19.61\pm0.048$  &  $19.48\pm0.078$   & $19.55\pm0.095$    &   $19.516\pm0.041$   &  $19.50\pm0.087$   &   $17.97\pm0.406$   &   $15.88\pm-999999488.000$   \\
SDSS & J1534+1327 &  233.74899 &   13.45039 &  5.04   &   $-999999500.00\pm-999999500.000$  &  $20.62\pm0.222$  &  $-999999500.00\pm-999999500.000$   & $-999999500.00\pm-999999500.000$    &   $18.709\pm0.020$   &  $18.59\pm0.038$   &   $17.95\pm0.406$   &   $16.02\pm0.483$   \\
PSO & J235.9450+17.0079 &  235.94507 &   17.00791 &  5.82   &   $-999999500.00\pm-999999500.000$  &  $20.03\pm0.137$  &  $-999999500.00\pm-999999500.000$   & $-999999500.00\pm-999999500.000$    &   $19.616\pm0.043$   &  $19.66\pm0.096$   &   $17.50\pm0.315$   &   $15.63\pm-999999488.000$   \\
SHELLQs & J1545+4232 &  236.27342 &   42.53656 &  6.50   &   $-999999500.00\pm-999999500.000$  &  $22.66\pm1.050$  &  $-999999500.00\pm-999999500.000$   & $-999999500.00\pm-999999500.000$    &   $-999999485.331\pm-999999488.000$   &  $-999999484.72\pm-999999488.000$   &   $-999999482.85\pm-999999488.000$   &   $-999999481.34\pm-999999488.000$   \\
PSO & J236.2912+16.6088 &  236.29124 &   16.60886 &  5.82   &   $-999999500.00\pm-999999500.000$  &  $20.42\pm0.177$  &  $-999999500.00\pm-999999500.000$   & $-999999500.00\pm-999999500.000$    &   $19.632\pm0.047$   &  $-999999484.72\pm-999999488.000$   &   $17.32\pm-999999488.000$   &   $15.27\pm-999999488.000$   \\
SDSS & J1545+6028 &  236.46704 &   60.47332 &  5.78   &   $-999999500.00\pm-999999500.000$  &  $-999999500.00\pm-999999500.000$  &  $-999999500.00\pm-999999500.000$   & $-999999500.00\pm-999999500.000$    &   $18.683\pm0.014$   &  $18.43\pm0.023$   &   $17.46\pm0.231$   &   $16.07\pm0.435$   \\
SHELLQs & J1550+4318 &  237.50387 &   43.30078 &  5.84   &   $-999999500.00\pm-999999500.000$  &  $24.65\pm9.982$  &  $-999999500.00\pm-999999500.000$   & $-999999500.00\pm-999999500.000$    &   $-999999485.331\pm-999999488.000$   &  $-999999484.72\pm-999999488.000$   &   $-999999482.85\pm-999999488.000$   &   $-999999481.34\pm-999999488.000$   \\
PSO & J238.8510-06.8976 &  238.85103 &   -6.89766 &  5.81   &   $20.21\pm0.149$  &  $20.42\pm0.241$  &  $20.51\pm0.468$   & $20.70\pm0.473$    &   $20.150\pm0.079$   &  $-999999484.72\pm-999999488.000$   &   $16.97\pm-999999488.000$   &   $14.95\pm-999999488.000$   \\
PSO & J239.7124-07.4026 &  239.71246 &   -7.40266 &  6.11   &   $19.56\pm0.074$  &  $19.37\pm0.073$  &  $19.26\pm0.099$   & $18.98\pm0.091$    &   $18.941\pm0.029$   &  $18.65\pm0.049$   &   $-999999482.85\pm-999999488.000$   &   $-999999481.34\pm-999999488.000$   \\
DELS & J1559+2212 &  239.78788 &   22.20401 &  6.07   &   $-999999500.00\pm-999999500.000$  &  $20.78\pm0.244$  &  $-999999500.00\pm-999999500.000$   & $-999999500.00\pm-999999500.000$    &   $19.766\pm0.047$   &  $19.62\pm0.089$   &   $17.42\pm-999999488.000$   &   $15.51\pm-999999488.000$   \\
SDWISE & J1601-1828 &  240.29650 &  -18.47641 &  5.06   &   $-999999500.00\pm-999999500.000$  &  $19.08\pm0.062$  &  $18.72\pm0.060$   & $18.60\pm0.021$    &   $18.275\pm0.019$   &  $18.35\pm0.042$   &   $16.80\pm0.252$   &   $15.17\pm0.457$   \\
SDSS & J1602+4228 &  240.72491 &   42.47360 &  6.09   &   $19.65\pm0.066$  &  $19.53\pm0.060$  &  $19.15\pm0.061$   & $18.95\pm0.063$    &   $18.704\pm0.017$   &  $18.54\pm0.029$   &   $17.52\pm0.256$   &   $16.01\pm-999999488.000$   \\
ELAIS & 1091000446 &  240.95446 &   55.17564 &  6.04   &   $-999999500.00\pm-999999500.000$  &  $-999999488.00\pm-999999488.000$  &  $-999999500.00\pm-999999500.000$   & $24.29\pm0.718$    &   $-999999485.331\pm-999999488.000$   &  $-999999484.72\pm-999999488.000$   &   $-999999482.85\pm-999999488.000$   &   $-999999481.34\pm-999999488.000$   \\
ULAS & J1609+3041 &  242.40529 &   30.69661 &  6.14   &   $20.67\pm0.118$  &  $20.49\pm0.096$  &  $20.17\pm0.190$   & $20.10\pm0.228$    &   $20.311\pm0.071$   &  $20.32\pm0.152$   &   $17.61\pm-999999488.000$   &   $15.92\pm-999999488.000$   \\
PSO & J242.4397-12.9816 &  242.43971 &  -12.98170 &  5.83   &   $-999999500.00\pm-999999500.000$  &  $19.71\pm0.094$  &  $-999999500.00\pm-999999500.000$   & $19.46\pm0.256$    &   $19.238\pm0.039$   &  $19.50\pm0.105$   &   $17.01\pm0.324$   &   $14.91\pm-999999488.000$   \\
SDSS & J1610+4117 &  242.56967 &   41.29827 &  5.01   &   $-999999500.00\pm-999999500.000$  &  $19.91\pm0.123$  &  $-999999500.00\pm-999999500.000$   & $-999999500.00\pm-999999500.000$    &   $19.252\pm0.026$   &  $19.35\pm0.058$   &   $17.78\pm-999999488.000$   &   $16.11\pm-999999488.000$   \\
SDSS & J1614+4640 &  243.60471 &   46.67471 &  5.31   &   $-999999500.00\pm-999999500.000$  &  $19.59\pm0.086$  &  $-999999500.00\pm-999999500.000$   & $-999999500.00\pm-999999500.000$    &   $18.488\pm0.014$   &  $18.26\pm0.023$   &   $18.07\pm0.335$   &   $15.75\pm-999999488.000$   \\
SDSS & J1614+2059 &  243.69600 &   20.98416 &  5.09   &   $-999999500.00\pm-999999500.000$  &  $19.53\pm0.085$  &  $-999999500.00\pm-999999500.000$   & $-999999500.00\pm-999999500.000$    &   $19.420\pm0.034$   &  $19.44\pm0.074$   &   $17.49\pm0.382$   &   $15.67\pm-999999488.000$   \\
PSO & J245.0636-00.1978 &  245.06368 &   -0.19786 &  5.68   &   $20.94\pm0.230$  &  $21.07\pm0.216$  &  $21.96\pm0.747$   & $20.81\pm0.382$    &   $20.789\pm0.125$   &  $-999999484.72\pm-999999488.000$   &   $-999999482.85\pm-999999488.000$   &   $-999999481.34\pm-999999488.000$   \\
SDSS & J1621+5155 &  245.25383 &   51.93022 &  5.71   &   $-999999500.00\pm-999999500.000$  &  $19.45\pm0.097$  &  $-999999500.00\pm-999999500.000$   & $-999999500.00\pm-999999500.000$    &   $18.324\pm0.011$   &  $18.11\pm0.019$   &   $18.04\pm0.316$   &   $16.19\pm-999999488.000$   \\
SDWISE & J1623+4705 &  245.81367 &   47.09997 &  5.13   &   $-999999500.00\pm-999999500.000$  &  $18.74\pm0.048$  &  $-999999500.00\pm-999999500.000$   & $-999999500.00\pm-999999500.000$    &   $18.227\pm0.011$   &  $18.14\pm0.020$   &   $16.57\pm0.096$   &   $15.61\pm0.276$   \\
SDSS & J1623+3112 &  245.88256 &   31.20015 &  6.26   &   $20.43\pm0.099$  &  $19.70\pm0.054$  &  $19.71\pm0.075$   & $19.56\pm0.069$    &   $19.330\pm0.030$   &  $19.02\pm0.049$   &   $17.70\pm-999999488.000$   &   $15.56\pm-999999488.000$   \\
SDSS & J1626+2751 &  246.61042 &   27.85903 &  5.16   &   $18.48\pm0.022$  &  $18.22\pm0.015$  &  $17.94\pm0.023$   & $17.84\pm0.027$    &   $17.669\pm0.009$   &  $17.51\pm0.015$   &   $17.07\pm0.255$   &   $15.10\pm-999999488.000$   \\
SDSS & J1626+2858 &  246.62167 &   28.98266 &  5.04   &   $19.63\pm0.045$  &  $19.52\pm0.027$  &  $19.37\pm0.015$   & $19.47\pm0.078$    &   $19.293\pm0.029$   &  $19.26\pm0.059$   &   $17.48\pm0.353$   &   $15.84\pm-999999488.000$   \\
PSO & J247.2970+24.1277 &  247.29707 &   24.12771 &  6.48   &   $-999999500.00\pm-999999500.000$  &  $20.44\pm0.188$  &  $-999999500.00\pm-999999500.000$   & $-999999500.00\pm-999999500.000$    &   $19.333\pm0.031$   &  $19.20\pm0.057$   &   $17.43\pm0.396$   &   $15.23\pm-999999488.000$   \\
SDSS & J1630+4012 &  247.64126 &   40.20269 &  6.07   &   $20.75\pm0.228$  &  $20.45\pm0.139$  &  $20.31\pm0.238$   & $20.13\pm0.214$    &   $20.129\pm0.052$   &  $20.19\pm0.117$   &   $18.06\pm-999999488.000$   &   $15.97\pm-999999488.000$   \\
CFHQS & J1641+3755 &  250.34053 &   37.92226 &  6.05   &   $-999999500.00\pm-999999500.000$  &  $21.14\pm0.261$  &  $-999999488.00\pm-999999488.000$   & $20.84\pm0.370$    &   $20.572\pm0.075$   &  $20.54\pm0.153$   &   $-999999482.85\pm-999999488.000$   &   $-999999481.34\pm-999999488.000$   \\
SDWISE & J1656+4541 &  254.14775 &   45.68710 &  5.34   &   $-999999500.00\pm-999999500.000$  &  $19.02\pm0.045$  &  $-999999500.00\pm-999999500.000$   & $-999999500.00\pm-999999500.000$    &   $18.920\pm0.018$   &  $18.79\pm0.032$   &   $17.83\pm0.383$   &   $15.70\pm-999999488.000$   \\
SDSS & J1659+2709 &  254.75883 &   27.15977 &  5.31   &   $-999999500.00\pm-999999500.000$  &  $18.68\pm0.042$  &  $-999999500.00\pm-999999500.000$   & $-999999500.00\pm-999999500.000$    &   $18.575\pm0.017$   &  $18.34\pm0.028$   &   $16.68\pm0.158$   &   $15.55\pm-999999488.000$   \\
SDWISE & J1659+3239 &  254.96263 &   32.65795 &  5.17   &   $-999999500.00\pm-999999500.000$  &  $19.61\pm0.093$  &  $-999999500.00\pm-999999500.000$   & $-999999500.00\pm-999999500.000$    &   $18.989\pm0.022$   &  $18.89\pm0.042$   &   $17.27\pm-999999488.000$   &   $15.28\pm-999999488.000$   \\
PSO & J261.0364+19.0286 &  261.03643 &   19.02864 &  6.44   &   $-999999500.00\pm-999999500.000$  &  $20.88\pm0.211$  &  $20.34\pm0.504$   & $20.23\pm0.195$    &   $20.338\pm0.078$   &  $20.39\pm0.172$   &   $17.50\pm-999999488.000$   &   $15.62\pm-999999488.000$   \\
PSO & J267.0021+22.7812 &  267.00211 &   22.78121 &  5.95   &   $-999999500.00\pm-999999500.000$  &  $-999999488.00\pm-999999488.000$  &  $-999999500.00\pm-999999500.000$   & $-999999500.00\pm-999999500.000$    &   $-999999485.331\pm-999999488.000$   &  $-999999484.72\pm-999999488.000$   &   $-999999482.85\pm-999999488.000$   &   $-999999481.34\pm-999999488.000$   \\
SDWISE & J1752+5036 &  268.18375 &   50.60918 &  5.02   &   $-999999500.00\pm-999999500.000$  &  $18.54\pm0.012$  &  $-999999500.00\pm-999999500.000$   & $-999999500.00\pm-999999500.000$    &   $17.770\pm0.008$   &  $17.71\pm0.014$   &   $17.76\pm0.374$   &   $15.95\pm0.438$   \\
PSO & J293.0317+71.6523 &  293.03177 &   71.65234 &  6.08   &   $-999999500.00\pm-999999500.000$  &  $-999999500.00\pm-999999500.000$  &  $-999999500.00\pm-999999500.000$   & $-999999500.00\pm-999999500.000$    &   $19.660\pm0.031$   &  $19.55\pm0.059$   &   $18.74\pm-999999488.000$   &   $16.35\pm-999999488.000$   \\
PSO & J308.0416-21.2339 &  308.04164 &  -21.23397 &  6.23   &   $20.35\pm0.051$  &  $20.19\pm0.065$  &  $19.87\pm0.187$   & $19.34\pm0.059$    &   $19.167\pm0.037$   &  $18.88\pm0.063$   &   $17.59\pm-999999488.000$   &   $14.81\pm-999999488.000$   \\
PSO & J308.4829-27.6485 &  308.48297 &  -27.64850 &  5.80   &   $19.64\pm0.101$  &  $19.79\pm0.104$  &  $19.77\pm0.126$   & $19.63\pm0.147$    &   $19.500\pm0.049$   &  $19.16\pm0.077$   &   $17.04\pm-999999488.000$   &   $15.29\pm-999999488.000$   \\
SDSS & J2053+0047 &  313.34070 &    0.78522 &  5.92   &   $21.57\pm0.453$  &  $20.89\pm0.141$  &  $20.36\pm0.139$   & $20.31\pm0.123$    &   $20.282\pm0.084$   &  $-999999484.72\pm-999999488.000$   &   $-999999482.85\pm-999999488.000$   &   $-999999481.34\pm-999999488.000$   \\
SDSS & J2054-0005 &  313.52704 &   -0.08744 &  6.04   &   $21.22\pm0.327$  &  $20.61\pm0.083$  &  $20.22\pm0.083$   & $20.27\pm0.101$    &   $19.847\pm0.058$   &  $19.77\pm0.119$   &   $-999999482.85\pm-999999488.000$   &   $-999999481.34\pm-999999488.000$   \\
CFHQS & J2100-1715 &  315.22758 &  -17.25625 &  6.08   &   $23.32\pm2.265$  &  $21.16\pm0.412$  &  $-999999500.00\pm-999999500.000$   & $21.10\pm0.682$    &   $20.108\pm0.088$   &  $-999999484.72\pm-999999488.000$   &   $-999999482.85\pm-999999488.000$   &   $-999999481.34\pm-999999488.000$   \\
SDSS & J2118-0003 &  319.55304 &   -0.06408 &  5.46   &   $20.96\pm0.283$  &  $21.02\pm0.099$  &  $20.89\pm0.125$   & $20.58\pm0.060$    &   $20.411\pm0.098$   &  $-999999484.72\pm-999999488.000$   &   $-999999482.85\pm-999999488.000$   &   $-999999481.34\pm-999999488.000$   \\
PSO & J319.6040-10.9326 &  319.60403 &  -10.93262 &  5.90   &   $19.84\pm0.047$  &  $19.89\pm0.066$  &  $-999999500.00\pm-999999500.000$   & $19.81\pm0.149$    &   $18.907\pm0.030$   &  $18.74\pm0.055$   &   $17.04\pm-999999488.000$   &   $15.43\pm-999999488.000$   \\
SDSS & J2119+1029 &  319.86800 &   10.48517 &  5.18   &   $-999999500.00\pm-999999500.000$  &  $20.09\pm0.163$  &  $-999999500.00\pm-999999500.000$   & $-999999500.00\pm-999999500.000$    &   $19.720\pm0.049$   &  $19.74\pm0.108$   &   $17.20\pm-999999488.000$   &   $15.42\pm-999999488.000$   \\
SDSS & J2119-0040 &  319.96621 &   -0.67225 &  5.87   &   $22.36\pm0.940$  &  $21.52\pm0.138$  &  $21.98\pm0.317$   & $21.40\pm0.120$    &   $20.882\pm0.144$   &  $-999999484.72\pm-999999488.000$   &   $-999999482.85\pm-999999488.000$   &   $-999999481.34\pm-999999488.000$   \\
PSO & J320.8703-24.3604 &  320.87033 &  -24.36040 &  5.73   &   $20.23\pm0.064$  &  $19.81\pm0.065$  &  $-999999500.00\pm-999999500.000$   & $19.55\pm0.113$    &   $19.756\pm0.059$   &  $19.94\pm0.152$   &   $16.80\pm-999999488.000$   &   $15.18\pm-999999488.000$   \\
PSO & J323.1382+12.2986 &  323.13830 &   12.29868 &  6.59   &   $-999999500.00\pm-999999500.000$  &  $19.63\pm0.107$  &  $-999999500.00\pm-999999500.000$   & $-999999500.00\pm-999999500.000$    &   $18.706\pm0.021$   &  $18.85\pm0.051$   &   $17.46\pm-999999488.000$   &   $15.61\pm-999999488.000$   \\
SUVAW & J2142-0120 &  325.66362 &   -1.33342 &  5.61   &   $-999999500.00\pm-999999500.000$  &  $20.22\pm0.108$  &  $20.13\pm0.133$   & $19.79\pm0.101$    &   $19.733\pm0.053$   &  $19.42\pm0.092$   &   $17.67\pm-999999488.000$   &   $15.36\pm-999999488.000$   \\
SDSS & J2147+0107 &  326.98087 &    1.13203 &  5.81   &   $21.41\pm0.273$  &  $21.00\pm0.111$  &  $21.32\pm0.259$   & $20.94\pm0.199$    &   $20.699\pm0.122$   &  $-999999484.72\pm-999999488.000$   &   $17.45\pm-999999488.000$   &   $15.54\pm-999999488.000$   \\
PSO & J328.7339-09.5076 &  328.73400 &   -9.50763 &  5.92   &   $20.39\pm0.096$  &  $20.19\pm0.127$  &  $-999999500.00\pm-999999500.000$   & $20.00\pm0.224$    &   $20.410\pm0.099$   &  $-999999484.72\pm-999999488.000$   &   $-999999482.85\pm-999999488.000$   &   $-999999481.34\pm-999999488.000$   \\
SDWISE & J2201+0302 &  330.27762 &    3.03547 &  5.06   &   $19.21\pm0.008$  &  $18.98\pm0.008$  &  $18.67\pm0.039$   & $18.66\pm0.050$    &   $18.612\pm0.021$   &  $18.69\pm0.047$   &   $16.46\pm0.186$   &   $14.49\pm0.218$   \\
SHELLQs & J2201+0155 &  330.38362 &    1.92472 &  6.16   &   $24.99\pm1.314$  &  $24.96\pm0.713$  &  $24.05\pm-999999488.000$   & $-999999500.00\pm-999999488.000$    &   $-999999485.331\pm-999999488.000$   &  $-999999484.72\pm-999999488.000$   &   $-999999482.85\pm-999999488.000$   &   $-999999481.34\pm-999999488.000$   \\
SDWISE & J2202+1509 &  330.61154 &   15.16455 &  5.07   &   $-999999500.00\pm-999999500.000$  &  $18.56\pm0.035$  &  $-999999500.00\pm-999999500.000$   & $-999999500.00\pm-999999500.000$    &   $18.306\pm0.015$   &  $18.43\pm0.035$   &   $17.32\pm0.313$   &   $15.18\pm-999999488.000$   \\
MMT & J2202+0131 &  330.63833 &    1.52231 &  5.23   &   $22.14\pm0.072$  &  $22.08\pm0.041$  &  $20.55\pm0.395$   & $20.80\pm0.425$    &   $-999999485.331\pm-999999488.000$   &  $-999999484.72\pm-999999488.000$   &   $-999999482.85\pm-999999488.000$   &   $-999999481.34\pm-999999488.000$   \\
IMS & J2204+0012 &  331.07467 &    1.19578 &  5.94   &   $-999999500.00\pm-999999488.000$  &  $22.44\pm0.100$  &  $21.56\pm0.332$   & $24.07\pm3.423$    &   $-999999485.331\pm-999999488.000$   &  $-999999484.72\pm-999999488.000$   &   $-999999482.85\pm-999999488.000$   &   $-999999481.34\pm-999999488.000$   \\
SDWISE & J2207-0416 &  331.79217 &   -4.28230 &  5.53   &   $18.66\pm0.031$  &  $18.79\pm0.035$  &  $18.27\pm0.031$   & $18.14\pm0.036$    &   $17.814\pm0.012$   &  $17.40\pm0.017$   &   $17.36\pm0.461$   &   $15.04\pm-999999488.000$   \\
SHELLQs & J2210+0304 &  332.61350 &    3.07458 &  6.90   &   $23.13\pm0.296$  &  $22.21\pm0.125$  &  $22.06\pm1.167$   & $22.96\pm2.682$    &   $-999999485.331\pm-999999488.000$   &  $-999999484.72\pm-999999488.000$   &   $-999999482.85\pm-999999488.000$   &   $-999999481.34\pm-999999488.000$   \\
ATLAS & J332.8017-32.1036 &  332.80175 &  -32.10356 &  6.34   &   $19.91\pm0.032$  &  $19.65\pm0.026$  &  $19.40\pm0.050$   & $19.07\pm0.031$    &   $18.920\pm0.027$   &  $18.80\pm0.055$   &   $17.30\pm-999999488.000$   &   $15.08\pm-999999488.000$   \\
SDSS & J2211+0011 &  332.92087 &    0.18858 &  5.23   &   $21.74\pm0.503$  &  $21.73\pm0.036$  &  $21.08\pm0.212$   & $21.05\pm0.030$    &   $20.734\pm0.131$   &  $-999999484.72\pm-999999488.000$   &   $-999999482.85\pm-999999488.000$   &   $-999999481.34\pm-999999488.000$   \\
SDSS & J2212-0042 &  333.21454 &   -0.70853 &  5.42   &   $20.71\pm0.226$  &  $20.42\pm0.011$  &  $19.97\pm0.021$   & $19.85\pm0.009$    &   $19.777\pm0.057$   &  $20.04\pm0.156$   &   $17.45\pm-999999488.000$   &   $15.22\pm-999999488.000$   \\
MMT & J2213+0034 &  333.27192 &    0.56883 &  5.31   &   $22.17\pm0.141$  &  $22.16\pm0.047$  &  $21.97\pm0.062$   & $21.84\pm0.056$    &   $-999999485.331\pm-999999488.000$   &  $-999999484.72\pm-999999488.000$   &   $-999999482.85\pm-999999488.000$   &   $-999999481.34\pm-999999488.000$   \\
MMT & J2215-0009 &  333.83425 &   -0.15233 &  5.28   &   $21.48\pm0.357$  &  $21.64\pm0.030$  &  $21.29\pm0.045$   & $21.12\pm0.028$    &   $20.979\pm0.161$   &  $-999999484.72\pm-999999488.000$   &   $-999999482.85\pm-999999488.000$   &   $-999999481.34\pm-999999488.000$   \\
PSO & J333.9859+26.1081 &  333.98598 &   26.10817 &  6.03   &   $-999999500.00\pm-999999500.000$  &  $20.44\pm0.142$  &  $-999999500.00\pm-999999500.000$   & $-999999500.00\pm-999999500.000$    &   $20.089\pm0.067$   &  $19.95\pm0.127$   &   $-999999482.85\pm-999999488.000$   &   $-999999481.34\pm-999999488.000$   \\
SDSS & J2216+0013 &  334.18342 &    0.23003 &  5.01   &   $20.30\pm0.010$  &  $20.16\pm0.008$  &  $19.99\pm0.099$   & $19.70\pm0.008$    &   $19.737\pm0.055$   &  $19.76\pm0.121$   &   $17.14\pm-999999488.000$   &   $15.58\pm-999999488.000$   \\
HSC & J2216-0016 &  334.18529 &   -0.28058 &  6.10   &   $22.13\pm0.645$  &  $22.80\pm0.112$  &  $22.00\pm0.324$   & $22.36\pm0.100$    &   $-999999485.331\pm-999999488.000$   &  $-999999484.72\pm-999999488.000$   &   $-999999482.85\pm-999999488.000$   &   $-999999481.34\pm-999999488.000$   \\
VIMOS & 2911001793 &  334.82175 &    1.04692 &  6.16   &   $-999999500.00\pm-999999488.000$  &  $24.18\pm0.276$  &  $23.24\pm0.225$   & $22.93\pm0.132$    &   $-999999485.331\pm-999999488.000$   &  $-999999484.72\pm-999999488.000$   &   $-999999482.85\pm-999999488.000$   &   $-999999481.34\pm-999999488.000$   \\
SDSS & J2220-0101 &  335.07704 &   -1.02969 &  5.62   &   $20.38\pm0.101$  &  $20.29\pm0.040$  &  $20.14\pm0.051$   & $19.77\pm0.049$    &   $19.558\pm0.049$   &  $19.38\pm0.089$   &   $-999999482.85\pm-999999488.000$   &   $-999999481.34\pm-999999488.000$   \\
SHELLQs & J2223+0326 &  335.78963 &    3.43897 &  6.05   &   $21.56\pm0.367$  &  $20.88\pm0.253$  &  $21.10\pm0.649$   & $23.86\pm7.276$    &   $20.959\pm0.151$   &  $20.24\pm0.180$   &   $-999999482.85\pm-999999488.000$   &   $-999999481.34\pm-999999488.000$   \\
SDWISE & J2225+0330 &  336.30992 &    3.50347 &  5.35   &   $19.46\pm0.058$  &  $19.28\pm0.043$  &  $19.39\pm0.139$   & $19.19\pm0.106$    &   $19.024\pm0.029$   &  $18.92\pm0.057$   &   $17.14\pm-999999488.000$   &   $14.95\pm-999999488.000$   \\
SDWISE & J2226-0618 &  336.55171 &   -6.30202 &  5.08   &   $18.64\pm0.026$  &  $18.70\pm0.033$  &  $18.45\pm0.041$   & $18.35\pm0.042$    &   $18.377\pm0.018$   &  $18.32\pm0.037$   &   $17.36\pm0.430$   &   $15.48\pm-999999488.000$   \\
HSC & J2228+0128 &  337.11596 &    1.46931 &  6.01   &   $22.84\pm1.187$  &  $-999999488.00\pm-999999488.000$  &  $21.91\pm1.215$   & $-999999488.00\pm-999999488.000$    &   $-999999485.331\pm-999999488.000$   &  $-999999484.72\pm-999999488.000$   &   $-999999482.85\pm-999999488.000$   &   $-999999481.34\pm-999999488.000$   \\
SDSS & J2228+0110 &  337.18141 &    1.17561 &  5.95   &   $22.61\pm0.611$  &  $22.67\pm0.375$  &  $22.20\pm0.467$   & $21.89\pm0.348$    &   $-999999485.331\pm-999999488.000$   &  $-999999484.72\pm-999999488.000$   &   $-999999482.85\pm-999999488.000$   &   $-999999481.34\pm-999999488.000$   \\
SDSS & J2228-0757 &  337.18812 &   -7.96538 &  5.14   &   $19.88\pm0.066$  &  $19.63\pm0.074$  &  $-999999500.00\pm-999999500.000$   & $19.25\pm0.097$    &   $19.029\pm0.032$   &  $18.90\pm0.062$   &   $17.02\pm-999999488.000$   &   $15.64\pm-999999488.000$   \\
SHELLQs & J2228+0152 &  337.19879 &    1.87792 &  6.08   &   $23.16\pm1.396$  &  $22.42\pm0.959$  &  $21.76\pm0.961$   & $22.32\pm1.616$    &   $-999999485.331\pm-999999488.000$   &  $-999999484.72\pm-999999488.000$   &   $-999999482.85\pm-999999488.000$   &   $-999999481.34\pm-999999488.000$   \\
CFHQS & J2229+1457 &  337.25687 &   14.95250 &  6.15   &   $-999999500.00\pm-999999500.000$  &  $23.89\pm5.141$  &  $-999999500.00\pm-999999500.000$   & $-999999500.00\pm-999999500.000$    &   $-999999485.331\pm-999999488.000$   &  $-999999484.72\pm-999999488.000$   &   $-999999482.85\pm-999999488.000$   &   $-999999481.34\pm-999999488.000$   \\
SHELLQs & J2231-0035 &  337.95371 &   -0.59653 &  5.87   &   $-999999500.00\pm-999999500.000$  &  $23.34\pm0.310$  &  $21.99\pm0.369$   & $23.63\pm1.128$    &   $-999999485.331\pm-999999488.000$   &  $-999999484.72\pm-999999488.000$   &   $-999999482.85\pm-999999488.000$   &   $-999999481.34\pm-999999488.000$   \\
HSC & J2232+0012 &  338.05012 &    0.21067 &  6.18   &   $22.66\pm1.141$  &  $22.55\pm0.322$  &  $-999999500.00\pm-999999500.000$   & $-999999500.00\pm-999999500.000$    &   $-999999485.331\pm-999999488.000$   &  $-999999484.72\pm-999999488.000$   &   $-999999482.85\pm-999999488.000$   &   $-999999481.34\pm-999999488.000$   \\
PSO & J338.2298+29.5089 &  338.22977 &   29.50898 &  6.67   &   $-999999500.00\pm-999999500.000$  &  $20.46\pm0.117$  &  $-999999500.00\pm-999999500.000$   & $-999999500.00\pm-999999500.000$    &   $20.168\pm0.068$   &  $20.36\pm0.173$   &   $17.19\pm-999999488.000$   &   $15.60\pm-999999488.000$   \\
SDSS & J2233-0107 &  338.36517 &   -1.11789 &  5.11   &   $-999999500.00\pm-999999500.000$  &  $21.22\pm0.251$  &  $21.22\pm0.230$   & $21.16\pm0.287$    &   $-999999485.331\pm-999999488.000$   &  $-999999484.72\pm-999999488.000$   &   $-999999482.85\pm-999999488.000$   &   $-999999481.34\pm-999999488.000$   \\
HSC & J2236+0032 &  339.18575 &    0.54914 &  6.40   &   $-999999500.00\pm-999999488.000$  &  $22.90\pm0.429$  &  $22.54\pm0.705$   & $22.58\pm0.551$    &   $-999999485.331\pm-999999488.000$   &  $-999999484.72\pm-999999488.000$   &   $-999999482.85\pm-999999488.000$   &   $-999999481.34\pm-999999488.000$   \\
SDSS & J2238-0027 &  339.70917 &   -0.45050 &  5.17   &   $21.37\pm0.289$  &  $21.38\pm0.096$  &  $20.59\pm0.145$   & $20.95\pm0.118$    &   $20.734\pm0.133$   &  $-999999484.72\pm-999999488.000$   &   $-999999482.85\pm-999999488.000$   &   $-999999481.34\pm-999999488.000$   \\
SDSS & J2239+0030 &  339.78150 &    0.50628 &  5.09   &   $21.11\pm0.295$  &  $21.22\pm0.081$  &  $21.11\pm0.275$   & $20.69\pm0.120$    &   $20.530\pm0.111$   &  $-999999484.72\pm-999999488.000$   &   $-999999482.85\pm-999999488.000$   &   $-999999481.34\pm-999999488.000$   \\
SHELLQs & J2239+0207 &  339.94779 &    2.12986 &  6.26   &   $21.76\pm0.453$  &  $21.84\pm0.647$  &  $21.58\pm0.537$   & $21.03\pm0.427$    &   $-999999485.331\pm-999999488.000$   &  $-999999484.72\pm-999999488.000$   &   $-999999482.85\pm-999999488.000$   &   $-999999481.34\pm-999999488.000$   \\
PSO & J340.2041-18.6621 &  340.20417 &  -18.66217 &  6.01   &   $19.94\pm0.081$  &  $21.83\pm0.711$  &  $-999999500.00\pm-999999500.000$   & $19.58\pm0.173$    &   $19.222\pm0.039$   &  $18.85\pm0.062$   &   $17.48\pm-999999488.000$   &   $15.34\pm-999999488.000$   \\
CFHQS & J2242+0334 &  340.65645 &    3.57267 &  5.88   &   $22.60\pm0.899$  &  $21.72\pm0.533$  &  $22.45\pm1.077$   & $24.01\pm6.175$    &   $-999999485.331\pm-999999488.000$   &  $-999999484.72\pm-999999488.000$   &   $-999999482.85\pm-999999488.000$   &   $-999999481.34\pm-999999488.000$   \\
SDSS & J2245+0024 &  341.35112 &    0.40394 &  5.16   &   $21.71\pm0.582$  &  $21.55\pm0.358$  &  $20.97\pm0.355$   & $20.81\pm0.136$    &   $20.795\pm0.145$   &  $-999999484.72\pm-999999488.000$   &   $17.43\pm-999999488.000$   &   $15.25\pm-999999488.000$   \\
VDES & J2250-5015 &  342.50838 &  -50.26171 &  6.00   &   $-999999500.00\pm-999999500.000$  &  $19.17\pm0.037$  &  $18.96\pm0.042$   & $18.94\pm0.052$    &   $18.917\pm0.024$   &  $18.85\pm0.048$   &   $17.10\pm0.258$   &   $15.40\pm-999999488.000$   \\
SHELLQs & J2252+0225 &  343.02267 &    2.42553 &  6.12   &   $22.40\pm0.876$  &  $-999999488.00\pm-999999488.000$  &  $24.22\pm7.583$   & $-999999488.00\pm-999999488.000$    &   $-999999485.331\pm-999999488.000$   &  $-999999484.72\pm-999999488.000$   &   $-999999482.85\pm-999999488.000$   &   $-999999481.34\pm-999999488.000$   \\
SHELLQs & J2255+0251 &  343.90850 &    2.85739 &  6.34   &   $27.35\pm-999999488.000$  &  $-999999488.00\pm-999999488.000$  &  $21.47\pm0.476$   & $-999999488.00\pm-999999488.000$    &   $20.491\pm0.110$   &  $-999999484.72\pm-999999488.000$   &   $-999999482.85\pm-999999488.000$   &   $-999999481.34\pm-999999488.000$   \\
SHELLQs & J2304+0045 &  346.09571 &    0.75150 &  6.36   &   $25.14\pm-999999488.000$  &  $22.74\pm0.394$  &  $22.71\pm0.995$   & $22.23\pm0.475$    &   $-999999485.331\pm-999999488.000$   &  $-999999484.72\pm-999999488.000$   &   $-999999482.85\pm-999999488.000$   &   $-999999481.34\pm-999999488.000$   \\
SDSS & J2307+0031 &  346.89729 &    0.53039 &  5.87   &   $22.47\pm1.042$  &  $21.24\pm0.098$  &  $20.69\pm0.167$   & $20.32\pm0.070$    &   $19.924\pm0.063$   &  $19.65\pm0.111$   &   $16.95\pm-999999488.000$   &   $15.41\pm-999999488.000$   \\
SDSS & J2310+1855 &  347.66206 &   18.92220 &  6.00   &   $-999999500.00\pm-999999500.000$  &  $18.86\pm0.047$  &  $-999999500.00\pm-999999500.000$   & $-999999500.00\pm-999999500.000$    &   $18.544\pm0.018$   &  $18.58\pm0.039$   &   $17.42\pm0.441$   &   $15.82\pm-999999488.000$   \\
SDSS & J2312+0100 &  348.06850 &    1.01431 &  5.08   &   $21.58\pm0.553$  &  $21.05\pm0.066$  &  $20.47\pm0.088$   & $20.53\pm0.077$    &   $20.751\pm0.134$   &  $-999999484.72\pm-999999488.000$   &   $-999999482.85\pm-999999488.000$   &   $-999999481.34\pm-999999488.000$   \\
SDSS & J2315-0023 &  348.94404 &   -0.39947 &  6.12   &   $21.51\pm0.277$  &  $21.31\pm0.101$  &  $21.16\pm0.118$   & $20.68\pm0.116$    &   $20.004\pm0.071$   &  $19.93\pm0.142$   &   $17.32\pm-999999488.000$   &   $15.38\pm-999999488.000$   \\
VIK & J2318-3113 &  349.57646 &  -31.22954 &  6.44   &   $20.76\pm0.069$  &  $20.69\pm0.070$  &  $20.88\pm0.165$   & $20.47\pm0.112$    &   $20.770\pm0.133$   &  $-999999484.72\pm-999999488.000$   &   $-999999482.85\pm-999999488.000$   &   $-999999481.34\pm-999999488.000$   \\
CFHQS & J2318-0246 &  349.51166 &   -2.77611 &  6.05   &   $22.76\pm1.427$  &  $22.15\pm0.796$  &  $21.08\pm0.398$   & $20.39\pm0.308$    &   $20.845\pm0.144$   &  $-999999484.72\pm-999999488.000$   &   $-999999482.85\pm-999999488.000$   &   $-999999481.34\pm-999999488.000$   \\
SDSS & J2325+2628 &  351.30935 &   26.47995 &  5.77   &   $-999999500.00\pm-999999500.000$  &  $18.90\pm0.042$  &  $-999999500.00\pm-999999500.000$   & $-999999500.00\pm-999999500.000$    &   $18.807\pm0.022$   &  $18.77\pm0.045$   &   $17.74\pm0.507$   &   $15.63\pm0.478$   \\
SUVAW & J2325-0553 &  351.40267 &   -5.89119 &  5.22   &   $19.26\pm0.057$  &  $19.06\pm0.052$  &  $19.02\pm0.070$   & $18.99\pm0.084$    &   $18.992\pm0.030$   &  $18.92\pm0.060$   &   $17.58\pm0.437$   &   $15.09\pm-999999488.000$   \\
CFHQS & J2329-0301 &  352.28450 &   -3.03300 &  6.42   &   $21.14\pm0.392$  &  $22.20\pm0.931$  &  $20.96\pm0.411$   & $20.95\pm0.478$    &   $20.643\pm0.124$   &  $-999999484.72\pm-999999488.000$   &   $-999999482.85\pm-999999488.000$   &   $-999999481.34\pm-999999488.000$   \\
CFHQS & J2329-0403 &  352.31025 &   -4.05669 &  5.90   &   $25.00\pm9.756$  &  $23.11\pm1.729$  &  $-999999488.00\pm-999999488.000$   & $22.41\pm1.516$    &   $-999999485.331\pm-999999488.000$   &  $-999999484.72\pm-999999488.000$   &   $-999999482.85\pm-999999488.000$   &   $-999999481.34\pm-999999488.000$   \\
SDWISE & J2329+3003 &  352.41375 &   30.06411 &  5.24   &   $-999999500.00\pm-999999500.000$  &  $18.98\pm0.042$  &  $-999999500.00\pm-999999500.000$   & $-999999500.00\pm-999999500.000$    &   $18.819\pm0.022$   &  $18.80\pm0.045$   &   $17.80\pm-999999488.000$   &   $15.73\pm-999999488.000$   \\
SUVAW & J2330+0957 &  352.53629 &    9.96214 &  5.30   &   $19.79\pm0.058$  &  $19.68\pm0.072$  &  $19.17\pm0.069$   & $19.14\pm0.056$    &   $18.866\pm0.025$   &  $18.42\pm0.037$   &   $17.29\pm0.386$   &   $15.58\pm0.538$   \\
SDSS & J2334-0010 &  353.72937 &   -0.17281 &  5.11   &   $22.69\pm1.205$  &  $20.83\pm0.051$  &  $20.93\pm0.171$   & $20.84\pm0.120$    &   $20.672\pm0.125$   &  $-999999484.72\pm-999999488.000$   &   $-999999482.85\pm-999999488.000$   &   $-999999481.34\pm-999999488.000$   \\
SDWISE & J2344+1653 &  356.13958 &   16.88791 &  5.00   &   $-999999500.00\pm-999999500.000$  &  $18.53\pm0.033$  &  $-999999500.00\pm-999999500.000$   & $-999999500.00\pm-999999500.000$    &   $17.928\pm0.012$   &  $17.85\pm0.022$   &   $17.15\pm0.281$   &   $15.62\pm-999999488.000$   \\
VIK & J2348-3054 &  357.13890 &  -30.90284 &  6.90   &   $21.18\pm0.079$  &  $21.10\pm0.078$  &  $20.95\pm0.157$   & $20.52\pm0.110$    &   $20.364\pm0.090$   &  $-999999484.72\pm-999999488.000$   &   $17.29\pm-999999488.000$   &   $15.80\pm0.487$   \\
PSO & J357.8289+06.4019 &  357.82899 &    6.40192 &  5.81   &   $21.66\pm0.399$  &  $22.07\pm0.800$  &  $22.08\pm0.900$   & $21.31\pm0.516$    &   $-999999485.331\pm-999999488.000$   &  $-999999484.72\pm-999999488.000$   &   $-999999482.85\pm-999999488.000$   &   $-999999481.34\pm-999999488.000$   \\
SUVAW & J2351-0459 &  357.85129 &   -4.98536 &  5.25   &   $19.78\pm0.106$  &  $20.02\pm0.140$  &  $19.68\pm0.129$   & $19.56\pm0.133$    &   $19.770\pm0.056$   &  $19.37\pm0.090$   &   $17.70\pm-999999488.000$   &   $15.55\pm-999999488.000$   \\
PSO & J359.1352-06.3831 &  359.13521 &   -6.38313 &  6.17   &   $20.07\pm0.121$  &  $19.96\pm0.110$  &  $19.76\pm0.115$   & $19.41\pm0.109$    &   $19.159\pm0.032$   &  $18.95\pm0.061$   &   $17.04\pm-999999488.000$   &   $15.36\pm-999999488.000$   \\
SDSS & J2356+0023 &  359.21491 &    0.39258 &  6.00   &   $22.37\pm0.793$  &  $21.85\pm0.233$  &  $25.01\pm7.726$   & $21.77\pm0.444$    &   $-999999485.331\pm-999999488.000$   &  $-999999484.72\pm-999999488.000$   &   $-999999482.85\pm-999999488.000$   &   $-999999481.34\pm-999999488.000$   \\
SUVAW & J2358+0634 &  359.60017 &    6.57706 &  5.32   &   $19.38\pm0.066$  &  $19.50\pm0.107$  &  $19.11\pm0.068$   & $19.19\pm0.088$    &   $18.998\pm0.030$   &  $18.66\pm0.047$   &   $17.26\pm0.376$   &   $15.77\pm-999999488.000$   \\
UHS & J0439+1634 &   69.94617 &   16.57103 &  6.51   &   $-999999500.00\pm-999999500.000$  &  $17.47\pm0.016$  &  $-999999500.00\pm-999999500.000$   & $16.85\pm0.010$    &   $16.651\pm0.005$   &  $16.56\pm0.009$   &   $15.42\pm0.087$   &   $13.82\pm0.125$   \\
DELS & J0038-1527 &    9.65042 &  -15.45656 &  7.02   &   $-999999500.00\pm-999999500.000$  &  $-999999500.00\pm-999999500.000$  &  $-999999500.00\pm-999999500.000$   & $-999999500.00\pm-999999500.000$    &   $19.410\pm0.041$   &  $19.59\pm0.105$   &   $17.46\pm-999999488.000$   &   $15.36\pm-999999488.000$   \\
DELS & J0839+3900 &  129.94533 &   39.00319 &  6.91   &   $-999999500.00\pm-999999500.000$  &  $20.39\pm0.196$  &  $-999999500.00\pm-999999500.000$   & $-999999500.00\pm-999999500.000$    &   $19.090\pm0.031$   &  $18.98\pm0.061$   &   $17.39\pm-999999488.000$   &   $15.25\pm-999999488.000$   \\
DELS & J0411-0907 &   62.86929 &   -9.13050 &  6.81   &   $-999999500.00\pm-999999500.000$  &  $-999999500.00\pm-999999500.000$  &  $-999999500.00\pm-999999500.000$   & $-999999500.00\pm-999999500.000$    &   $19.494\pm0.043$   &  $19.33\pm0.079$   &   $17.77\pm-999999488.000$   &   $15.41\pm-999999488.000$   \\
DELS & J0829+4117 &  127.38321 &   41.29456 &  6.77   &   $-999999500.00\pm-999999500.000$  &  $20.26\pm0.146$  &  $-999999500.00\pm-999999500.000$   & $-999999500.00\pm-999999500.000$    &   $19.915\pm0.061$   &  $19.88\pm0.128$   &   $17.61\pm-999999488.000$   &   $15.68\pm-999999488.000$   \\
DELS & J1104+2134 &  166.08996 &   21.57467 &  6.74   &   $-999999500.00\pm-999999500.000$  &  $19.91\pm0.114$  &  $-999999500.00\pm-999999500.000$   & $-999999500.00\pm-999999500.000$    &   $19.894\pm0.059$   &  $19.81\pm0.124$   &   $17.80\pm-999999488.000$   &   $15.52\pm-999999488.000$   \\
DELS & J0910+1656 &  137.55679 &   16.94161 &  6.72   &   $-999999500.00\pm-999999500.000$  &  $20.74\pm0.269$  &  $-999999500.00\pm-999999500.000$   & $-999999500.00\pm-999999500.000$    &   $20.173\pm0.082$   &  $-999999484.72\pm-999999488.000$   &   $17.56\pm-999999488.000$   &   $15.72\pm-999999488.000$   \\
DELS & J0837+4929 &  129.40767 &   49.48344 &  6.71   &   $-999999500.00\pm-999999500.000$  &  $20.31\pm0.188$  &  $-999999500.00\pm-999999500.000$   & $-999999500.00\pm-999999500.000$    &   $19.923\pm0.061$   &  $19.29\pm0.074$   &   $17.73\pm-999999488.000$   &   $15.81\pm-999999488.000$   \\
DELS & J1216+4519 &  184.11492 &   45.31964 &  6.65   &   $-999999500.00\pm-999999500.000$  &  $21.27\pm0.454$  &  $-999999500.00\pm-999999500.000$   & $-999999500.00\pm-999999500.000$    &   $19.999\pm0.056$   &  $19.75\pm0.097$   &   $17.77\pm-999999488.000$   &   $15.66\pm-999999488.000$   \\
VHS & J2102-1458 &  315.58008 &  -14.98167 &  6.65   &   $20.96\pm0.202$  &  $21.03\pm0.280$  &  $-999999500.00\pm-999999500.000$   & $22.22\pm1.480$    &   $20.461\pm0.116$   &  $-999999484.72\pm-999999488.000$   &   $16.55\pm-999999488.000$   &   $15.37\pm-999999488.000$   \\
DELS & J0910-0414 &  137.72721 &   -4.23522 &  6.63   &   $-999999500.00\pm-999999500.000$  &  $20.23\pm0.073$  &  $-999999500.00\pm-999999500.000$   & $19.47\pm0.107$    &   $19.527\pm0.043$   &  $19.27\pm0.075$   &   $17.46\pm-999999488.000$   &   $15.79\pm-999999488.000$   \\
DELS & J0706+2921 &  106.60996 &   29.35153 &  6.58   &   $-999999500.00\pm-999999500.000$  &  $19.14\pm0.051$  &  $-999999500.00\pm-999999500.000$   & $-999999500.00\pm-999999500.000$    &   $18.610\pm0.022$   &  $18.63\pm0.046$   &   $17.58\pm0.483$   &   $15.20\pm0.340$   \\
DELS & J1135+5011 &  173.78721 &   50.19250 &  6.58   &   $-999999500.00\pm-999999500.000$  &  $20.44\pm0.172$  &  $-999999500.00\pm-999999500.000$   & $-999999500.00\pm-999999500.000$    &   $19.901\pm0.052$   &  $19.74\pm0.096$   &   $17.42\pm-999999488.000$   &   $15.41\pm-999999488.000$   \\
DELS & J1535+1943 &  233.88696 &   19.72225 &  6.40   &   $-999999500.00\pm-999999500.000$  &  $19.63\pm0.107$  &  $-999999500.00\pm-999999500.000$   & $-999999500.00\pm-999999500.000$    &   $18.553\pm0.018$   &  $18.46\pm0.034$   &   $17.73\pm0.346$   &   $15.97\pm0.449$   \\
DELS & J0803+3138 &  120.77258 &   31.64283 &  6.38   &   $-999999500.00\pm-999999500.000$  &  $20.19\pm0.133$  &  $-999999500.00\pm-999999500.000$   & $-999999500.00\pm-999999500.000$    &   $19.643\pm0.053$   &  $19.75\pm0.123$   &   $17.20\pm-999999488.000$   &   $15.37\pm0.402$   \\
DELS & J1316+1028 &  199.03392 &   10.47578 &  6.35   &   $20.87\pm0.148$  &  $20.74\pm0.109$  &  $20.79\pm0.351$   & $19.65\pm0.094$    &   $19.212\pm0.033$   &  $19.02\pm0.061$   &   $17.86\pm0.522$   &   $15.59\pm-999999488.000$   \\
SDSS & J0012+3632 &    3.13700 &   36.53781 &  5.44   &   $-999999500.00\pm-999999500.000$  &  $19.01\pm0.061$  &  $-999999500.00\pm-999999500.000$   & $-999999500.00\pm-999999500.000$    &   $18.490\pm0.017$   &  $18.51\pm0.036$   &   $17.15\pm0.235$   &   $15.35\pm0.329$   \\
SDSS & J0034+3759 &    8.55979 &   37.99833 &  5.63   &   $-999999500.00\pm-999999500.000$  &  $19.70\pm0.113$  &  $-999999500.00\pm-999999500.000$   & $-999999500.00\pm-999999500.000$    &   $19.149\pm0.029$   &  $19.01\pm0.056$   &   $17.18\pm-999999488.000$   &   $15.76\pm-999999488.000$   \\
SDSS & J0056+2241 &   14.23350 &   22.68671 &  5.49   &   $-999999500.00\pm-999999500.000$  &  $19.99\pm0.126$  &  $-999999500.00\pm-999999500.000$   & $-999999500.00\pm-999999500.000$    &   $19.605\pm0.048$   &  $19.28\pm0.078$   &   $17.33\pm-999999488.000$   &   $15.81\pm-999999488.000$   \\
SDSS & J0114+3238 &   18.72962 &   32.63787 &  5.22   &   $-999999500.00\pm-999999500.000$  &  $19.93\pm0.121$  &  $-999999500.00\pm-999999500.000$   & $-999999500.00\pm-999999500.000$    &   $19.515\pm0.041$   &  $19.46\pm0.085$   &   $17.64\pm-999999488.000$   &   $15.67\pm-999999488.000$   \\
SDSS & J0120+2147 &   20.22471 &   21.78506 &  5.42   &   $-999999500.00\pm-999999500.000$  &  $20.09\pm0.127$  &  $-999999500.00\pm-999999500.000$   & $-999999500.00\pm-999999500.000$    &   $19.216\pm0.033$   &  $19.20\pm0.072$   &   $17.61\pm-999999488.000$   &   $15.93\pm-999999488.000$   \\
SDSS & J0157+3001 &   29.43937 &   30.01963 &  5.63   &   $-999999500.00\pm-999999500.000$  &  $18.98\pm0.052$  &  $-999999500.00\pm-999999500.000$   & $-999999500.00\pm-999999500.000$    &   $18.111\pm0.014$   &  $17.94\pm0.025$   &   $17.09\pm-999999488.000$   &   $15.21\pm-999999488.000$   \\
SDSS & J1048+3339 &  162.15304 &   33.66324 &  5.61   &   $-999999500.00\pm-999999500.000$  &  $19.79\pm0.098$  &  $-999999500.00\pm-999999500.000$   & $-999999500.00\pm-999999500.000$    &   $19.977\pm0.061$   &  $19.84\pm0.118$   &   $17.44\pm-999999488.000$   &   $15.67\pm-999999488.000$   \\
SDSS & J1054+4637 &  163.52217 &   46.62507 &  5.47   &   $-999999500.00\pm-999999500.000$  &  $19.51\pm0.085$  &  $-999999500.00\pm-999999500.000$   & $-999999500.00\pm-999999500.000$    &   $19.373\pm0.035$   &  $19.23\pm0.065$   &   $17.30\pm-999999488.000$   &   $15.47\pm0.360$   \\
SDSS & J1218+1807 &  184.54662 &   18.13071 &  5.30   &   $-999999500.00\pm-999999500.000$  &  $20.14\pm0.134$  &  $-999999500.00\pm-999999500.000$   & $-999999500.00\pm-999999500.000$    &   $19.859\pm0.059$   &  $19.65\pm0.106$   &   $17.27\pm-999999488.000$   &   $15.33\pm-999999488.000$   \\
SDSS & J1236+4657 &  189.02521 &   46.95698 &  5.55   &   $-999999500.00\pm-999999500.000$  &  $19.61\pm0.084$  &  $-999999500.00\pm-999999500.000$   & $-999999500.00\pm-999999500.000$    &   $19.176\pm0.028$   &  $18.82\pm0.044$   &   $17.47\pm0.339$   &   $15.76\pm0.489$   \\
SDSS & J1314+5432 &  198.66837 &   54.54367 &  5.52   &   $-999999500.00\pm-999999500.000$  &  $19.71\pm0.086$  &  $-999999500.00\pm-999999500.000$   & $-999999500.00\pm-999999500.000$    &   $19.255\pm0.028$   &  $18.96\pm0.046$   &   $17.62\pm0.317$   &   $15.81\pm0.448$   \\
SDSS & J1500+2816 &  225.15350 &   28.26751 &  5.55   &   $-999999500.00\pm-999999500.000$  &  $19.19\pm0.072$  &  $-999999500.00\pm-999999500.000$   & $-999999500.00\pm-999999500.000$    &   $19.077\pm0.025$   &  $18.90\pm0.044$   &   $17.54\pm0.240$   &   $15.61\pm-999999488.000$   \\
SDSS & J1614+0114 &  243.64733 &    1.24578 &  5.78   &   $-999999500.00\pm-999999500.000$  &  $20.06\pm0.125$  &  $-999999500.00\pm-999999500.000$   & $-999999500.00\pm-999999500.000$    &   $19.529\pm0.042$   &  $19.44\pm0.085$   &   $17.67\pm-999999488.000$   &   $15.59\pm-999999488.000$   \\
SDSS & J1650+1617 &  252.67608 &   16.28931 &  5.52   &   $-999999500.00\pm-999999500.000$  &  $19.53\pm0.084$  &  $-999999500.00\pm-999999500.000$   & $-999999500.00\pm-999999500.000$    &   $18.866\pm0.023$   &  $18.70\pm0.042$   &   $17.01\pm-999999488.000$   &   $15.75\pm-999999488.000$   \\
SDSS & J2317+2244 &  349.40938 &   22.73601 &  5.50   &   $-999999500.00\pm-999999500.000$  &  $18.98\pm0.055$  &  $-999999500.00\pm-999999500.000$   & $-999999500.00\pm-999999500.000$    &   $18.794\pm0.022$   &  $18.64\pm0.042$   &   $17.65\pm0.532$   &   $15.37\pm-999999488.000$   \\
VDES & J0216-5226 &   34.16188 &  -52.43906 &  6.41   &   $-999999500.00\pm-999999500.000$  &  $21.22\pm0.257$  &  $-999999500.00\pm-999999500.000$   & $20.64\pm0.300$    &   $20.229\pm0.058$   &  $20.18\pm0.120$   &   $18.04\pm-999999488.000$   &   $15.38\pm-999999488.000$   \\
VDES & J0246-5219 &   41.73292 &  -52.33053 &  6.87   &   $-999999500.00\pm-999999500.000$  &  $21.20\pm0.135$  &  $-999999500.00\pm-999999500.000$   & $20.43\pm0.167$    &   $20.133\pm0.053$   &  $20.22\pm0.124$   &   $-999999482.85\pm-999999488.000$   &   $-999999481.34\pm-999999488.000$   \\
VDES & J0252-0503 &   43.06933 &   -5.05883 &  7.02   &   $-999999500.00\pm-999999500.000$  &  $-999999500.00\pm-999999500.000$  &  $-999999500.00\pm-999999500.000$   & $-999999500.00\pm-999999500.000$    &   $20.080\pm0.074$   &  $20.19\pm0.177$   &   $17.69\pm-999999488.000$   &   $15.68\pm-999999488.000$   \\
VDES & J0319-1008 &   49.92358 &  -10.14611 &  6.83   &   $21.14\pm0.276$  &  $20.88\pm0.295$  &  $-999999500.00\pm-999999500.000$   & $20.32\pm0.306$    &   $19.771\pm0.051$   &  $19.38\pm0.079$   &   $17.27\pm-999999488.000$   &   $15.56\pm-999999488.000$   \\
IMS & J0850-0506 &  132.61733 &   -5.10192 &  5.36   &   $21.79\pm0.080$  &  $22.34\pm0.172$  &  $-999999500.00\pm-999999500.000$   & $21.70\pm0.760$    &   $20.107\pm0.076$   &  $19.62\pm0.103$   &   $-999999482.85\pm-999999488.000$   &   $-999999481.34\pm-999999488.000$   \\
IMS & J1401+5143 &  210.45817 &   51.71953 &  5.17   &   $23.55\pm0.328$  &  $22.76\pm0.232$  &  $-999999500.00\pm-999999500.000$   & $-999999500.00\pm-999999500.000$    &   $-999999485.331\pm-999999488.000$   &  $-999999484.72\pm-999999488.000$   &   $-999999482.85\pm-999999488.000$   &   $-999999481.34\pm-999999488.000$   \\
VDES & J2131-4359 &  322.79287 &  -43.98403 &  6.45   &   $-999999500.00\pm-999999500.000$  &  $21.27\pm0.179$  &  $-999999500.00\pm-999999500.000$   & $20.62\pm0.232$    &   $20.671\pm0.111$   &  $-999999484.72\pm-999999488.000$   &   $-999999482.85\pm-999999488.000$   &   $-999999481.34\pm-999999488.000$   \\
IMS & J2206+0201 &  331.64504 &    2.02675 &  5.10   &   $22.19\pm0.133$  &  $22.13\pm0.081$  &  $21.63\pm1.051$   & $21.46\pm0.754$    &   $-999999485.331\pm-999999488.000$   &  $-999999484.72\pm-999999488.000$   &   $-999999482.85\pm-999999488.000$   &   $-999999481.34\pm-999999488.000$   \\
IMS & J2210+0243 &  332.65413 &    2.72047 &  5.20   &   $20.93\pm0.039$  &  $20.86\pm0.034$  &  $20.48\pm0.274$   & $20.36\pm0.249$    &   $20.481\pm0.102$   &  $-999999484.72\pm-999999488.000$   &   $17.55\pm-999999488.000$   &   $15.52\pm-999999488.000$   \\
VDES & J2211-6320 &  332.75250 &  -63.34883 &  6.88   &   $-999999500.00\pm-999999500.000$  &  $21.27\pm0.176$  &  $-999999500.00\pm-999999500.000$   & $21.07\pm0.433$    &   $20.877\pm0.122$   &  $-999999484.72\pm-999999488.000$   &   $-999999482.85\pm-999999488.000$   &   $-999999481.34\pm-999999488.000$   \\
SUHAW & J1016+2541 &  154.15713 &   25.69219 &  5.64   &   $-999999500.00\pm-999999500.000$  &  $18.80\pm0.046$  &  $-999999500.00\pm-999999500.000$   & $-999999500.00\pm-999999500.000$    &   $18.449\pm0.018$   &  $18.37\pm0.035$   &   $17.52\pm0.462$   &   $15.57\pm-999999488.000$   \\
PS1 & J0052+4556 &   13.18104 &   45.94223 &  5.31   &   $-999999500.00\pm-999999500.000$  &  $19.29\pm0.078$  &  $-999999500.00\pm-999999500.000$   & $-999999500.00\pm-999999500.000$    &   $19.080\pm0.027$   &  $18.92\pm0.050$   &   $17.66\pm0.357$   &   $15.95\pm-999999488.000$   \\
PS1 & J0332+1811 &   53.15408 &   18.19980 &  5.12   &   $-999999500.00\pm-999999500.000$  &  $19.32\pm0.072$  &  $-999999500.00\pm-999999500.000$   & $18.93\pm0.071$    &   $18.973\pm0.029$   &  $19.06\pm0.067$   &   $17.11\pm-999999488.000$   &   $15.59\pm0.520$   \\
PS1 & J0511-0754 &   77.97804 &   -7.91231 &  5.13   &   $-999999500.00\pm-999999500.000$  &  $19.59\pm0.058$  &  $-999999500.00\pm-999999500.000$   & $19.25\pm0.105$    &   $19.069\pm0.029$   &  $18.95\pm0.054$   &   $16.97\pm0.228$   &   $15.35\pm0.365$   \\
PS1 & J0616-1338 &   94.10158 &  -13.63511 &  5.58   &   $-999999500.00\pm-999999500.000$  &  $19.41\pm0.059$  &  $-999999500.00\pm-999999500.000$   & $19.06\pm0.091$    &   $19.013\pm0.029$   &  $18.70\pm0.045$   &   $17.79\pm0.529$   &   $15.63\pm-999999488.000$   \\
PS1 & J0757-0002 &  119.44125 &   -0.03364 &  5.54   &   $-999999500.00\pm-999999500.000$  &  $19.87\pm0.142$  &  $-999999500.00\pm-999999500.000$   & $19.07\pm0.140$    &   $18.783\pm0.025$   &  $18.37\pm0.037$   &   $16.94\pm-999999488.000$   &   $15.07\pm-999999488.000$   \\
PS1 & J0817-1633 &  124.25275 &  -16.55814 &  5.06   &   $-999999500.00\pm-999999500.000$  &  $19.06\pm0.036$  &  $-999999500.00\pm-999999500.000$   & $18.55\pm0.044$    &   $18.505\pm0.018$   &  $18.55\pm0.039$   &   $17.10\pm0.247$   &   $14.91\pm-999999488.000$   \\
PS1 & J1034-1233 &  158.65358 &  -12.56180 &  5.51   &   $19.93\pm0.081$  &  $20.08\pm0.117$  &  $19.51\pm0.163$   & $19.51\pm0.201$    &   $19.516\pm0.045$   &  $19.15\pm0.072$   &   $17.67\pm-999999488.000$   &   $15.15\pm-999999488.000$   \\
PS1 & J1057-1758 &  164.36500 &  -17.97547 &  5.34   &   $19.34\pm0.033$  &  $19.22\pm0.043$  &  $-999999500.00\pm-999999500.000$   & $18.78\pm0.061$    &   $18.873\pm0.026$   &  $18.53\pm0.041$   &   $17.14\pm0.351$   &   $15.30\pm-999999488.000$   \\
PS1 & J1121-0718 &  170.43187 &   -7.31102 &  5.71   &   $20.08\pm0.170$  &  $19.90\pm0.166$  &  $19.68\pm0.233$   & $19.72\pm0.202$    &   $19.684\pm0.053$   &  $19.43\pm0.091$   &   $16.95\pm-999999488.000$   &   $15.66\pm-999999488.000$   \\
PS1 & J1137-1049 &  174.39738 &  -10.82626 &  5.50   &   $19.58\pm0.052$  &  $19.51\pm0.047$  &  $19.40\pm0.056$   & $19.01\pm0.077$    &   $19.052\pm0.033$   &  $18.86\pm0.063$   &   $17.38\pm-999999488.000$   &   $15.41\pm-999999488.000$   \\
PS1 & J1310-0639 &  197.55462 &   -6.66432 &  5.06   &   $20.05\pm0.089$  &  $20.04\pm0.088$  &  $19.60\pm0.085$   & $19.53\pm0.116$    &   $19.169\pm0.035$   &  $19.25\pm0.079$   &   $17.26\pm0.365$   &   $15.52\pm0.471$   \\
PS1 & J1313-2617 &  198.35858 &  -26.28940 &  5.54   &   $19.21\pm0.044$  &  $19.10\pm0.047$  &  $-999999500.00\pm-999999500.000$   & $18.61\pm0.064$    &   $18.520\pm0.019$   &  $18.30\pm0.035$   &   $17.90\pm0.508$   &   $15.47\pm-999999488.000$   \\
PS1 & J1427-0503 &  216.83983 &   -5.06473 &  5.08   &   $18.84\pm0.034$  &  $18.84\pm0.031$  &  $18.55\pm0.048$   & $18.59\pm0.048$    &   $18.664\pm0.022$   &  $18.76\pm0.051$   &   $17.18\pm0.263$   &   $15.00\pm-999999488.000$   \\
PS1 & J1533-1810 &  233.49900 &  -18.17422 &  5.03   &   $18.76\pm0.024$  &  $18.61\pm0.025$  &  $-999999500.00\pm-999999500.000$   & $18.19\pm0.031$    &   $18.124\pm0.016$   &  $18.09\pm0.032$   &   $16.43\pm0.215$   &   $14.83\pm-999999488.000$   \\
PS1 & J2033+1218 &  308.29363 &   12.31430 &  5.11   &   $-999999500.00\pm-999999500.000$  &  $18.56\pm0.045$  &  $-999999500.00\pm-999999500.000$   & $-999999500.00\pm-999999500.000$    &   $18.154\pm0.014$   &  $18.24\pm0.030$   &   $17.48\pm0.506$   &   $15.53\pm-999999488.000$   \\
OGLE & J015531-752807 &   28.87921 &  -75.46861 &  5.09   &   $20.42\pm0.140$  &  $20.29\pm0.177$  &  $-999999500.00\pm-999999500.000$   & $20.10\pm0.271$    &   $19.584\pm0.031$   &  $19.68\pm0.070$   &   $17.41\pm0.223$   &   $15.95\pm-999999488.000$   \\
TN & J0924-2201 &  141.08300 &  -22.02819 &  5.19   &   $-999999500.00\pm-999999500.000$  &  $22.38\pm1.227$  &  $-999999500.00\pm-999999500.000$   & $21.76\pm1.228$    &   $-999999485.331\pm-999999488.000$   &  $-999999484.72\pm-999999488.000$   &   $-999999482.85\pm-999999488.000$   &   $-999999481.34\pm-999999488.000$   \\
XMM & J125329+30 &  193.37255 &   30.92762 &  5.08   &   $22.47\pm0.790$  &  $22.56\pm1.182$  &  $20.75\pm0.462$   & $20.96\pm0.442$    &   $20.303\pm0.079$   &  $-999999484.72\pm-999999488.000$   &   $-999999482.85\pm-999999488.000$   &   $-999999481.34\pm-999999488.000$   \\
SDSS & J141912.03+53 &  214.80013 &   53.67756 &  5.38   &   $-999999500.00\pm-999999500.000$  &  $20.30\pm0.057$  &  $-999999500.00\pm-999999500.000$   & $20.89\pm0.105$    &   $21.267\pm0.140$   &  $-999999484.72\pm-999999488.000$   &   $-999999482.85\pm-999999488.000$   &   $-999999481.34\pm-999999488.000$   \\
TGSS & J1530+1049 &  232.70792 &   10.82531 &  5.72   &   $-999999488.00\pm-999999488.000$  &  $23.24\pm1.266$  &  $-999999488.00\pm-999999488.000$   & $-999999488.00\pm-999999488.000$    &   $-999999485.331\pm-999999488.000$   &  $-999999484.72\pm-999999488.000$   &   $-999999482.85\pm-999999488.000$   &   $-999999481.34\pm-999999488.000$   \\
PSO & J352.4034-15.337 &  352.40348 &  -15.33735 &  5.84   &   $20.92\pm0.130$  &  $20.88\pm0.163$  &  $-999999500.00\pm-999999500.000$   & $20.64\pm0.306$    &   $20.439\pm0.110$   &  $-999999484.72\pm-999999488.000$   &   $-999999482.85\pm-999999488.000$   &   $-999999481.34\pm-999999488.000$   \\
PSO & J0046-2837 &   11.59854 &  -28.62982 &  5.99   &   $21.25\pm0.125$  &  $20.89\pm0.079$  &  $20.61\pm0.112$   & $20.22\pm0.111$    &   $19.732\pm0.050$   &  $19.68\pm0.105$   &   $17.46\pm-999999488.000$   &   $15.35\pm-999999488.000$   \\
VIK & J2318-3029 &  349.63794 &  -30.49260 &  6.15   &   $20.57\pm0.076$  &  $20.20\pm0.056$  &  $19.96\pm0.060$   & $19.68\pm0.059$    &   $19.390\pm0.040$   &  $19.47\pm0.093$   &   $17.43\pm-999999488.000$   &   $15.73\pm-999999488.000$   \\
HSC & 1732+6531 &  263.17966 &   65.52041 &  6.60   &   $-999999500.00\pm-999999500.000$  &  $-999999500.00\pm-999999500.000$  &  $-999999500.00\pm-999999500.000$   & $-999999500.00\pm-999999500.000$    &   $21.163\pm0.074$   &  $-999999484.72\pm-999999488.000$   &   $18.64\pm-999999488.000$   &   $16.25\pm-999999488.000$   \\
    \hline
    \hline
    \end{tabular}
    \caption{The first 23 (i.e. 5\%) of 463 very high-$z$ quasars in Right Ascension order with near and mid-infrared photometry.
                  The full table can be found \href{https://github.com/d80b2t/VHzQ/tree/master/data}{here}.
                  The AB magnitude system is used with the WISE Vega to AB offsets being ($\Delta$W1, $\Delta$W2, $\Delta$W3 $\Delta$W4)=(2.669, 3.281, 5.148, 6.66)
                  Since none of the first 23 objects have $Z$-band detections, we don't report that column here (but is reported in the main table).
                  WISE AllWISE W3 and W4 values without formal errors are low-SNR detections. 
                  } 
     \label{tab:output_table}
     \end{table}
     


==> notes_for_replacement <==

The Near and Mid-infrared photometric properties of known redshift $z\geq5$ Quasars

Nicholas P. Ross
Nicholas J. G. Cross 
Institute for Astronomy, University of Edinburgh, Royal Observatory, Edinburgh, EH9 3HJ, United Kingdom


We assemble a catalogue of 488 spectroscopically confirmed very high
($z\geq5.00$) redshift quasars and report their near- ($ZYJHK_{s}/K$)
and mid- (WISE W1234) infrared properties. 97\% of the VH$z$Q sample
is detected in one or more NIR ($ZYJHK/K_{s}$) band, with lack of
coverage rather than lack of depth being the reason for the
non-detections. 389 (80\%) of the very high redshift quasars are
detected at 3.4$\mu$m in the W1 band from the unWISE catalog and all
of the $z\geq7$ quasars are detected in both unWISE W1 and W2. Using
archival WFCAM/UKIRT and VIRCAM/VISTA data we check for photometric
variability that might be expected from super-Eddington accretion. We
find 28 of the quasars have sufficient NIR measurements and
signal-to-noise ratio to look for variability. Weak variability was detected
in multiple bands of SDSS J0959+0227, and very marginally in the
$Y$-band of MMT J0215-0529. Only one quasar, SDSS J0349+0034, shows
significant differences between WFCAM and VISTA magnitudes in one band.
With supermassive black hole accretion likely to be redshift invariant
up to very high-redshift, further monitoring of these sources is
warranted.  All the data, analysis codes and plots used and generated
here can be found at:
\href{https://github.com/d80b2t/VHzQ}{\tt github.com/d80b2t/VHzQ}.


Publication: 
Monthly Notices of the Royal Astronomical Society, Volume 494, Issue 1, pp.789-803
Pub Date: March 2020
DOI: 10.1093/mnras/staa544
Bibcode: 2020MNRAS.494..789R 

15 pages; 12 figures; 6 tables. Databases available at WFCAM Science Archive and the VISTA Science Archive. All data, analysis codes and plots can be found at github.com/d80b2t/VHzQ. Play the Five Tones.

